SANTOS: Relationship-based Semantic Table Union Search

Existing techniques for unionable table search define unionability using metadata (tables must have the same or similar schemas) or column-based metrics (for example, the values in a table should be drawn from the same domain). In this work, we introduce the use of semantic relationships between pairs of columns in a table to improve the accuracy of union search. Consequently, we introduce a new notion of unionability that considers relationships between columns, together with the semantics of columns, in a principled way. To do so, we present two new methods to discover semantic relationship between pairs of columns. The first uses an existing knowledge base (KB), the second (which we call a "synthesized KB") uses knowledge from the data lake itself. We adopt an existing Table Union Search benchmark and present new (open) benchmarks that represent small and large real data lakes. We show that our new unionability search algorithm, called SANTOS, outperforms a state-of-the-art union search that uses a wide variety of column-based semantics, including word embeddings and regular expressions. We show empirically that our synthesized KB improves the accuracy of union search by representing relationship semantics that may not be contained in an available KB. This result hints at a promising future of creating a synthesized KBs from data lakes with limited KB coverage and using them for union search.

==> sections/KB_details.tex <==
\subsection{Knowledge Base}
\label{section:knowledge_base}
SANTOS uses a Knowledge Base to create semantic graphs over the tables and annotate their columns and relationships.
%and understand the table semantics. 
% \wolf{3/23: Did you earlier describe what `table semantics' means? column types, and pairwise relationship semantics? 
% How does this problem related to the problem of ``table interpretation''? or is ``understanding the table semantics'' the same as ``table interpretation''?}
% \aamod{03/28: updated the sentence above. Rephrased and removed ``table semantics`` to avoid confusion.}
% For the purpose of this paper, a knowledge base is used to represent relationships between the concepts represented in each column explicitly.
%rjm this is resolved below
% \wolf{10/21: shortly describe the criteria of a knowledge base, relative to what it is used for. ``for the purpose of this paper, a knowledge base is an explicit representation between the concepts represented in each column'' (do we have an unambiuous name for that? In other words, one could use the column name to represent that concept from the knowledge base (if present)}
%  With minor changes, 
Broadly speaking, SANTOS can be used with any general, enterprise-level and domain-specific knowledge base (KB), 
such as DBpedia \cite{auer_07_dbpedia}, Wikidata \cite{vrande_14_wikidata}, YAGO \cite{tanon_20_yago}, Freebase \cite{DBLP:conf/sigmod/BollackerEPST08} and so on.
% \grace{3/17: Either here or in the experiments section, say we can also use a KB for enterprise data, and use the same approach}
%aamod: updated in the experiment section
For now, due to its clean type hierarchy and semantic consistencies in their predicate types (e.g. constraints on the possible predicates that each subject can have), 
%logically reasonable 
%and consistent semantic constraints, 
% \wolf{3/23: will the readers know what a semantic constraint is?} \aamod{we assume that readers have some experience with the KBs and refer them to YAGO. This is YAGO's main argument against DBPedia and wikidata. Should we go into more details?}
% \wolf{3/24: yes, please repeat in short the argument. Actually there are two:
% 1. type hierarchy: that's what you seem to explicitly use later.
% 2. semantic constraint: I don't know what this is. Is it essential for your method? If yes, then you anyway have to define it and explain how the methods uses those ``semantic constraints''}
% \aamod{03/28: In DBPedia, since it is extracted automatically, it has some triples like: company -> birthplace -> city. However, company should have location but not the birthplace. This is handled by YAGO by defining semantic constraints manually.
% As Semantic constraints do not have a lot to do, we decided to use type hierarchy only as motivation.}
we use YAGO 4~\cite{tanon_20_yago} for our evaluations. Hereafter, we will use YAGO interchangeably with YAGO 4. 

YAGO contains the set of entities and types where, 
%over 64 million entities and 10,124 types (or classes). 
each entity is mapped to at least one type. 
The types are taken from \url{https://schema.org}~\cite{guha_16_schema.org},
%\wolf{3/23: these links don't work. What would work is \url{https://schema.org}}
\url{https://bioschema.org}~\cite{Gray_17_bioschema.org}
and \url{https://wikidata.org}~\cite{vrande_14_wikidata}
and arranged in a consistent type hierarchy with \texttt{schema:Thing} as its root. Let $T$ be a set of all types. Any type $t \in T$ is a \textit{Top Level Type} if it is directly connected to the knowledge base root type.
% \wolf{3/24: 
% Define T: `Let $T$ be the set of 10,124 types.'
% Alternatively, further up introduce the symbols: `... a set [symbol] of 64 millions entities and set $T$ of 10,124 types...'}
% \aamod{03/28: We decided to remove the numbers (like 10,124 2714 etc. and just mention the types.}
%rjm resolved
%\wolf{10/19: ``type hierarchy'' here means relations as 
%Thus say ``living thing'' must be top type, correct? } \aamod{10/22: Yes, however we don't have living things explicitly in the KB. Person is an example of top level type and president can be its subtype.} Being the root of the hierarchy, schema:Thing does not have parent types and we call it ``Knowledge Base Root Type" throughout this paper. We use $T$ and $E$ to denote the set of all types and entities in the KB, respectively.
%\begin{definition}[Top Level Type]
%Any type $t \in T$ is a top level type if it is directly connected to the knowledge base root type.
%\end{definition}
%In our setup, 
%schema:Thing is the knowledge base root type
%\wolf{3/23: repeated statement from before}
%and 
%we have 2,714 \textit{Top Level Types}. 
\wolf{3/24: is it worth to add here a quick overview figure? Just so everyone is on the page: you'd show a top node,
then below an example path via place, location, city (or so) and have number of hierarchy levels and a few key statistics. 
You should definitely add that figure to your talk slides, because it helps show what is going on, and make sure everyone sees the "type hierarchy", but I would also add it to the online appendix, and optionally the paper if space permits. It's a simple figure that helps a first time reader enormously. And a figure that will be remembers after reading. 
Researchers / reviewers read several papers per days, it's figures that help remember important concepts. And here the type hierarchy seems to be essential}
\aamod{03/30: Yes, we have a slide showing the type hierarchy example (added to 2021\_SANTOS\_figures.pptx). However, due to space constraints, we did not add that to the paper.}
We use $T_{\mathit{top}}$ to denote a set of all top level types. Using the KB, we maintain four dictionaries
which we describe next:
% , namely, entity dictionary, inheritance dictionary, type dictionary, and relationship dictionary.

%We represent the set of all top level types using $T_{\mathit{top}}$.
%rjm resolved
% \wolf{10/19: suggestion: $T_{\mathrm{top}}$ or $T_{\mathit{top}}$}
% \roee{consider moving the technical part into an experimental settings section within the experiments section.} 




\introparagraph{1. Entity Dictionary} 
YAGO contains a set of KB entities each with a set of labels and alternate names (like synonyms) that describe the corresponding entity \footnote{\label{footnote:rdf_labels} \url{https://www.w3.org/2004/12/q/doc/rdf-labels.html}}. 
% \wolf{3/23: what is the meaning of those labels?}
% \aamod{3/23: They are standard KB labels and alternate names}
% \wolf{3/24: what are `standard' labels? I don't hink there is a standard for the word standard. It's unspecific. 
% Are labels synonyms, isA relationships, types? I would not know how to restrict the endless possibilities to define labels to those tha are standard}
% \aamod{03/28: added a footnote with a link to rdf query language.}
We store these 
%(and the entity Uniform Resource Identifiers or URIs) 
in a key-value dictionary that we call the {\em entity dictionary}.
The key is any label or alternate name and the value is the entity Uniform Resource Identifiers or URIs.\footnote{\label{footnote:labels_alternate_names}We only index labels and alternate names in English Language.
\wolf{3/23: how many of the originally 64 mio are left?}
\aamod{03/23: we keep all entities. Only alternate names are omitted. Each entity can have numerous alternate names.}
}
We connect tables with the KB by mapping the column values to the entity labels or the alternate names in the KB.
Note that YAGO permits  multiple entities to have the same label or alternate name. 
Hence, one value may be mapped to different entities with different types (that is, the value is a homograph with multiple meanings~\cite{21_leventidis_homograph_detection}).
%rjm:  this belongs in experiments
%For completeness, we now describe some more technical details on how we use YAGO in this paper. For querying the KB efficiently, we preprocess YAGO 4 files and convert them into four key-value dictionaries. First, we use label dictionary that stores the labels and alternate names in YAGO as keys and the list of the KB entities related to those labels and alternate names as values.
%For unique identification, we represent KB entities using their Uniform Resource Identifiers (URIs) in YAGO.


% \wolf{3/24: want to also add here a quick example. e.g. the william\_shakespear from fig 4: there this key gets mapped to several synonyms. If W.S. has 9 alternatives, does this dictionary have 10 entries for W.S.?}
% \aamod{03/29: If W.S has 9 alternatives, these 9 alternatives are keys in the dictionary and for all of them, the value is yago:William\_Shakespeare.
% For example, william shakespeare has one label: ``William Shakespeare`` and 1 alternate name: ``Shakespeare``. so, ``William Shakespeare`` and ``Shakespeare`` are keys and yago:William\_Shakespeare is a value for both of them. Should we add a table like other cases for this too?  
% }
\begin{figure}[h]
    \includegraphics[scale = 0.55]{110821_SIGMOD2022_Submission/figures/entity_dict.png}
\captionof{figure}{Entity dictionary example}
\label{fig:entity_dict}
\end{figure}

\introparagraph{2. Inheritance Dictionary} 
Next, we build 
%a {\em class dictionary} 
an {\em inheritance dictionary} that stores each Top level type as a key and the set of their children types as value. 
\wolf{3/23: @Mirek: is this the ``right'' definition: A key mapping to a set of values?
The values are then not atomic and can't be queried. Would it make more sense to have the 
children map to their unique parent? Thus way both the set of keys, and the set of values are atomic.}
An inheritance dictionary example 
%inline with our running example, 
is shown in \cref{fig:inheritance_dict}.
%For instance, {\em inheritance dictionary} has a top level type \texttt{place} as key having the set of its children \{administrative\_area, city, country, $\dots$\} as value.

% \begin{figure}[h]
%     \includegraphics[scale = 0.45]{110821_POST_VLDB_Submission/figures/yago_indexes.png}
%   \captionof{figure}{Example of the dictionaries built using YAGO.}
% \label{fig:yago_indexes}
% \end{figure}
\begin{figure}[h]
    \includegraphics[scale = 0.55]{figures/inheritance_dict.pdf}
\captionof{figure}{Inheritance dictionary example
% \wolf{3/24: Oh, I thought it was not just the `top level types' and wanted to point out the confusion. Like city could also be the key for some value like town? Or a chain artist-musician-piano player. Musician can also be in the left column, right?}
% \aamod{03/29: We only consider top level types as the keys. So, there are 2714 keys in this dictionary. The intuition is that: each column can be of 1 among 2714 top level types. Once we select the top level type for a column, we annotate it with that type and also its children types with difference confidence scores.}
}
\label{fig:inheritance_dict}
\end{figure}



\introparagraph{3. Type Dictionary} 
We use Type dictionary to lookup entities and find their types.
As a set of entities belonging to a descendant type is always a subset of entities belonging to its ancestor types in the knowledge base hierarchy,
the higher level types always have larger number of entities than lower level types and hence, receive unfair bias against the children types. 
%\updated{Grace 2/20: Can we say that the type-level 1's are a superset of the granular types? Or vice versa, the children types contain a subset of the higher-level types, inheriting the higher-level type while being more granular? Also, is it confusing to express type level 1's as higher level types?}
%aamod: Addressed by changing the text above.
In other words, for a pair of ancestor-descendant types, the ancestor type always appear more frequently, hence resulting in the bias towards it.
For instance, there are over 6M {places} in YAGO among which only 42k are {cities}.
From the perspective of the information theory, the less probable outcome has greater information \cite{mackay2003information}.
In our case, a type that appears more frequently is less informative.
For example, {cities} should be more informative than {places}.

Inspired by the well-known tf–idf measure~\cite{aizawa2003information}, we penalize the frequent ancestor types by using a frequency-based strategy utilizing knowledge base statistics and assign a \textit{type score} to each type.
The basic idea is to count the frequency of each type t by counting the entities that belong to t in the KB and penalize the frequent types.
The type score is computed based on the following formula \cref{eq:type_score}. 
A logarithm function is used here because we do not want excessive penalization that may make our algorithm ignore the case that the column is indeed of a top level type. 
%Also, to make the type score in $(0, 1]$, 
We ignore the types having less than 10 entities.
%don't penalize rare types whose appearance count is no more than 10.
\begin{equation}\label{eq:type_score}
    %ts(t) = \frac{1}{\log (max(t.count, 10))}
    ts(t) = \frac{1}{\log(t.count)}
\end{equation}

In this way, we prioritize granular types and penalize frequent types.
For example, $ts(place) = 0.1633$ and $ts(city) = 0.2115$.
% \wolf{3/24:
% You also need to explain why you care about keeping the level in the hierarchy around: is it used later?}
% \zixuan{3/28: We're trying to use it in the experiments now so I keep the levels here for now.}
% \wolf{3/24:
% ``
% Basic information theory, if a biased coin comes up 90\% head and 10\% tail, then every tail drop is more surprising and thus more informative [cite some intro to information theory book]. 
% In the same way, for us,
% a concept or type declaration that appears more frequently is less informative. 
% For example,  there are over 6M {places} in YAGO among which only 42k are {cities}.
% Thus the type declaration Boston isA city is more informative than Boston isA place.
% Inspired by tfid ... and with the log ...
% we consider city to be about 30\% more informative (0.2115 / 0.1633) than place. 
% [That is surprising that something that 100 times rares, gets only a 30\% boost: can you add some intuitive discussion why that ratio is good? Have you tried with different log bases, e.g. 100 times rares gives a 100\% boost, etc.?] ''}
% \zixuan{3/28: Paragraph updated. There is a trade-off here. We can't penalize the top type too much. Or there will be such case: The table is about places, containing 60\% cities and 40\% provinces. If we boost city too much like 100\%, this table is considered a table about cities.}

After getting the type scores, we build a {\em type dictionary} based on YAGO.
%which is similar to the (proprietary) isA database used to recover semantics of webtables~\cite{venetis_11_recovering_semantics}. 
Note that each key in the {\em type dictionary} must be a value 
%in at least one tuple of label 
in the  {\em entity dictionary}.

---

\wolf{! 3/24: So the intuition needs to come before the math, at the very start of the type dictionary section.
You also need to explain why you care about keeping the level in the hierarchy around: is it used later?
``
Basic information theory, if a biased coin comes up 90\% head and 10\% tail, then every tail drop is more surprising and thus more informative [cite some intro to information theory book]. 
In the same way, for us,
a concept or type declaration that appears more frequently is less informative. 
For example,  there are over 6M {places} in YAGO among which only 42k are {cities}.
Thus the type declaration Boston isA city is more informative than Boston isA place.
Inspired by tfid ... and with the log ...
we consider city to be about 30\% more informative (0.2115 / 0.1633) than place. 
[That is surprising that something that 100 times rares, gets only a 30\% boost: can you add some intuitive discussion why that ratio is good? Have you tried with different log bases, e.g. 100 times rares gives a 100\% boost, etc.?] ''}

---


% \wolf{3/23: I am confused: do you recreate / or do you create something from YAGO? But you can't `create' something that is part of YAGO because others did YAGO}
% \zixuan{3/28: Updated}
% \wolf{3/24: That other isA database also has weights like here or is just an isA graph? 
% Also, your type dictionary is actually a weighted type dictionary? Or more a type distribution? Because in a ``dictionary'' you normally look up one thing, here it is actually a distribution. That is not immediately intuitive.}
% \zixuan{3/28: It is still a dictionary. You look up for one entity in the dictionary, and it returns the type with type score and type level of that entity.}
If we look for an entity in this dictionary, the returned result is this entity and the set of tuples of its (type, type score, type level), where the type score of any type t, $ts(t) \in (0, 1]$ and \textit{type level} refers to its level in the type hierarchy i.e. the shortest path from the root.
For example, the entity \textit{boston}\footnote{\label{footnote:preprocessings}We convert all texts to lowercase and perform preprocessings like stemming and punctuation removal.} is a key in {\em type dictionary} as shown in \cref{fig:type_dict}. \textit{boston} is mapped to values $place$, which is a top level type so it has \textit{type level} = 1, and $city$, which is a descendant of $place$ and thus has \textit{type level} = 3.
% \wolf{3/24: interesting that here the word is not capitalized. Fig 1 shows capitalized words, later examples not. best to add somewhere a quick explanation with your convention}
%as shown in \cref{fig:yago_indexes}.


---

% \wolf{3/23: At this point I am left confused about the score. So it is not just a `dictionary' but a `type distribution'?
% What is the intuition of the distribution = ts? Is it a weight that is created not from YAGO itself, but from the data in the data lake?
% Thus may vary for different applications? 
% Because you explain the calculation in detail, what is the intuition of the calculations?}
% \zixuan{3/28: No. It is based on YAGO itself. Indeed we tried some strategies like TF-IDF to get some score based on the tables but after discussions in our meetings, we gave it up.}

\begin{figure}[h]
    \includegraphics[scale = 0.55]{figures/type_dict.pdf}
  \captionof{figure}{Type dictionary example}
\label{fig:type_dict}
\end{figure}

\introparagraph{4. Relationship Dictionary} 
Finally, we build a {\em relationship dictionary} to store the relationships (properties) from YAGO. As shown in \cref{fig:relationship_dict}, the keys are pairs of entities and each value is a set of tuples of (YAGO properties/binary relationships, type score). This dictionary is similar to the (proprietary) relation database used to recover semantics of webtables~\cite{venetis_11_recovering_semantics}.
As before, we again allow these relationships to be weighted to reflect a difference in importance. However in case of YAGO properties, we do not have hierarchy like YAGO types and hence, the type score is 1. Later in \cref{section:synthetic_knowledge_base}, we create synthesized KB and add entity pairs with non-integral type scores.
% \wolf{3/24: 1. So this dictionary just reflects the existing information in YAGO, right? In constrast to the type dictionary where you invent new value like distributions and hierarchy level?
% 2. `therefore the confidence score is 1': this sentence implies that you interpret the other log transformed frequency in the type dictionary as some confidence, but that is not really justified. Also I don't see why the `therefore' is justified here.
% 3. you likely keep the weights 1 here because you later in the synthetic KB you allow those values to be non integral. Thus motivate this here. Something like
% ``as before, we again allow these relationships to be weighted to reflect a difference in importance.
% However in the case of YAGO ... become 1... (we later in section XYZ then create KBs with non-integral weights)''}
% \aamod{03/29: Yes, we kept the type score so that later on we can use that space for storing non-integral scroes. I updated the text above accordingly.}
%between the entities. 
%Here, we append the KB entities having a relation to get a key.
%Then, the list of relationship between them is a value.

%\cref{fig:yago_indexes} shows the example entries of \textit{Type Dictionary}, \textit{Relationship Dictionary} and \textit{Inheritance Dictionary}. 
%\roee{Should we move all of next sentence into a footnote?:} 
%aamod: That would be a lots of footnote.
%\wolf{3/24: maybe combine them into one single footnote}
%rjm resolved - I've made this more conceptual and less implementation
%\wolf{10/19: wow, this past paragraph contains a lot of practical information on design decisions. Is there any way to quickly give a few illustrating examples together with reasons for individual decisions (e.g., examples that would otherwise not work, or that led to those decisions)}
%\aamod{10/22: I think this is a very general information for anyone familiar with the knowledge base use and the idea is similar to how people index the KB before using it. Shall we invest paperspace and create figures to illustrate it?}

% \roee{IMHO, these details should be given in a experimental setting section in the experiments and here we should state ``"}

%%rjm we are resolving this by removing example
%\rjm{how important is this discussion of homographs?  Do we have a clever solution for this?}
%rjm I don't think we've said this year
% Recall that 
\begin{figure}[h]
    \includegraphics[scale = 0.55]{110821_SIGMOD2022_Submission/figures/relationship_dict.pdf}
  \captionof{figure}{Relationship dictionary example}
\label{fig:relationship_dict}
\end{figure}
As we index only the necessary KB triples, the total space taken by these dictionaries in main memory is 3.75 GB and fit the modern computers.
Also, we need 965.18 MB to store them persistently\footnote{\label{footnote:memory_size} We report main memory space returned by sys.getsizeof() (\url{https://docs.python.org/3/library/sys.html}) and indexes are stored as compressed pickle files (\url{https://docs.python.org/2/library/pickle.html}).}.

%rjm:  I don't think we need this since we don't do anything super special with homographs
%In our setup, we consider them as  homographs.
%Homographs are the words having multiple meanings %\cite{21_leventidis_homograph_detection}.
%Precisely, we consider two entities to be homographs if they have same label or the alternate name in the knowledge base.
%\begin{example}
%\label{example:homographs}
%Let us consider \cref{tab:city_and_details} that illustrates the information about different places, their geographical coordinates, famous people born in those places and their occupation. "Boston" from \texttt{Place} attribute in \cref{tab:city_and_details} is the label for both Boston song and Boston city in the KB. Since it is the label for more than one entity and has multiple meanings, we consider it a homograph following Leventidis' definition \cite{21_leventidis_homograph_detection}. 
%\end{example}

% \aamod{10/19:With minor changes,} SANTOS can be used with any general or domain specific knowledge bases (KBs) like DBpedia \cite{auer_07_dbpedia}, Wikidata \cite{vrande_14_wikidata}, YAGO \cite{tanon_20_yago}  and so on.
% However, being captivated by the clean type hierarchy and logically reasonable and consistent semantic constraints, we selected YAGO 4 for running our experiments \cite{tanon_20_yago}.
% Hereafter, we will use YAGO interchangeably with YAGO 4. YAGO has different flavors according to the sources of the entities. 
% We used full YAGO having over 64 million entities and 10124 types (or classes).
% Each entity is mapped to at least one type. The types are taken from schema.org, bioschema.org and wikidata \cite{guha_16_schema.org, Gray_17_bioschema.org, vrande_14_wikidata}.
% They are arranged in a consistent type hierarchy with schema:Thing as a root.
% \wolf{10/19: ``type hierarchy'' here means relations as "IsA". Thus say ``living thing'' must be top type, correct? }
% Being a root of the hierarchy, schema:Thing does not have parent types and we call it Knowledge Base Root Type throughout this paper.
% Also, we use T to represent the set of all types in the KB and E to represent the set of all entities.

% \begin{definition}[Top Level Type]
% Any type $t \in T$ is said to be a top level type if it is directly connected to the Knowledge base root type.
% \end{definition}
% In our setup, schema:Thing is the Knowledge base root type and we have 2714 top level types. 
% We represent the set of all top level types using $T_{top}$.
% \wolf{10/19: suggestion: $T_{\mathrm{top}}$ or $T_{\mathit{top}}$}

% \aamod{08/18: I added the paragraph below about using YAGO just for our reference. I dont think we need such low level details in the paper.}
% For querying the KB efficiently, we preprocess YAGO 4 files and convert them into four key-value dictionaries.
% First, we use label dictionary that stores the labels and alternate names in YAGO 
% \wolf{10/19: if I understand correctly, that is important information here: the knowledge base also provides synonyms}
% as keys and the list of the KB entities related to those labels and alternate names as values.
% For unique identification, we represent KB entities using their Uniform Resource Identifiers (URIs) in YAGO.
% Second, we use a type dictionary which is similar to isA database used by \cite{venetis_11_recovering_semantics}.
% In this dictionary, the entities in the KB are keys and the list of their types are values.
% Note that each key in type dictionary must be a value in at least one tuple of label dictionary.
% Third, we use relation dictionary to store the relationship between the entities. Here, we append the KB entities having a relation to get a key.
% Then, the list of relationship between them is a value.
% This dictionary is similar to the relation database in \cite{venetis_11_recovering_semantics}.
% Finally, we create a class dictionary that stores each KB types as a key and the list of their children types as value.
% \wolf{10/19: wow, this past paragraph contains a lot of practical information on design decisions. Is there any way to quickly give a few illustrating examples together with reasons for individual decisions (e.g., examples that would otherwise not work, or that led to those decisions)}


% Recall that we connect tables with the KB by mapping the attribute values to the entity labels or the alternate names in the KB. 
% There can be multiple entities having same label or alternate name. 
% In our setup, we consider them as  homographs.
% Homographs are the words having multiple meanings \cite{21_leventidis_homograph_detection}.
% Precisely, we consider two entities to be homographs if they have same label or the alternate name in the knowledge base.
% \begin{example}
% \label{example:homographs}
% "Boston" from Place column in \cref{tab:city_and_details} is the label for both Boston song and Boston city in the KB. Since it is the label for more than one entity and has multiple meanings, we consider it a homograph following Leventidis' definition \cite{21_leventidis_homograph_detection}. 
% \end{example}

==> sections/algorithm.tex <==
\section{Algorithm---Move to Main Paper}

\begin{algorithm}[t]
\setstretch{0.85} % sets line height
\small
\SetAlgoLined
\LinesNumbered
\textbf{Input}: data-lake table $D$; knowledge base $\mathcal{K}$\\
\textbf{Output}: updates applied to synthesized relation dictionary $\mathcal{R}$
and inverted index $\mathcal{I}$\\
% \algocomment{--------------------}\;

\For{each column $c$ in $D$}{
    Look up all of $c$'s values in $\mathcal{K}$, tally how many times each top-level type appears in the result, and let $\type(c)$ be the top-level type with the highest count and $\score(c)$ its confidence score\;
    \algocomment{If $\mathcal{K}$ does not return any type for any value in $c$, then $\type(c) = \bot$, i.e., NULL}\;
}
\For{each column pair $(c, c')$ in $D$}{
    Look up all value pairs in $\mathcal{K}$, tally how many times each type appears in the result, and let $\type(c, c')$ be the type with the highest count and $\score(c, c')$ its confidence score\;
    \eIf{$\type(c, c') \neq \bot$}{
        Insert key $(\type(c), \type(c, c'), \type(c))$ with
        value $(D.\id, c.\id, c'.\id, \score(c), \score(c, c'), \score(c'))$
        into $\mathcal{I}$
    }{
        \If{$c \rightarrow c'$ is a candidate FD}{
            In $\mathcal{R}$, for each value pair $(v, v')$ in columns $(c, c')$, update the value for key $(v, v')$\;
            In $\mathcal{I}$, insert a new key $(\bot, (c.\id, c'.\id), \bot)$ whose value is a list containing tuple
            $(D.\id, c.\id, c'.\id, \bot, \score(c, c'), \bot)$ and analogous tuples for all tables and column pairs that share value pairs with $(c, c')$\;
        }
    }
}
\caption{SANTOS pre-processing algorithm.}
\label{alg:SANTOSpre}
\end{algorithm}


\aamod{Yes! This algorithm captures what we are doing in high level. We will change macros to make it consistent.}


\begin{algorithm}[tbp]
\setstretch{0.85} % sets line height
\small
\SetAlgoLined
\LinesNumbered
\textbf{Input}: query table $Q$ with subject column $Q.S$; knowledge base $\mathcal{K}$;
synthesized relation dictionary $\mathcal{R}$;
inverted index $\mathcal{I}$; constant $k$\\
\textbf{Output}: Top-$k$ SANTOS-unionable tables\\
% \algocomment{--------------------}\;

\algocomment{Determine the semantic tree $\mathcal{T}$ for $Q$, which is rooted at $Q.S$}\;
\For{each column $c$ in $Q$}{
    Look up all of $c$'s values in $\mathcal{K}$, tally how many times each top-level type appears in the result, and let $\type(c)$ be the top-level type with the highest count and $\score(c)$ its confidence score\;
    \algocomment{If $\mathcal{K}$ does not return any type for any value in $c$, then $\type(c) = \bot$, i.e., NULL}\;
}
\For{each column pair $(Q.S, c)$ in $Q$}{
    \algocomment{First search the knowledge base $\mathcal{K}$ for binary relations. If that fails, search the synthesized relation dictionary $\mathcal{R}$.}\;
    Look up all value pairs in $\mathcal{K}$, tally how many times each type appears in the result, and let $\type(Q.S, c)$ be the type with the highest count and $\score(Q.S, c)$ its confidence score\;
    \eIf{$\type(Q.S, c) \neq \bot$}{
        Insert key $(\type(Q.S), \type(Q.S, c), \type(c))$ with
        value $(Q.\id, Q.S.\id, c.\id, \score(Q.S), \score(Q.S, c), \score(c))$
        into $\mathcal{T}$\;
    }{
        Look up all value pairs in $\mathcal{R}$ and tally how many times each type appears to compute its confidence score\;
        \For{each type $\type(Q.S, c)$ found}{
            Insert key $(\bot, (Q.S.\id, c.\id), \bot)$ with value $(Q.\id, Q.S.\id, c.\id, \bot, \score(Q.S, c), \bot)$
            into $\mathcal{T}$\;
        }
    }
}

\algocomment{Using the inverted index $\mathcal{I}$, find all relevant tables, i.e., those whose semantic graph
contains an edge (i.e., type triple) of query-table semantic tree $\mathcal{T}$.}\;
\algocomment{$\Phi$ stores for each relevant data-lake table found the list of column pairs (i.e., graph edges)
whose type triples match an edge in $Q$'s semantic tree and their scores.}\;
\For{each pair of key $(\type(Q.S), \type(Q.S, c), \type(c))$ and value $(Q.\id, Q.S.\id, c.\id, \score(Q.S), \score(Q.S, c), \score(c))$ in $\mathcal{T}$}{
    Look up $(\type(Q.S), \type(Q.S, c), \type(c))$ in inverted index $\mathcal{I}$\;
    \For{each returned value $(D.\id, c.\id, c'.\id, \score(c), \score(c, c'), \score(c'))$}{
        Insert key $D.\id$ with value $(c.\id, c'.\id, \score(c), \score(c, c'), \score(c'))$ into $\Phi$
    }
}

\For{each table $D$ in $\Phi$}{
    \algocomment{$\Phi$ contains all of $D$'s column pairs that match the type of some pair formed by the subject column and another column in $Q$, as well as the corresponding type scores. This, together with the type scores for $Q$'s
    columns and column pairs is all the information needed to compute the table matching score.}
    Compute the matching score between $Q$ and $D$\;
}
Rank the tables by matching score and return the top-$k$\;
\caption{SANTOS query algorithm.}
\label{alg:SANTOSquery}
\end{algorithm}

==> sections/alt_KB_details.tex <==
\subsection{Knowledge Base}
\aamod{04/02: I don't think we still need this section in details.}
\label{section:knowledge_base}
%and understand the table semantics. 
% \wolf{3/23: Did you earlier describe what `table semantics' means? column types, and pairwise relationship semantics? 
% How does this problem related to the problem of ``table interpretation''? or is ``understanding the table semantics'' the same as ``table interpretation''?}
% \aamod{03/28: updated the sentence above. Rephrased and removed ``table semantics`` to avoid confusion.}
% For the purpose of this paper, a knowledge base is used to represent relationships between the concepts represented in each column explicitly.
%rjm this is resolved below
% \wolf{10/21: shortly describe the criteria of a knowledge base, relative to what it is used for. ``for the purpose of this paper, a knowledge base is an explicit representation between the concepts represented in each column'' (do we have an unambiuous name for that? In other words, one could use the column name to represent that concept from the knowledge base (if present)}
%  With minor changes, 
We now focus specifically on the existing KB that SANTOS uses to find these semantics.
SANTOS can be used with any general, enterprise-level and domain-specific knowledge base (KB), 
such as DBpedia \cite{auer_07_dbpedia}, Wikidata \cite{vrande_14_wikidata}, YAGO \cite{tanon_20_yago}, Freebase \cite{DBLP:conf/sigmod/BollackerEPST08} and so on.
% \grace{3/17: Either here or in the experiments section, say we can also use a KB for enterprise data, and use the same approach}
%aamod: updated in the experiment section
For now, due to its clean type hierarchy and semantic consistencies in their predicate types (e.g. constraints on the possible predicates that each subject can have), 
%logically reasonable 
%and consistent semantic constraints, 
% \wolf{3/23: will the readers know what a semantic constraint is?} \aamod{we assume that readers have some experience with the KBs and refer them to YAGO. This is YAGO's main argument against DBPedia and wikidata. Should we go into more details?}
% \wolf{3/24: yes, please repeat in short the argument. Actually there are two:
% 1. type hierarchy: that's what you seem to explicitly use later.
% 2. semantic constraint: I don't know what this is. Is it essential for your method? If yes, then you anyway have to define it and explain how the methods uses those ``semantic constraints''}
% \aamod{03/28: In DBPedia, since it is extracted automatically, it has some triples like: company -> birthplace -> city. However, company should have location but not the birthplace. This is handled by YAGO by defining semantic constraints manually.
% As Semantic constraints do not have a lot to do, we decided to use type hierarchy only as motivation.}
we use YAGO 4~\cite{tanon_20_yago} for our evaluations. Hereafter, we will use YAGO interchangeably with YAGO 4. 

YAGO contains the set of entities and types where, 
%over 64 million entities and 10,124 types (or classes). 
each entity is mapped to at least one type. 
The types are taken from \url{https://schema.org}~\cite{guha_16_schema.org},
%\wolf{3/23: these links don't work. What would work is \url{https://schema.org}}
\url{https://bioschema.org}~\cite{Gray_17_bioschema.org}
and \url{https://wikidata.org}~\cite{vrande_14_wikidata}
and arranged in a consistent type hierarchy with \texttt{schema:Thing} as its root. Thus, the \textit{Top Level Types} are direct descendants of this root type. 
% Let $T$ be a set of all types. Any type $t \in T$ is a  if it is directly connected to the knowledge base root type.
% \wolf{3/24: 
% Define T: `Let $T$ be the set of 10,124 types.'
% Alternatively, further up introduce the symbols: `... a set [symbol] of 64 millions entities and set $T$ of 10,124 types...'}
% \aamod{03/28: We decided to remove the numbers (like 10,124 2714 etc. and just mention the types.}
%rjm resolved
%\wolf{10/19: ``type hierarchy'' here means relations as 
%Thus say ``living thing'' must be top type, correct? } \aamod{10/22: Yes, however we don't have living things explicitly in the KB. Person is an example of top level type and president can be its subtype.} Being the root of the hierarchy, schema:Thing does not have parent types and we call it ``Knowledge Base Root Type" throughout this paper. We use $T$ and $E$ to denote the set of all types and entities in the KB, respectively.
%\begin{definition}[Top Level Type]
%Any type $t \in T$ is a top level type if it is directly connected to the knowledge base root type.
%\end{definition}
%In our setup, 
%schema:Thing is the knowledge base root type
%\wolf{3/23: repeated statement from before}
%and 
%we have 2,714 \textit{Top Level Types}. 
% \wolf{3/24: is it worth to add here a quick overview figure? Just so everyone is on the page: you'd show a top node,
% then below an example path via place, location, city (or so) and have number of hierarchy levels and a few key statistics. 
% You should definitely add that figure to your talk slides, because it helps show what is going on, and make sure everyone sees the "type hierarchy", but I would also add it to the online appendix, and optionally the paper if space permits. It's a simple figure that helps a first time reader enormously. And a figure that will be remembers after reading. 
% Researchers / reviewers read several papers per days, it's figures that help remember important concepts. And here the type hierarchy seems to be essential}
% \aamod{03/30: Yes, we have a slide showing the type hierarchy example (added to 2021\_SANTOS\_figures.pptx). However, due to space constraints, we did not add that to the paper.}
Using the KB, we maintain four dictionaries to capture the entities, their column semantics with associated hierarchies, and relationship semantics. For a given column, \textit{entity dictionary} first maps each column value to entities in the KB. Next,  \textit{inheritance dictionary} stores each Top level type and all their descendants. Then, we create a \textit{type dictionary} to find a set of types and associated confidence scores for each entity. Finally, we create a \textit{relationship dictionary} that stores the relationship semantic with a corresponding score.
%rjm resolved
% \wolf{10/19: suggestion: $T_{\mathrm{top}}$ or $T_{\mathit{top}}$}
% \roee{consider moving the technical part into an experimental settings section within the experiments section.} 




\introparagraph{1. Entity Dictionary} 
YAGO contains a set of KB entities each with a set of labels and alternate names (like synonyms) that describe the corresponding entity \footnote{\label{footnote:rdf_labels} \url{https://www.w3.org/2004/12/q/doc/rdf-labels.html}}. 
% \wolf{3/23: what is the meaning of those labels?}
% \aamod{3/23: They are standard KB labels and alternate names}
% \wolf{3/24: what are `standard' labels? I don't hink there is a standard for the word standard. It's unspecific. 
% Are labels synonyms, isA relationships, types? I would not know how to restrict the endless possibilities to define labels to those tha are standard}
% \aamod{03/28: added a footnote with a link to rdf query language.}
We store these 
%(and the entity Uniform Resource Identifiers or URIs) 
in a key-value dictionary that we call the {\em entity dictionary}.
The key is any label or alternate name and the value is the entity Uniform Resource Identifiers or URIs.\footnote{\label{footnote:labels_alternate_names}We only index labels and alternate names in English Language.
\wolf{3/23: how many of the originally 64 mio are left?}
\aamod{03/23: we keep all entities. Only alternate names are omitted. Each entity can have numerous alternate names.}
}
We connect tables with the KB by mapping the column values to the entity labels or the alternate names in the KB.
Note that YAGO permits  multiple entities to have the same label or alternate name. 
Hence, one value may be mapped to different entities with different types (that is, the value is a homograph with multiple meanings~\cite{21_leventidis_homograph_detection}).
%rjm:  this belongs in experiments
%For completeness, we now describe some more technical details on how we use YAGO in this paper. For querying the KB efficiently, we preprocess YAGO 4 files and convert them into four key-value dictionaries. First, we use label dictionary that stores the labels and alternate names in YAGO as keys and the list of the KB entities related to those labels and alternate names as values.
%For unique identification, we represent KB entities using their Uniform Resource Identifiers (URIs) in YAGO.


% \wolf{3/24: want to also add here a quick example. e.g. the william\_shakespear from fig 4: there this key gets mapped to several synonyms. If W.S. has 9 alternatives, does this dictionary have 10 entries for W.S.?}
% \aamod{03/29: If W.S has 9 alternatives, these 9 alternatives are keys in the dictionary and for all of them, the value is yago:William\_Shakespeare.
% For example, william shakespeare has one label: ``William Shakespeare`` and 1 alternate name: ``Shakespeare``. so, ``William Shakespeare`` and ``Shakespeare`` are keys and yago:William\_Shakespeare is a value for both of them. Should we add a table like other cases for this too?  
% }
\begin{figure}[h]
    \includegraphics[scale = 0.55]{figures/entity_dict.pdf}
\captionof{figure}{Entity dictionary example \aamod{03/31: ``W`` and ``S`` in URIs should be in small letters (w and s)}}\grace{3/31: YAGO has it as upper-cased: \url{https://yago-knowledge.org/graph/yago:William_Shakespeare}}
\aamod{04/01: These are the dictionaries we create after pre-processing YAGO. Therefore, all of them are lower-cased although they are not all lower in YAGO.}
\label{fig:entity_dict}
\end{figure}

\introparagraph{2. Inheritance Dictionary} 
Next, we build 
%a {\em class dictionary} 
an {\em inheritance dictionary} that stores each Top level type as a key and the set of their children types as value. 
\wolf{3/23: @Mirek: is this the ``right'' definition: A key mapping to a set of values?
The values are then not atomic and can't be queried. Would it make more sense to have the 
children map to their unique parent? Thus way both the set of keys, and the set of values are atomic.}
An inheritance dictionary example 
%inline with our running example, 
is shown in \cref{fig:inheritance_dict}.
%For instance, {\em inheritance dictionary} has a top level type \texttt{place} as key having the set of its children \{administrative\_area, city, country, $\dots$\} as value.

% \begin{figure}[h]
%     \includegraphics[scale = 0.45]{110821_POST_VLDB_Submission/figures/yago_indexes.png}
%   \captionof{figure}{Example of the dictionaries built using YAGO.}
% \label{fig:yago_indexes}
% \end{figure}
\begin{figure}[h]
    \includegraphics[scale = 0.55]{figures/inheritance_dict.pdf}
\captionof{figure}{Inheritance dictionary example
% \wolf{3/24: Oh, I thought it was not just the `top level types' and wanted to point out the confusion. Like city could also be the key for some value like town? Or a chain artist-musician-piano player. Musician can also be in the left column, right?}
% \aamod{03/29: We only consider top level types as the keys. So, there are 2714 keys in this dictionary. The intuition is that: each column can be of 1 among 2714 top level types. Once we select the top level type for a column, we annotate it with that type and also its children types with difference confidence scores.}
}
\label{fig:inheritance_dict}
\end{figure}



\introparagraph{3. Type Dictionary} 
We use Type dictionary to lookup entities and find their types.
% \wolf{3/24:
% You also need to explain why you care about keeping the level in the hierarchy around: is it used later?}
% \zixuan{3/28: We're trying to use it in the experiments now so I keep the levels here for now.}
% \wolf{3/24:
% ``
% Basic information theory, if a biased coin comes up 90\% head and 10\% tail, then every tail drop is more surprising and thus more informative [cite some intro to information theory book]. 
% In the same way, for us,
% a concept or type declaration that appears more frequently is less informative. 
% For example,  there are over 6M {places} in YAGO among which only 42k are {cities}.
% Thus the type declaration Boston isA city is more informative than Boston isA place.
% Inspired by tfid ... and with the log ...
% we consider city to be about 30\% more informative (0.2115 / 0.1633) than place. 
% [That is surprising that something that 100 times rares, gets only a 30\% boost: can you add some intuitive discussion why that ratio is good? Have you tried with different log bases, e.g. 100 times rares gives a 100\% boost, etc.?] ''}
% \zixuan{3/28: Paragraph updated. There is a trade-off here. We can't penalize the top type too much. Or there will be such case: The table is about places, containing 60\% cities and 40\% provinces. If we boost city too much like 100\%, this table is considered a table about cities.}

After getting the type scores, we build a {\em type dictionary} based on YAGO.
%which is similar to the (proprietary) isA database used to recover semantics of webtables~\cite{venetis_11_recovering_semantics}. 
Note that each key in the {\em type dictionary} must be a value 
%in at least one tuple of label 
in the  {\em entity dictionary}.
% \wolf{3/23: I am confused: do you recreate / or do you create something from YAGO? But you can't `create' something that is part of YAGO because others did YAGO}
% \zixuan{3/28: Updated}
% \wolf{3/24: That other isA database also has weights like here or is just an isA graph? 
% Also, your type dictionary is actually a weighted type dictionary? Or more a type distribution? Because in a ``dictionary'' you normally look up one thing, here it is actually a distribution. That is not immediately intuitive.}
% \zixuan{3/28: It is still a dictionary. You look up for one entity in the dictionary, and it returns the type with type score and type level of that entity.}
If we look for an entity in this dictionary, the returned result is this entity and the set of tuples of its (type, type score, type level), where the type score of any type t, $ts(t) \in (0, 1]$, as defined in \cref{subsection:type_hierarchy}, and \textit{type level} refers to its level in the type hierarchy i.e. the shortest path from the root.
For example, the entity \textit{boston}\footnote{\label{footnote:preprocessings}We convert all texts to lowercase and perform preprocessings like stemming and punctuation removal.} is a key in {\em type dictionary} as shown in \cref{fig:type_dict}. \textit{boston} is mapped to values $place$, which is a top level type so it has \textit{type level} = 1, and $city$, which is a descendant of $place$ and thus has \textit{type level} = 3.
% \wolf{3/24: interesting that here the word is not capitalized. Fig 1 shows capitalized words, later examples not. best to add somewhere a quick explanation with your convention}
%as shown in \cref{fig:yago_indexes}.

% \wolf{3/23: At this point I am left confused about the score. So it is not just a `dictionary' but a `type distribution'?
% What is the intuition of the distribution = ts? Is it a weight that is created not from YAGO itself, but from the data in the data lake?
% Thus may vary for different applications? 
% Because you explain the calculation in detail, what is the intuition of the calculations?}
% \zixuan{3/28: No. It is based on YAGO itself. Indeed we tried some strategies like TF-IDF to get some score based on the tables but after discussions in our meetings, we gave it up.}

\begin{figure}[h]
    \includegraphics[scale = 0.55]{figures/type_dict.pdf}
  \captionof{figure}{Type dictionary example}
\label{fig:type_dict}
\end{figure}

\introparagraph{4. Relationship Dictionary} 
Finally, we build a {\em relationship dictionary} to store the relationships (properties) from YAGO. As shown in \cref{fig:relationship_dict}, the keys are pairs of entities and each value is a set of tuples of (YAGO properties/binary relationships, type score). This dictionary is similar to the (proprietary) relation database used to recover semantics of webtables~\cite{venetis_11_recovering_semantics}.
As before, we again allow these relationships to be weighted to reflect a difference in importance. However in case of YAGO properties, we do not have hierarchy like YAGO types and hence, the type score is 1. Later in \cref{section:synthetic_knowledge_base}, we create synthesized KB and add entity pairs with non-integral type scores.
% \wolf{3/24: 1. So this dictionary just reflects the existing information in YAGO, right? In constrast to the type dictionary where you invent new value like distributions and hierarchy level?
% 2. `therefore the confidence score is 1': this sentence implies that you interpret the other log transformed frequency in the type dictionary as some confidence, but that is not really justified. Also I don't see why the `therefore' is justified here.
% 3. you likely keep the weights 1 here because you later in the synthetic KB you allow those values to be non integral. Thus motivate this here. Something like
% ``as before, we again allow these relationships to be weighted to reflect a difference in importance.
% However in the case of YAGO ... become 1... (we later in section XYZ then create KBs with non-integral weights)''}
% \aamod{03/29: Yes, we kept the type score so that later on we can use that space for storing non-integral scroes. I updated the text above accordingly.}
%between the entities. 
%Here, we append the KB entities having a relation to get a key.
%Then, the list of relationship between them is a value.

%\cref{fig:yago_indexes} shows the example entries of \textit{Type Dictionary}, \textit{Relationship Dictionary} and \textit{Inheritance Dictionary}. 
%\roee{Should we move all of next sentence into a footnote?:} 
%aamod: That would be a lots of footnote.
%\wolf{3/24: maybe combine them into one single footnote}
%rjm resolved - I've made this more conceptual and less implementation
%\wolf{10/19: wow, this past paragraph contains a lot of practical information on design decisions. Is there any way to quickly give a few illustrating examples together with reasons for individual decisions (e.g., examples that would otherwise not work, or that led to those decisions)}
%\aamod{10/22: I think this is a very general information for anyone familiar with the knowledge base use and the idea is similar to how people index the KB before using it. Shall we invest paperspace and create figures to illustrate it?}

% \roee{IMHO, these details should be given in a experimental setting section in the experiments and here we should state ``"}

%%rjm we are resolving this by removing example
%\rjm{how important is this discussion of homographs?  Do we have a clever solution for this?}
%rjm I don't think we've said this year
% Recall that 
\begin{figure}[h]
    \includegraphics[scale = 0.55]{figures/relationship_dict.pdf}
  \captionof{figure}{Relationship dictionary example}
\label{fig:relationship_dict}
\end{figure}
As we index only the necessary KB triples, the total space taken by these dictionaries in main memory is 3.75 GB and fit the modern computers.
Also, we need 965.18 MB to store them persistently\footnote{\label{footnote:memory_size} We report main memory space returned by sys.getsizeof() (\url{https://docs.python.org/3/library/sys.html}) and indexes are stored as compressed pickle files (\url{https://docs.python.org/2/library/pickle.html}).}.

%rjm:  I don't think we need this since we don't do anything super special with homographs
%In our setup, we consider them as  homographs.
%Homographs are the words having multiple meanings %\cite{21_leventidis_homograph_detection}.
%Precisely, we consider two entities to be homographs if they have same label or the alternate name in the knowledge base.
%\begin{example}
%\label{example:homographs}
%Let us consider \cref{tab:city_and_details} that illustrates the information about different places, their geographical coordinates, famous people born in those places and their occupation. "Boston" from \texttt{Place} attribute in \cref{tab:city_and_details} is the label for both Boston song and Boston city in the KB. Since it is the label for more than one entity and has multiple meanings, we consider it a homograph following Leventidis' definition \cite{21_leventidis_homograph_detection}. 
%\end{example}

% \aamod{10/19:With minor changes,} SANTOS can be used with any general or domain specific knowledge bases (KBs) like DBpedia \cite{auer_07_dbpedia}, Wikidata \cite{vrande_14_wikidata}, YAGO \cite{tanon_20_yago}  and so on.
% However, being captivated by the clean type hierarchy and logically reasonable and consistent semantic constraints, we selected YAGO 4 for running our experiments \cite{tanon_20_yago}.
% Hereafter, we will use YAGO interchangeably with YAGO 4. YAGO has different flavors according to the sources of the entities. 
% We used full YAGO having over 64 million entities and 10124 types (or classes).
% Each entity is mapped to at least one type. The types are taken from schema.org, bioschema.org and wikidata \cite{guha_16_schema.org, Gray_17_bioschema.org, vrande_14_wikidata}.
% They are arranged in a consistent type hierarchy with schema:Thing as a root.
% \wolf{10/19: ``type hierarchy'' here means relations as "IsA". Thus say ``living thing'' must be top type, correct? }
% Being a root of the hierarchy, schema:Thing does not have parent types and we call it Knowledge Base Root Type throughout this paper.
% Also, we use T to represent the set of all types in the KB and E to represent the set of all entities.

% \begin{definition}[Top Level Type]
% Any type $t \in T$ is said to be a top level type if it is directly connected to the Knowledge base root type.
% \end{definition}
% In our setup, schema:Thing is the Knowledge base root type and we have 2714 top level types. 
% We represent the set of all top level types using $T_{top}$.
% \wolf{10/19: suggestion: $T_{\mathrm{top}}$ or $T_{\mathit{top}}$}

% \aamod{08/18: I added the paragraph below about using YAGO just for our reference. I dont think we need such low level details in the paper.}
% For querying the KB efficiently, we preprocess YAGO 4 files and convert them into four key-value dictionaries.
% First, we use label dictionary that stores the labels and alternate names in YAGO 
% \wolf{10/19: if I understand correctly, that is important information here: the knowledge base also provides synonyms}
% as keys and the list of the KB entities related to those labels and alternate names as values.
% For unique identification, we represent KB entities using their Uniform Resource Identifiers (URIs) in YAGO.
% Second, we use a type dictionary which is similar to isA database used by \cite{venetis_11_recovering_semantics}.
% In this dictionary, the entities in the KB are keys and the list of their types are values.
% Note that each key in type dictionary must be a value in at least one tuple of label dictionary.
% Third, we use relation dictionary to store the relationship between the entities. Here, we append the KB entities having a relation to get a key.
% Then, the list of relationship between them is a value.
% This dictionary is similar to the relation database in \cite{venetis_11_recovering_semantics}.
% Finally, we create a class dictionary that stores each KB types as a key and the list of their children types as value.
% \wolf{10/19: wow, this past paragraph contains a lot of practical information on design decisions. Is there any way to quickly give a few illustrating examples together with reasons for individual decisions (e.g., examples that would otherwise not work, or that led to those decisions)}


% Recall that we connect tables with the KB by mapping the attribute values to the entity labels or the alternate names in the KB. 
% There can be multiple entities having same label or alternate name. 
% In our setup, we consider them as  homographs.
% Homographs are the words having multiple meanings \cite{21_leventidis_homograph_detection}.
% Precisely, we consider two entities to be homographs if they have same label or the alternate name in the knowledge base.
% \begin{example}
% \label{example:homographs}
% "Boston" from Place column in \cref{tab:city_and_details} is the label for both Boston song and Boston city in the KB. Since it is the label for more than one entity and has multiple meanings, we consider it a homograph following Leventidis' definition \cite{21_leventidis_homograph_detection}. 
% \end{example}

==> sections/alt_unionability_components.tex <==
\section{Creating Semantic Graph}
\label{section:unionability_components}
We now introduce two methods that
SANTOS uses to create semantic graphs. %relationships. 
\rjm{The first uses a KB and is described in this section.  The second (\cref{section:synthetic_knowledge_base}): is designed to be used when there is either no reliable KB covering the data lake or a KB with only partial coverage (a very common case in enterprise and open data lakes). We present experiments (\cref{section:experiments})  using each method independently, but also using the methods in concert  to provide better accuracy.}
%rjm SANTOS mainly uses a Knowledge Base (KB) to create semantic graphs over the tables and annotate their columns and relationships.
%rjm First, we describe how we can use any KB to annotate the nodes of the semantic graph 
%rjm with a (set of) semantic types from the KB and
%rjm the edges of the semantic graph with properties from the KB.  
%rjm We continue to explain how we use an existing knowledge base (KB) \cite{21_hogan_knoweledge_graph_survery} to do so in this section.Then later in \cref{section:synthetic_knowledge_base}, we introduce a {\em synthesized knowledge base}.

\subsection{Column Semantics}
\label{section:column_semantics}
% \begin{figure}[t]
%     \includegraphics[scale = 0.55]{figures/sem_illustration.pdf}
%   \captionof{figure}{Column Semantics (CS) and relationship semantics (RS) in a given table
%   \wolf{3/23: best to draw the RS as directed edges, it's an ordered relationship S-P-O}}
% \label{fig:sem_illustration}
% \end{figure}

%Column semantics is one of the important unionability features in SANTOS.
%It is the list of knowledge base types that represent the semantics of the data values in a column.
%rjm For determining table unionability,
%inferring the semantics of a table, 
%rjm we must understand the semantics of its columns.
To create column semantics, we seek to associate a set of KB types to each column.
% ~(\cref{fig:sem_illustration}).
%label each text column of table using the KB types as shown in \cref{fig:cs_and_rs}. 
Associating columns with types from a KB is a 
%Labeling a table column is 
well-studied problem~\cite{venetis_11_recovering_semantics,ritze_15_matching_tables_to_dbpedia,zhang_17_tableminer+,hulsebos_19_sherlock,zhang_20_sato}.
%Column semantics are the nodes in the semantic graph.
%rjm right, fixed
%\wolf{10/21: aren't the columns the nodes, but their semantics the interpretation of the relationshipships (may depend on whether you like to formalize in terms of S-P-O triple, or just S-P pairs}
Like previous work on unionability~\cite{nargesian_18_TUS} and column semantic type detection~\cite{zhang_20_sato,2020_ota_d4, suhara_2021_doduo}, we are only using values within a column to determine the associated KB types.
%rjm resolved
%\renee{Careful, doesn't sherlock use metadata features?  Am I wrong?}
%\aamod{04/03: corrected! removed SHERLOCK, added SATO and DODUO.}
However, unlike other approaches, we make use of both the KB types and the KB type hierarchy to define the column semantics.
%, which we explain later.
%Intuitively, we want to assign a type distribution to each column based on the aggregate of the types of individual values in the column. This is based on three objectives: 

\renee{The following is sub-optimal as I could only think of a procedural way to describe this.  Feel free to change to a declarative definition.  }

\rjm{
To begin, we define a set of top level types that are the potential roots of the type tree in a column's column semantics.  These top level types will depend on the KB.  We will use YAGO 4~\cite{tanon_20_yago} which has a single root \texttt{schema:Thing}.   As this generic type is uninformative to use as part of a columns semantics and as YAGO has a large and rich set of types that are direct descendants of the root, we choose to use all direct descendants of this root as the top level types denoted by $T_{top}$.  These are the types that can be the root of a column's semantics.}\footnote{In a different KB, a different choice may be made to select an informative and distinct set of top level types.}

\rjm{
To define the column semantics of $c$, we map each value in $c$ to the KB.   If the value appears in the KB in a type $t$, we add $t$ and all its ancestors up to a top level type to a set $CS_{candidate}(c)$.  Note that a single value may map to multiple types (for example, using YAGO, \texttt{Boston} maps to both \texttt{City} and 
}
\ak{
\texttt{Music Album}
}
%aamod: updated to music album to ensure that we have creative work and place as the top level types. For boston as a band, the top-level type is organization. Should we change it to (well-known) band rather than creative work to make it more intuitive?
\rjm{)
, and certainly different values may map to different types.  After going through all values, if $CS_{candidate}(c)$ contains more than one top level type, then we keep only the top level type (and all its descendants in $CS_{candidate}(c)$) with the most entities that map to it.\footnote{In the rare case of ties, we keep the top level type that has the 
%most 
least
entities in the KB preferring the rarer type.%rjm modified to "least" as per aamod's comment}  This creates $CS(c)$ which is either empty (if no values appear in the KB) or contains a single top level type with a subset of its descendents to which at least one value in $c$ has been mapped. 
} 
\grace{4/4: Do we need a justification for why we only select one top-level type?}
}
\renee{4/4:  Yes we do, if you don't think the discussion in Sec 3 on why we restrict the CS to be a tree of types (aka one top-level type), then try to add more intuition there.  Maybe move semantic consistency discussion there?}
%rjm resolved
%\renee{I don't think it is acceptable to say ties never occur.  We need a rule to break them.  You can pick a different way if you like.}
%\aamod{I agree. I would prefer to select the type that is rare (having the least entities in the KB) because we have story about rare types prioritization later.}

\renee{I didn't find a lot of benefit in these principles.  Could you reduce and say something like ``this method'' has the benefits of producing column semantics that are semantically consistent (meaning X).}

(i) \introparagraph{Semantic consistency} Due to the low coverage of entities in any existing KB , as well as the heterogeneity of the data, annotating column values with only a set of types of the same granularity leads to sparsity. 
%\aamod{04/01: Should we make this statement? If we say low coverage of entities is the reason to form hierarchy, then there might be a question that doesn't using granular types need even more coverage?} 
%\grace{4/1: I was trying to give a motivation for why we're not just considering one granularity of types. Right, if we use only granular types, we would need more coverage. That's why we're considering broader types too}
Thus, we also want to include each type's ancestor types. For instance, for an entity \texttt{boston}, it would naturally have the type \texttt{city}. We would also want to include the broader type \texttt{place}, in which \{\texttt{city}\} $\subseteq$ \texttt{place}.
However, when we assign multiple types to a column, we want to ensure that the assigned types are semantically consistent. For example, if a column is assigned a type \textit{place}, it can also be assigned another granular type \textit{city} but not \textit{music album}, which is semantically inconsistent.
To maintain the semantic consistency--assuming that the top level types in the KB are semantically disjoint--
% we annotate column values with KB types, along with its corresponding type hierarchy. We also have disjoint hierarchies (e.g. one type's hierarchy has $T_{\mathit{top}}$ = place, another has $T_{\mathit{top}}$ = Person). This introduces a lot of noise in the annotations, especially in heterogeneous data with homographs \cite{21_leventidis_homograph_detection}.
we assign one top level type and only its descendants for a given column $c$. To do so, we use an unweighted
voting strategy and select only one top-level type that has maximum count among all top level types of the column. %\footnote{\label{footnote:no_ties} In our experiments, we never encountered "ties" on real data.}. 
Formally, we call this type \em{Top Level Column Semantics}.
%Specifically, we want to trace each entity type's ancestors back to its \textit{Top Level Type}.
%$\in T_{\mathit{top}}$, where $T_{\mathit{top}}$ is all direct descendants of a given KB's root type.
%We next define the semantics of the top level types connecting to types of the data values.
%i.e., 

% \begin{definition}[Top-Level Column Semantics]
% Let $T$ be the set of all types in the KB. 
% Let $T_c \subseteq T$ be the set of types for any column c such that $t \in T_c$ is the type of at least one column data value $v \in c$.
% % \wolf{3/24: Let me clarify: if the value is Boston, then will this value be assigned both place and city, or just city, based on the dictionary? Assume the transitive closure up the hierarchy is *not* encoded in the dictionary (it would be a waste).
% % But do you then still do find the top one? Thus $t$ is the set of top level hierarchies mapped to by some value? How do you exactly calculat the weight?}
% % \aamod{03/29: We get boston's type as place, city, state\_capital, creative\_work, movie, etc. However, we only keep the semantics that belongs to the top level type place i.e., this column will be annotate with place, city, state, etc. but not with createive work and movie. We first explained the top-level semantics assignment. Then we talk about how we assign the children types.}
% Now, among all $t \in (T_c \cap T_{\mathit{top}})$, $t$ is said to be the Top-level Column Semantics (TL$_{CS}$) for $c$ 
% if it is the top level type for the highest number of unique values in $c$.
% For a column c, there can be at most one TL$_{CS}$ and it is represented by TL$_{CS}$(c).
% \end{definition}

% Once TL$_{CS}$ is determined, we solely focus on TL$_{CS}$ and its descendants which ensures semantic consistency. The column semantics for a given column $c$ is thus TL$_{CS}$(c) and its descendants in the type hierarchy that are mapped to c. Note that $CS(c)$ may be empty for some columns.

\begin{example}
\label{example:top_type_explanation }
Let us consider, the \texttt{Birthplace} column in Table (c) of \cref{fig:running_examples} having five unique values.
%\cref{tab:city_and_details}.
In type hierarchy, \texttt{place} and \texttt{creative work} are among the top level types. The value \texttt{boston} is associated with both types. Hence, the KB returns both types for {\tt Birthplace} column. Also, the KB returns descendants of \texttt{place} \rjm{to which at least one value is mapped}: \emph{\{administrative area, city, country, sovereign state, emirate\}} and the descendant of \texttt{creative work} \rjm{to which at least one value is mapped}: \ak{\emph{\{music album\}}} for this column.
\renee{Why movie?  Boston is a band.}
\aamod{updated, used music album so that the top level type is still creative work. \url{https://en.wikipedia.org/wiki/Boston_(album)}. Should we use "more popular" band and update top level types in the examples to organization?}
%rjm resolved by correcting text above
%\renee{You include ALL descendants like emirate (and even subtypes of emirate) even if there is no value that maps to emirate?  If so correct the prose above and justify this choice.}
%\aamod{No, we only include those descendants which map to at least one value. Here, Qatar maps to emirates, that's why it is included in the column semantics.}
%will have both KB types associated with it.  
Notice the majority of the values are only associated with the place type, hence, we will select this as the TL$_{CS}$ for the {\tt Birthplace} column.  Hence, we discard "creative work" and its descendants.
The column semantics for the column \texttt{Birthplace} are the set of types:
\emph{\{place, administrative area, city, country, sovereign state, emirate\}}.  %The top-level type is {\em place} and all other types are specializations (children) of {\em place}.

% \wolf{3/24: make his a full example:
% 1. we have 5 different values (I assume you ignore duplicates, please mention).
% 2. one of them (Boston) maps to two: place and cw. All the other ones mape to place. Thus we get votes:
% place 4.5, cw: 0.5 (you giving each value the same number of total votes, right?).
% 3. thus the algorithm determines place as the top level.

% Question: why do you only focus on the top level type, not the more fine-grained ones? You likely would not want to union towns with countries. Alice born in Boston, Bob born in Canada. Leads to union countries with cities.}
%ak: resolved by adding full example
\end{example}

%Given TL$_{CS}$, we can define Column Semantics as follows: 

% \begin{definition}[Column Semantics]
% For a column $c$, its column semantics is a distribution over the hierarchy of types $t_0, t_1, \dots t_t$ s.t. $t_t \in$ TL$_{CS}$. We represent column semantics for 
% column $c$ using $CS(c)$. 
% \wolf{3/24: I am confused: is the focus only on top hierarchies, or any hierarchy? 
% I think the explanation so far allows both interpretations}
% \end{definition}

% \begin{example}
% %rjm In \cref{tab:city_and_details}, 
% In~\cref{fig:running_examples} (c), the column semantics for the column \texttt{Birthplace} are the set of types:
% \emph{\{place, administrative area, city, country, sovereign state, emirate\}}.  The top-level type is {\em place} and all other types are specializations (children) of {\em place}.
% \end{example}

\subsection{Column Semantics Confidence}
\label{sec:csconfidence}

\rjm{
For each type in $CS(c)$ we need to assign a confidence score.}


(ii) \introparagraph{Monotone in input weight} If a type gets assigned to more values in the column, it should obviously be prioritized over a type assigned to less values.
To model this, we assign a \em{frequency score} to each type in the column semantics.
\begin{definition}[Frequency Score]
Let $CS(c)$ be the column semantics of $c$.
The frequency score of type $t \in CS(c)$ ($fs(t)$)
is the ratio of the number of unique data values associated to type $t$ 
to the number of unique data values in this column that are mapped to the knowledge base.
\end{definition}

\begin{example}
\label{example:confidence_explanation }
Let us return to the {\tt Birthplace} column in~\cref{fig:running_examples}(c).
The column semantics includes both city and country.  
% \wolf{3/24: I am confused: didn't Example 5 also include creative work?} \aamod{03/29: No, it was discarded. We only select 1 top level type for each column. Then, the children of only the selected top level types will be assigned to the column with different confidence scores.}
These are siblings in the KB and both children of type {\em place}. Notice however, that only one unique data value out of 5 is associated with country while three are associated with city (Barnet is mapped to neither city nor country). To model this difference, we assign a frequency score to each type i.e., fs(\texttt{country}) = 0.2 and fs(\texttt{city} = 0.6). Also, fs(\texttt{place}) = 1.0.
\end{example}
\introparagraph{(iii) Prioritize Rare Types}\label{subsection:type_hierarchy}
%The rare types in the knowledge base are more informative and hence, should be prioritized over the frequent types (see \cref{section:knowledge_base}).
As a set of entities belonging to a descendant type is always a subset of entities belonging to its ancestor types in the knowledge base hierarchy,
the higher level types always have larger number of entities than children types and hence, receive unfair bias against the children types. 
In other words, for a pair of ancestor-descendant types, the ancestor type always appear more frequently, hence resulting in the bias towards it.
From the perspective of the information theory, the less probable outcome has greater information \cite{mackay2003information}.
In our case, a type that appears more frequently is less informative.
Inspired by the well-known tf–idf measure~\cite{aizawa2003information}, we penalize the frequent ancestor types by using a frequency-based strategy utilizing knowledge base statistics and assign a \textit{type score (ts)} to each type.
The basic idea is to count the frequency of each type t by counting the entities that belong to t in the KB and penalize the frequent types.
The type score is computed based on the following formula \cref{eq:type_score}. 
A logarithm function is used here because we do not want excessive penalization that may make our algorithm ignore the case that the column is indeed of a top level type. 
%Also, to make the type score in $(0, 1]$, 
We ignore the types having less than 10 entities.
%don't penalize rare types whose appearance count is no more than 10.
\begin{equation}\label{eq:type_score}
    %ts(t) = \frac{1}{\log (max(t.count, 10))}
    ts(t) = \frac{1}{\log(t.count)}
\end{equation}

%In this way, we prioritize granular types and penalize frequent and general types.
\begin{example}
Consider the entity \texttt{boston}, which belongs to the types \texttt{city} and \texttt{place}.
In the KB we use(specifically YAGO4), over 6 million entities have type \texttt{place}, and $\sim$42,000 entities have type \texttt{city}. 
Then, city is a more informative type than place that is one of its ancestor types.
Hence, the type scores are $ts(\texttt{place}) = 0.1475$ and $ts(\texttt{city}) = 0.2163$.
% Their type scores are respectively $ts(\texttt{place}) = 0.1633$ and $ts(\texttt{city}) = 0.2115$.
\end{example}
%By retrieving $CS(c)$, which contains types along possibly different type hierarchies \aamod{04/01: What are additional disjoint types here?} \grace{4/1: Types that do not appear in this hierarchy path at all, and are completely disjoint. Updated}, we must weigh each semantics according to their confidence.  
Finally, we aggregate each type's \em{type score} and \em{frequency score} to get its column semantics confidence score which ranges from 0 to 1.
%to each type in the column semantics by using \textit{type score} and using the type statistics returned by KB.
% \wolf{3/24: here I am completely confused: the details here contradict everything what was said before:
% 1. is the focus on just top or not?
% 2. why 4 values and not 5? where is creative work?}
% \aamod{03/29: There are 5 values. We have one value (Barnet) that is neither country nor city. It is only mapped up to administrative area.}
% We name this score Column Semantics Confidence Score, CS$_{\textsc{Conf}}$, and it ranges from 0 to 1.
% \wolf{3/24: why not column type score? To be consistent with type detection. 
% Conceptually, it is still a type detection, yet with a more careful intermediate aggregation step, and as output a weighted type.}
%We start by assigning CS$_{\textsc{Conf}}$ to TL$_{CS}$, which is the ratio of the total number of 
%unique column values mapped to TL$_{CS}$ to the total number of unique column values mapped to the knowledge base multiplied by its \textit{type score}.
% \wolf{3/24: I can't follow that description of the particular algorithm in text, without first a high-level description of where the journey goes.}
%Next, for each children type, we get CS$_{\textsc{Conf}}$ by dividing its count by the total number of unique column values mapped to the knowledge base and multiplying it by the respective \textit{type score}.
%Here, count refers to the number of unique column values each type is mapped to.
\begin{definition}[Column Semantics Confidence Score]
Let $CS(c)$ be the column semantics of $c$.
For a type $t \in CS(c)$, 
the column semantics confidence score  (CS$_{\textsc{Conf}}$) of
%a column semantics s of a column c 
$t$ is the product of fs(t) and ts(t).
%\aamod{03/31: We cannot use ts(t) here if we move Knowledge base section to 4.3. Same with the example below.}
We represent CS$_{\textsc{Conf}}$ for a type $t$ of column $c$ using CS$_{\textsc{Conf}}$($c,t$).
\end{definition}
\begin{example}
\label{example:column_semantics}
In Table (c) of \cref{fig:running_examples}, the column semantics with their confidence score for all columns are:
[{\tt Person}: \{ person: 1.0 * 0.1605, human: 1.0 * 0.1605 \},
{\tt Occupation}: \{ occupation: 1.0 * 0.2728, profession: 1.0 * 0.3118 \},
{\tt Birthplace}: \emph{ \{ place:
1.0 * 0.1475, administrative\_area: 1.0 * 0.1720, city: 0.6 * 0.2163, country: 0.2 * 0.2712, sovereign\_state: 0.2 * 0.434, emirate: 0.2 * 0.5 \}
}].
Recall that we do not compute the column semantics for numerical columns like {\tt Geo}. 
\end{example}
%The assignment of CS$_{\textsc{Conf}}$ to each type fulfills our second and third objectives.

% \wolf{3/24: I see, so you use ``semantics'' as synonym for ``type distribution''? 
% I'd still suggest to be clear: your idea is to deviate from prio work that determines a mapping froma column to a type (type detection), the goal of this approach is to determine a type distribution. What is a good name (other than semantics):
% probabilistic type detection (only if the weights have a clear probabilistic interpretation),
% weighted type detection,
% type distribution detection,
% type distribution assignment,
% assigning each column a type distribution
% }
% \aamod{03/30: Yes, if we say column type detection only, it sounds like we are annotating each column with 1 type with full confidence. However, this is not the case. Therefore, we want to name it differently.}

% In summary, we annotate column values with KB types, along with its corresponding type hierarchy. We also have disjoint hierarchies (e.g. one type's hierarchy has $T_{\mathit{top}}$ = place, another has $T_{\mathit{top}}$ = Person). This introduces a lot of noise in the annotations, especially in heterogeneous data with homographs \cite{21_leventidis_homograph_detection}. Thus, we need to narrow down TL$_{CS}$(c) to only 1 top level type for a given column $c$.
% \wolf{! 3/24: stop here. This becomes a description of a particular algorithm. Please first describe the intuition, the goal of what the algorithm tries to achieve. Some axioms. Something like:
% 1. we want to assign a type distribution to each column.
% 2. the idea is do this based on the aggregate values their individual types. 
% 3. intuitively each value has a distribution, the problem then becomes to somehow aggregate those.
% Intuitively, the aggregation should follow certain desiderata:
% 1. monotone in appearance: If a type appears more often, then higher weight
% 2. monotone in input weight: if a type gets assigned more for a value, then also the aggregate value higher
% 3. types that are more discriminative (appear less frequently, or are more specific) should be given higher weight.
% 4. ???
% 5. ???
% Next we show a `weight distribution assignment' that fulfills all of these 5 desiderata.
% }
% \aamod{03/30: updated the section and added the objectives before the algorithm. I would be happy to update further.}
% Assuming all the top-level types are semantically disjoint \cite{tanon_20_yago}, we argue that a column should have only one top level type.
% Ideally, we assume that the KB returns a single top-level type for each column.  However, due to homographs and the deep heterogeneity in data lakes that may lead to a value being mapped to an incorrect entity, we may get multiple top-level types for the same column.
% To do so, we use an unweighted
% voting strategy and select only one top-level type that has maximum count among all top level types of the column \footnote{\label{footnote:no_ties} In our experiments, we never encountered "ties" on real data.}.
% \wolf{3/24: I see, so this particular algorithm does not assign a distribution but the goal is to determine the most likely (one single) top level domain. I am not exactly sure why this works better in practice / experimentally as suggested below.
% Is it that keeping around a (90/10) distribution would introduce more noise than information because the 10\% are more likely to be spurious than useful?}
% Thus selected type is considered as the Top-Level Column Semantics (TL$_{CS}$) for that column.
%We experimented with different type selection strategies and found that this unweighted one was the best and that we never encountered "ties" on real data.  





% \wolf{! 3/24: An essential idea that appears to be missing in the scoring algorithm is the idea of downweighting ambiguous types.
% Say there are 1000 values that are assigned type A. 
% And there are other 1000 values that are assigned both B and C.
% Then if I understand correctly, the current math gives all three types A, B, C the same weight (the weight is only determined by how often those appear). But shouldn't A have a clearly higher weight? Whenever you assign B, it could also be C and v.v.
% So it is less discriminating}
% \aamod{03/29: Thinking about this possibility, we experimented with the scoring idea that you suggested. However, we did not find such cases in the real data. Instead we found opposite case in almost all tables as discussed in the example below:
% Consider a column about cities having 9 values that are cities and let 1 value is a random noise value that maps to a noisy type, say Arson cases. Now since 9 other are famous cities, they are also the name of movies, products, organizations, etc. For example, Boston is the name of movie (creative work), place, organization, product, etc. Let it maps to 10 such top level types. Consider all other 8 cities map to place but also to 9 other top level types (may be same as Boston or different). Due to this, we get score for place = (0.1 * 9)/10 = 0.09. However, as arson case, although is a noise, maps to a single top level type, it gets a score of 1.0/ 10 = 0.1. In this way, instead of considering the top level type of the column as place, we considered it as Arson cases. To avoid this, we count each type equally first. Later, we select a top level type and handle the hierarchy.
% }


\subsection{Relationship Semantics}
\label{subsection:relation_semantics}
%rjm this is arguing from the negative, let's turn this into a positive
%As discussed in \cref{example:intent_column_importance}, the false table unioning occurs when we do not determine the relationshipship between the columns in a table. 
%Furthermore, knowing the column pairs and understanding who are related to one another helps to marginalize the false column unioning.
Given the column semantics, we now present how we compute the SANTOS  
relationship semantics (RS).
The relationship semantics models binary relationships between columns in a table and are represented as 
edges in the semantic graph.
% We begin our discussion with an example.

% \wolf{3/24: Just to get an early intuition: is the RS at the end a forest, or a weighted forest?}
% \aamod{03/29: RS is an edge in the semantic graph.}

\begin{example}
Consider again the table (b) in 
\cref{fig:running_examples} about park and films. We would like to understand if there are binary relationships (properties) in the KB that represent the semantics captured by a pair of columns in a table.  For example, given that the column semantics of {\tt Park Name} includes the KB type {\tt park}, and the column semantics of {\tt Film Director} includes {\tt movie director}, does the KB have a relationship between the types {\tt park} and {\tt movie director} that models the same relationship as the table?  In this example, this is unlikely.  However, the KB may well have a relationship between {\tt movies} (a KB type in the column semantics of {\tt Film Title}) and {\tt movie director}.  In this section, we discuss how we determine if the relationship modeled by a pair of columns in a table likely has the same semantics as a binary relationship in a KB.
\end{example}

%We also take the help of relationship semantics for better entity mapping that eliminates some homographs from the equation.
%F%or example, we have another column providing the geographical coordinates for the places in \cref{tab:city_and_details}. When we look for the relationship semantics in the KB with Place column values as subjects and Geo column values as objects, only URIs related to the places from the first column would be able to find a relationship with the second column.
%This way, we can easily discard URIs that are related with "creative work".
%T%his increases the gap between the counts of candidate top level types and makes it easier to select one among them.
%L%ike relationship semantics, we compute the column semantics for both data lake and query tables.


We compute relationship semantics for every binary pair of string (non-numeric) columns.
The relationship semantics is computed for both query and data lake tables. Note that many pairs of columns (like {\tt Park Name} and {\tt Film Director}) may not have a semantic relationship represented in the KB.  Intuitively, there is at least an indirect relationship between all columns in a table (in this case, the director of a film shown in the park), but in this section, we are only interested in relationships represented in the KB.
%every pair of columns may not have a semantic relationship between them. They may be the properties of other columns. For such column pairs, we do not get any relationship semantics.
Suppose columns $c_1$ and $c_2$ in table $D$ have non-empty column semantics, meaning some of their values have been associated with entities in the KB.
To determine relationship semantics, we determine if a pair of values in $\Pi_{c_1,c_2}(D)$ are associated with entities $(e_1,e_2)$ that are in a KB relationship $p$.

\aamod{04/02: We already defined RS in section 3. Should we explain it only on language now?}
\begin{definition}[Relationship Semantics]
\label{def:rs}
Let $P$ be  the set of all binary relations (or predicates) in the KB.
Let $p \in P$ be a relationship between types $t_1$ and $t_2$.  Let 
$c_1$ and $c_2$ be columns in a table whose column semantics include $t_1$ and $t_2$, respectively.
If there exists a pair of data values in $\Pi_{(c_i,c_2)}(D)$ where the values map to entities $(e_1,e_2)$ in $t_1$ and $t_2$, respectively, and the pair $(e_1,e_2) \in p$, then we say the $p$ is in the relationship semantics of $\Pi_{(c_i,c_2)}(D)$.
If there is more than one KB relationship $p$ that qualifies, then  $p$ with the most associated pairs is used as the relationship semantics. We denote the Relationship Semantics between column pair $(c_1, c_2)$ using $RS(c_1, c_2)$.
\end{definition}
\begin{definition}[Relationship Predicate Confidence Score]
\label{def:brcs}
The Relationship Predicate Confidence Score (RS$_p$) for binary relationship p of $\Pi_{(c_i,c_2)}(D)$ is the fraction of the number of unique rows in $\Pi_{c_1,c_2}$ mapped to type RS($c_1,c_2$) 
to the total number of unique rows in $\Pi_{c_1,c_2}$. We denote it using $RS_p(c_1,p,c_2)$.
\end{definition}
\begin{example}
\label{example:rscs}
In Table (c) of \cref{fig:running_examples}, the Relationship Semantics for (\texttt{Person}, \texttt{Birthplace}) is $RS(\texttt{Person}, \texttt{Birthplace})$ = \texttt{birthplace} and RS$_p$(\texttt{Famous Person}, \texttt{birthplace}, \texttt{Birthplace}) = 1.0.
\end{example}
Finally, we combine CS and RS to get Relationship Semantics Confidence Score (RS$_{\textsc{Conf}}$) as we define next.
\begin{definition}[Relationship Semantics Confidence Score]
\label{def:rscs}
The Relationship Semantics Confidence Score, RS$_{\textsc{Conf}}$, of a column pair $\Pi_{(c_i,c_j)}(D)$ with $CS(c_i) = t_i$, $CS(c_j) = t_j$ and $RS(c_i, c_j) = p_{ij}$ is given by $CS_{\textsc{Conf}}(c_i, t_i) * RS_p(c_i, p_{ij}, c_j) * CS_{\textsc{Conf}}(c_j, t_j)$. It is denoted using RS$_{\textsc{Conf}}$($c_i.t_i, p_{ij}, c_j.t_j$).
\end{definition}
\begin{example}
\label{example:rscs}
In Table (c) of \cref{fig:running_examples}, {\tt (person, birthplace, city)} is RS$_{\textsc{Conf}}$ for ({\tt Person}, {\tt place}) and RS$_{\textsc{Conf}}$({\tt person, birthplace, city}) = $1.0 * 0.1475 * 1.0 * 0.6 * 0.2163$.
\end{example}
We compute RS$_{\textsc{Conf}}$ for both data lake tables and query tables. For data lake tables, we store RS$_{\textsc{Conf}}$ in an inverted index
where, ($c_i.t_i, p_{ij}, c_j.t_j$) is key and the set of tuples of (table name, RS$_{\textsc{Conf}}$($c_i.t_i, p_{ij}, c_j.t_j$)) is value. Recall that, a column may have more than 1 Column Semantics. Hence, there may be multiple RS$_{\textsc{Conf}}$ for a column pair. We store all of them in the inverted index and use one that contributes maximum score during query time which we will discuss in \cref{section:semantic_union_search}. Before we do this, 
we detail the computation of relationships that are not in the KB.

\input{sections/alt_KB_details}

==> sections/cover_letter.tex <==

\section*{Cover Letter}
% Dear reviewing team,

Thank you %so much for taking your time to review our manuscript and 
for providing us with constructive feedback
%rjm, which 
that helped us improve our manuscript. %They helped a lot to improve our manuscript during the revision.
All the major changes %from the last submission 
are \revision{highlighted in blue.}
% During the revision, we addressed all the comments in meta reviews. 
The revision addresses all meta review comments. We further corrected typos and addressed the minor issues.
%For example, we re-phrased the last line of Abstract and second paragraph (first line) of Introduction section to address minor remarks 1 and 2 ,respectively, by R2.
Due to space constraints, we focus here on the major revision items from the meta review and explain how we addressed them.

\introparagraph{Diversity and Inclusion}
We updated Figures~\ref{fig:running_examples}-\ref{fig:synth_dict} to enhance accessibility.
%rjme for people having color blindness. 
For example, colors were replaced or augmented with
%, for example, 
shapes (dotted, solid, etc. in~\cref{fig:running_examples}), font style (bold, italic, normal in~\cref{fig:synthetic_kb}) and text decorations (normal, underlined and bold in~\cref{fig:score_calculation}).

% In our previous submission, we used colors to convey information in Figure 1-5, which can be a problem for people having color blindness. So, we replaced/ supplemented colors with other encoding like the shape of lines (dotted, solid, etc. in Figure 1), font style (bold, italic, normal in Figure 2), text decorations (normal, underlined and bold) in Figure 3 and so on. We believe that these changes will help to enhance accessibility.

% In our previous submission, we used colors to convey information in Figure 1-5, which can be a problem for people having color blindness. So, we replaced/ supplemented colors with other encoding like the shape of lines (dotted, solid, etc. in Figure 1), font style (bold, italic, normal in Figure 2), text decorations (normal, underlined and bold) in Figure 3 and so on. We believe that these changes will help to enhance accessibility.

\introparagraph{Reviewer 2}
\begin{itemize}
    % \item \textbf{O1 and minor remarks:} This revision item is about improving the paper presentation and clarifying design decisions that has been taken when extracting the semantics. Specifically, we observed a confusion on if SANTOS uses meta data. During revision, we proof-read the paper to improve the presentation, fixed the typos and addressed the minor comments. To clarify that we do not use meta data like column headers, etc. when mapping to the knowledge base, we added a description at the opening paragraph of section 4 (Semantic Graph Creation with KB). We updated Section 7.1 to further clarify the mapping.
    
    \item \textbf{O1 and Minor Remarks:} We 
    %rjm use active voice:  aimed at improving the paper
    improved the
    presentation and clarified design decisions that have been made when extracting the semantics. We 
    highlighted 
    %reiterated
    the fact that SANTOS does not use metadata (opening paragraph of \cref{section:unionability_components}) and clarified that data values are mapped to KB labels and alternative names
    %rjm the mappings in 
    \cref{subsection:kb_details}. We fixed all other minor remarks throughout the paper. E.G., we updated the 
    %the words abstract and introduction are not capitalized unless enumerated
    abstract and introduction, addressing the minor remarks 1 and 2, respectively.
    
    \item \textbf{Scoring Functions (O2):}  We added more related %rjm again work is a collective noun:  works
    work~\cite{frank2005comparingrankingfunctions, GOSWAMI2017rankingfunctions, 2019_vinh_thinh_qsearch, 2021_vinh_thinh_qute} in \cref{section:semantic_union_search} that we use to motivate our scoring function. Accordingly, we re-wrote the "Scoring function" paragraph (second paragraph \cref{section:semantic_union_search}) to further clarify our intuition. 
    %metareviewer asked for citation so we need to say we did this!!!
    We cite Ho et al.\cite{2021_vinh_thinh_qute} which uses a similar intuition for the scoring function. Moreover, we re-worded and added explanations in \cref{subsection:csconfidence}, along with more related work~\cite{1957_luhn_tf, 1988_sparck_idf, ramos2003using}
    to better explain the equations.
    
    \item \textbf{O3, Compare against \textit{Seeping Semantics
    %rjm this is not full title Linking Datasets using Word 
    (SemProp)}:}
    %Thank you for pointing out this paper. 
    We cited this work~\cite{Fernandez2018SeepingSL} and explained how it differs from SANTOS in the related work section (\cref{section:related_search}). Specifically, Seeping Semantics relies solely on metadata like column and table names to find  related tables. SANTOS, however, is based on the cell values rather than the metadata. As we explained in \cref{section:intro} (first paragraph), the motivation behind using cell values and not using metadata is that the open data tables generally have missing, inconsistent or incomplete metadata. We include Seeping Semantics (SemProp) in our experiments (see 
    \cref{section:experimental_setup}, \cref{section:results_effectiveness}, \cref{fig:pr_results}) on the REAL Benchmark. We do not run SemProp on the other two benchmarks (TUS and LABELED) since they synthetically generate unionable tables from the same seed tables (\cref{section:experimental_setup}). Thus, these benchmarks by construction artifically have identical column names for unionable columns and different names for non-unionable columns.  
    %, which makes them unsuitable for evaluating techniques that rely on such meta data.
    %rjm:  you have to state the results!!!
    For a fair comparison, we modified SemProp to use YAGO instead of the Experimental
Factor Ontology (EFO) from their code repository as YAGO has much better coverage over the REAL benchmark.
    SemProp outperforms D$^3$L, but has a much lower MAP@K (40\%) than SANTOS (77\%).
\end{itemize}

\introparagraph{Reviewer 3}
\begin{itemize}
    \item \textbf{Fix Writing (O1):}
    We 
    %aimed to clarify 
    clarified the definitions and simplified the manuscript according to O1. Other specific comments O7, O13 and O14 (related to O1) are also resolved.
    % So, we will explain how we address each specific comment.
    We addressed O7 which is related to SANTOS Top-k Union Search Solution (\cref{def:new_santos_unionability}). We re-worded the definition as suggested in the review. Furthermore, to clarify the intuition behind the definition, we explained the nature of the scoring function (\cref{section:alt_relationship_unionability}) and swapped the position of \cref{def:new_santos_unionability} and the following example (\cref{example:definition_motivation}) to make it easier to follow.
    Next, O13 and O14 are related to the distinction of pre-processing and query tasks. 
    For simplicity, we split Section 7.3 (Pre-processing and Query phases) from the last submission into \cref{section:preprocessing_phase} (Pre-processing Phase) and \cref{section:query_phase} (Query Phase). 
    The tasks in the pre-processing and query phases are added to their respective sections. We also report the indexing time needed to pre-process the KB (a one-time task) in \cref{subsection:kb_details} and updated 
    \cref{section:results_effeciency} (second paragraph) to clarify pre-processing and query time.
    
    \item \textbf{Fix Writing (O2):}
    % This revision item is about providing better  motivation for 
    For O2, we refined the motivation for
    our hypotheses, also incorporating other related comments: O6, O9 and O11. To address O6,
    % is about how many rows a query table needs. 
    we explain at the end of 
    \cref{section:results_KB} (\revision{\textit{Recall that, SANTOS only uses $\dots$}}) that SANTOS is effective because the number of rows is fairly high in data lake tables. We reported the number of rows in each benchmark in \cref{fig:benchmark_statistics}. 
    Similarly, we resolved O9 in \cref{subsection:csconfidence} and O11 in \cref{section:results_effeciency}. We also explained that the absence of homographs is helpful, but not a necessary condition for \SANTOS to be effective as reported in \cref{section:results_effectiveness}.
    
    \item \textbf{Fix Writing (O3) and Clarify (O4 and O5):}
    For O3, in the newly separated subsections for pre-processing \cref{section:preprocessing_phase} and query phases (\cref{section:query_phase}), we have provided an analysis of time complexity (this also addresses O8 and O10).
    For O4, we added further discussion on SANTOS scalability in \cref{section:results_effeciency}.
    We also clarified all the pre-processing steps in ~\cref{section:preprocessing_phase} and also reported computation time for each step (\cref{section:results_effeciency}).
    To address O5 concerning symmetric relations, we added an explanation in \cref{section:semantic_union_search}, below \cref{eq:rel_match}. Indeed, depending on the KB, $RS(C_1, C_2)$ can be different from $RS(C_2, C_1)$, so the KB can possibly return $RS(C_1, C_2)$ for the data lake table and $RS(C_2, C_1)$ for the query table. To model this difference, if we find a relationship semantics (RS)  in both directions for a data lake table, we preserve them both. Then in the query phase, we select the RS that maximizes the relationship match score w.r.t. a query table’s RS (see ~\cref{eq:rel_match}).
\end{itemize}

\introparagraph{Reviewer 5}
\begin{itemize}
    \item \textbf{O1 and O2}: We removed the verbosity in \cref{subsection:theory_synthesized_cs} as suggested (O1). We rephrased the opening paragraph of \cref{section:synthetic_knowledge_base} to emphasize that we do not use an external KB in this section. Also, we rephrased the sentences in \cref{subsection:theory_synth_relationship} to make it clear (O2).
    %\item \textbf{O2}: We rephrased the opening paragraph of \cref{section:synthetic_knowledge_base} to emphasize that we do not use an external KB in this section. Also, we rephrased the sentences in \cref{subsection:theory_synth_relationship} to make it clear.
    \item \textbf{O3}: We moved the technical proposal motivated by \cref{example:multiple_annotations} outside of the example environment and placed it below the example.
    \item \textbf{O4}: The typo is corrected (see \cref{section:semantic_union_search}, below \cref{example:multiple_annotations}).
    \item \textbf{O5}: We explained the type of values that exist in the benchmarks that we used in the experiments (see \cref{section:experimental_setup}, Benchmarks Paragraph). We also added the number of rows in different benchmarks in \cref{fig:benchmark_statistics}.
\end{itemize}

We really appreciate all your time and help and we will be happy to provide further details.

- SANTOS Authors

==> sections/main_contributions.tex <==
\section{Main Contributions}

Note that this is not a real section for the final paper. It simply serves as a
place to keep track of our main contributions. These determine
how we define unionability and contrast our work against related approaches,
and they guide the design of the experiments and the benchmark.
Let $Q$ and $D$ denote \emph{query table} (QT) and
candidate \emph{data-lake table} (DLT), respectively.


\newcommand{\qtab}{Q}

\begin{table}[h]
\centering
\small
\begin{tabularx}{\linewidth}{@{\hspace{0pt}} >{$}l<{$} @{\hspace{2mm}}X@{}} 
% table over whole line width; first column in $-mode
\hline
\textrm{Symbol}		& Definition 	\\
\hline
	A		& attribute \\
	B       & back up for attribute if we need to distinguish the attributes of different tables\\
	c/C     & Columns (just as a backup, we will use attribute in most of the cases) \wolf{10/18: even if column is used as synonym for attribute, won't the symbol used still be the same?}\\
	D       & data lake table \\
	E   &set of all the entities in KB\\
	P   &Set of all the predicates (relation semantics) in the KB\\
	Q   &Query Table\\
	r   &a conceptual root node of the table\\
	T   &set of all the types (classes/column semantics) in the KB \\
	t   & any arbitrary $t \in T$\\
	V_D   & set of all the attribute values in the data lake\\
	V_Q & set of all the attribute values in the query table\\
	X_D   & set of all the attributes in all the data lake tables\\
	X_Q   & set of all the attributes in all the query tables\\
	T_{top} &Set of all the top level types in the KB \\
	TLCS(A) & Top level column semantics for the attribute A. For example: TLCS(A) = "Person"
		\wolf{10/18: better use a macro with $\mathit{TLCS}$ instead of $TLCS$}	\\
	CSCS(c_{t}) & Column Semantic Confidence Score for type t of column c\\    
\hline
\end{tabularx}
\end{table}

\subsection{Definition of Unionability}

\introparagraph{Table Union Search (TUS) \cite{nargesian_18_TUS}}
Bipartite matching of columns from $Q$ and $D$;
2 columns match if they have the same type.
\begin{itemize}
    \item Table semantics: TUS table unionability does not check if $Q$ and $D$ are
    about the same subject. For instance, tables about students and restaurants may share
    many columns of the exact same type (address, phone number,
    birth date/date the restaurant opened), but they are not unionable.
    (TUS may be able to determine that student and restaurant names are not
    of the same type, but the many other perfectly matching columns would still
    result in an overly high unionability score.)

    \item Column-relationship semantics: TUS table unionability
    does not consider semantic relationships between columns in a table.
    Consider a table of students with columns \texttt{name} and
    \texttt{academic-advisor-phone-number}.
    If QT $Q$ is about people and their phone numbers, the advisor's
    number in DLT $D$ is a false positive: it is a phone number (correct type),
    but not of the person the row is about (incorrect semantics).
    
\end{itemize}

\introparagraph{Sarma et al. ``Finding Related Tables'' 
\cite{sarma_12_finding_related_tables}}
Bipartite matching of columns from $Q$ and $D$;
2 columns match if they have the same type;
$Q$ and $D$ must have the same subject column.
\begin{itemize}
    \item By matching tables with the same type of subject column,
    the TUS table semantics problem is only partially addressed. Unfortunately,
    the authors assume that each table has only a single subject column,
    which is the (quasi-)key of the table. This does not cover relationship
    tables, e.g., a table about movies that were shown in parks and whose
    columns report (1) park properties (e.g., address),
    (2) movie properties (e.g., director, rating), and
    (3) relationship properties (e.g., date the movie was shown, ticket price).
    
    \item Like TUS, this approach does not consider column-relationship semantics.
    
    \item \grace{9/2: Their approach, Sarma, requires that entity-complement tables have similar, if not the same schemas. We do not have this limiting requirement, so we can retrieve more candidate tables for a given query table. Also, without this constraint, we are able to return relationship tables as unionable tables for entity query tables.}
\end{itemize}

\introparagraph{Solution}
To address the issues of table semantics and column-relationship semantics, we
introduce the notion of a \emph{semantic tree} for a table.
A relationship table has a conceptual root node $r$ whose children are the
keys of the participating entities. In the movie-park example, there are 2
children: \texttt{park-name} and \texttt{movie-title}. Each inner node
(i.e., a node that is not a root or leaf)
points to all attributes that functionally depend on it.
E.g., the children of \texttt{movie-title} could be \texttt{director}
and \texttt{rating}. There could be more levels, e.g., \texttt{director}
may functionally determine \texttt{won-Oscar}, and so on.
An entity table is a special case of a relationship table where the root has
only 1 child.

Intuitively, the children of an inner node in the semantic tree describe
properties of
the corresponding attribute. This way it is clear if a phone number belongs
to a student or their advisor. The semantic tree also enables a QT about parks
to be unioned with the (properly projected) movie-park DLT. Similarly,
a QT of famous award winners could be unioned with the \texttt{director}
and \texttt{won-Oscar} columns of the movie-park table.

In general, we assume for the QT that the analyst specifies a semantic tree
by identifying a root node---called the \emph{intent column}---and its
children---the \emph{property columns} of the intent column. Then
QT and DLT are considered unionable only if the DLT's semantic tree
(1) contains a node of the same type as the intent column and
(2) there is a large number of matches between their children as well.

\mirek{8/5: This needs more work. Could the semantic tree be a DAG?
Could there be cycles?
Do we need directed edges or can some attributes be in the same equivalence class?
For instance, a park may be uniquely identified by its name but also
by its address or by its contact phone number. In that case it may
be difficult to determine automatically what the actual key
selected by a human expert should be and
one might need to assign name, address, and phone to the same ``bag'' of
attributes.
Similarly, a key may consist of multiple columns, e.g., only first
and last name together sufficiently identify a person; same for
city name and state combinations in the US. What is an elegant way to handle this?}

\nikos{8/13: How do we measure similarity between the QT tree and the DLT subtree?}
\aamod{08/24: We compare how many nodes and edges from the QT tree are found in the DLT subtree. For this, the nodes and edges i.e., column and relation semantics from the QT tree are computed. Then, they are compared with Tuple of Bag of words for the DLT that contains all score, token and column information.}
How do we automatically determine the semantic tree for a given DLT?
Abstractly, we search for functional dependencies and check for possible
semantic relationships between columns in the KB and based on column
co-occurrence in other DLTs. However, this is tricky in the presence
of multi-valued dependencies. E.g., a movie may have
2 directors and 2 lead actors.



\subsection{Notion of Same Column Type}

\mirek{8/5: This needs to be expanded by including other related work on
identifying column types or determining if 2 columns have the same type.
Start with the ``Finding related tables'' paper.}

\introparagraph{TUS} TUS relies on 3 different measures of column unionability,
which are discussed below. It expresses the probability of 2 tables being
unionable as a function of the probability of pairs of columns being
unionable for a bipartite matching between the columns of the QT and DLT.
\begin{itemize}
    \item Problem with value-set-based column unionability:
    This measure only considers the direct intersection between column pairs
    $(C_Q, C_D)$ from $Q, D$.
    We also need to consider ``transitive intersection:'' if $C_Q$ and $C_D$ both
    have a large intersection with some column $C$ in another table $U$, then they
    still are likely to be of the same type.
        
    \item Problem with semantic-type-based column unionability:
    This measure considers the set of distinct types found for the column values
    in the knowledge base (KB). Homographs and expanded search criteria (e.g.,
    search for entire exact string vs. a normalized version where stop words
    are removed and stemming etc is applied vs. search for a substring) can lead to
    false positives in the set of types for a table column. Due to set semantics,
    a single false type has the same weight as 100 appearances of the correct type.
    TUS also considers the option of looking only at the top-$k$ most frequent
    types in the column, but that still suffers from weighing all top-$k$
    types equally.
        
    \item Problem with NLP-based column unionability:
    This measure relies on ``generic'' embeddings obtained from some text corpus
    that may or may not be related to the data in the data lake. EmbDI showed that
    the outcome of data integration tasks such as schema matching
    improves when working with embeddings based on table content, not generic
    text collections. This raises the question if the NLP-based measure can be
    improved by using more customized embeddings as well. SANTOS currently
    does not use this, but it could be added.
\end{itemize}
We can discover transitive intersections by creating a graph where each node
is a DLT column and there is an edge between each pair of columns from
different tables that have a non-empty intersection of values; edge weight
is determined by intersection size. We can then either find clusters
of connected nodes (dense neighborhood of heavy edges) or perform a
random walk from a start node guided by edge weights to determine the
``nearby'' nodes (and thus the transitively most overlapping columns)
for that start node.

For the issue of determining the column type from the KB responses, we need
a probability-based framework where the total number of KB responses and their
diversity determine the probability of a type. Here we can either limit ourselves
to the top-level types in YAGO (children of ``thing'') or also
distinguish types at finer granularity.


\subsection{Ranking Dependent on the number of attributes}




\introparagraph{TUS and multi-valued dependencies}
Let us consider \cref{fig:entity_films} about movies. Since a movie can have
multiple actors, the table creator here decided to added three columns
to store the names of up to 3 main actors.
Another table creator may decide to violate first normal form (1NF) by simply storing
the list of actors as a String-type ``value'' in a single actor column.
Yet another table creator may also use a single actor column, but create multiple
rows for the same movie, each with a different actor value.
These are very common cases in the open data tables.
\mirek{8/10: Cite some concrete numbers here for a real data lake.}
Even though all 3 table versions encode the same information (assuming at most 3 actors
per movie are recorded), TUS' unionability score would change because it depends
on value overlap in a column and on the total number of unionable attributes.
\mirek{8/10: Can we quantify this by showing some actual unionability scores
for an example?} 
\aamod{08/10: The ultimate score TUS uses is the  percentile position of each table. First, the percentile distribution is created using a large number of tables for different alignments. Now, for any table D, first the percentile score is determined for different alignment conditions (2,3,4,... upto the number of attributes) by comparing the attribute unionabiity scores for the respective alignments on the repository. Note that the product of attribute unionability score is used to map on the percentile distribution. Then, the alignment at the highest percentile is selected for D and same percentile score is the unionability score that D uses to compete with other tables. Once the local percentile for all D's are found, same percentile score will be the unionability score for the table. Hence, when the number of attribute differs, the comparing percentile distribution changes. Even for 1 more attribute, the distribution used to compute the unionability score changes which impacts the ranking. However, its difficult to quantify as we also need to consider the percentile distribution.}

However, we argue that since the tables contain equivalent information, their
unionability scores ideally should not be affected by changing the encoding.

\introparagraph{Solution} Even if a table has multiple actor columns, our algorithm
determines unionability based on the \emph{set} of types and hence does not
``double-count'' repeat occurrences of the actor column.
Notice that this is not straightforward. For example, in case of the movie-park table,
we want to keep both park location vs movie location separate. This is achieved
by making the type set ``aware'' of the semantic tree, i.e., by only
applying set semantics to children of the same node.
\mirek{8/10: Aamod and Grace, please explore this a little more. Aamod's initial statement
said that the location types would also be merged. I think we can fix this by taking the
semantic tree into account.}
\aamod{08/10: Yes, I agree. Once we have the intent graph, this problem gets solved easily.}

\mirek{8/11: We also need to discuss if our scores are affected by the multiple-row
encoding. Can show this mathematically by thoroughly exploring the possible cases?
E.g., consider scenarios where all/some/none of the actors of a movie appear in the KB
and take into account if any of those actors appears in another movie.}


\subsection{TUS Benchmark issues}

\begin{itemize}
    \item The 10 seed tables used by TUS were real  and meaningful tables. However, the process TUS used to generate the benchmark by projecting and selecting columns and rows from those real tables
    produced many tables with meaningless information. These kind of tables are not found in the data lake. Hence, we argue that such
    tables should not be included in the benchmark. For example, the generated table
    \texttt{t\_1f6b65ebc2ab3ed3\_\_\_\_c2\_1\_\_\_\_3.csv}
    has columns updated date and updated month, but there is no information
    what was updated on that date.
    Table \texttt{t\_013a2f8c584d44d7\_\_\_\_c2\_0\_\_\_\_2.csv}
    has two columns about quality containing values A, B, C and E.
    However, there is no information what these quality ratings are for.
    \item Some labeling are biased on the KB. E.g., continent, country
    and city are treated as the same types based on KB.
    \mirek{8/11: If the KB declares these to be the same type, can we do anything
    about this at all?} 
    
    \aamod{08/11: I agree! In terms of benchmark, I think there's very little we can do in that case. Still in case of algorithm, since we consider the granularity too, we might be a bit better on that. For example, continent name and country name are considered equally unionable by TUS because both of them are location. So, if there are two data lake tables-- D1 having continent name and D2 having country name-- and a query table Q having country name column, both D1 and D2 are considered equally unionable with Q. However, SANTOS will also see the granular types which will at least rank D2 higher than D1 when Q is the query table.}
    
    \nikos{8/13: I don't follow: if the KB says 2 columns have the same type how is SANTOS going to figure out that they are different?
    Maybe elaborate a bit in the text what the situation is through this example, including what the KB returns.}
    
    \item For benchnmark, only 10 tables having disjoint attributes were used to create the benchmark tables. Those columns had no joinable columns between them. 
    \introparagraph{Problem:} In the benchmark, there are a total of 1530 data lake tables generated from 10 seed tables. In average, it means 153 tables per seed table. In accuracy reporting, we saw that the SET unionability precision differs by 13\% with NLP unionability precision. So, if there are 9 seed tables where SET unionability is working well and there is just one seed table where SET fails and NLP is needed, the precision of SET is affected a lot. This is because when SET fails in 1 seed table, it fails almost in all 153 tables generated from it. So, if we just remove that one table, and compare the precision, may be SET is not that bad than NLP. So, my point is that with only 10 seed tables, the skewness is high and we need more seed tables to see the proper precision pattern of SET and NLP.
    \item Intent columns are not specified, because TUS did not need them.
    For our approach, we need to identify possible intent columns for QTs.
    
    \nikos{8/13: I assume this also means that we need to be more careful than TUS when defining the ground truth since the intent column affects unionability.
    We may also need to argue *why* knowing the intent column in the QT is a justified assumption.}
\end{itemize}
\subsection{Experiments and TO-DOs}
\begin{itemize}
    \item \introparagraph{Shortlist query tables} Select some entity tables from the data lake having a single intent column and all other columns as its properties. For example: \href{https://northeastern-my.sharepoint.com/:x:/g/personal/m_riedewald_northeastern_edu/Ef00c89QxD9Ahx0YyQvs19UB-m27OfBleKWvNZx5snbjYA?e=5lkcxi}{film location table}. Here, the film title is the intent column and all other columns are its properties.
    \item \introparagraph{Number of relation semantics covered in the KB} For each table, mark the intent column manually. Then see how many relation semantics are returned by the KB considering the intent column values as subjects in the KB.
    Record two numbers:
    
    1. Given n tuples after projecting a pair of columns from the table, how many tuples can be mapped to the KB when one value in the tuple is subject and next value is object?
    
    2. Given an intent column and m property columns, we expect to find m relation semantics from the KB. Run an experiment to see how many we can find. 
    
    Record the data in the following schema to cover both cases:
    \{Table Name, attribute1 Name, attribute2 Name, number of unique tuples in the projection, projected unique tuples covered in the KB, coverage percentage, predicate for maximum number of tuples from the KB\}.
    
    Example:  \{presidents.csv, Name, political party, 10, 8, 0.8, memberOf\}
    \item \introparagraph{Functional dependencies} If we are not able to find the relationship between the columns from the KB, we use Functional Dependency to know the related columns. Then, the synthetic relation semantics will be assigned to the values.
    
    \introparagraph{TODO} Code our existing FD concept and see if it works or not in the tables we shortlisted.
    \item Use FD and yago separately (and together) to create the intent graph and verify if we get what we are looking for. 
    \item Verify table union search precision in the following way:
        
        For same QT, project out subject column and 1 property and consider the resulting table as a query. Next, project out subject column and 2 property columns and consider the resulting table as a query. Do same for 3,4,.. properties and see if the returned DLT also have those properties, and report the precision. 
        
        We would do this for just YAGO, just the Synthetic KB (with the FDs involved), and YAGO and Synthetic KB combined.
\end{itemize}

==> sections/meta_reviews.tex <==
\section*{Meta-reviews}
\revision{This section is temporary!!!}
\begin{verbatim}
Please use \revision{} to make changes for the revision.
\end{verbatim}

\subsection{Use of colors}
\begin{enumerate}
    \item Using color \dots. Figures 1-5 use colors to convey information, which can be a problem for people who are color-blind (lack of accessibility). Please update your figures accordingly.
\end{enumerate}

\subsection{Reviewer 2: major revision}
\begin{enumerate}
    \item \introparagraph{Clarify if schema is used to extract semantics} \aamod{Updated opening paragraph in \cref{section:unionability_components} to clarify that we do not use schema information. Also updated \cref{subsection:kb_details} to clarify mapping of tables to the KB.}
    
    "The paper presentation needs improvements to make the discussion clear and especially explaining some of the decisions that has been taken when extracting the semantics. For example, how to deal with the names of the columns that contains abbreviations and synonyms of the object in the Knowledge base such as dept. name instead of department name and so on. ", The authors should address all the comments and proof read the paper to improve the presentation. (O1 \& Minor Remarks)
    \item  \introparagraph{Justify scoring functions}
    
    The scoring functions are based on heuristics that has not been justified. The authors need to explain for each scoring function why it makes sense to use such function. ", For the scoring functions, a good explanation or referring to a published paper will be enough. (O2)
    \item \introparagraph{Compare with seeping semantics}
    
    "The experimental evaluation needs to compare with more systems that exist in the area", "For the systems, you can check "Seeping Semantics: Linking Datasets using Word (O3)".
\end{enumerate}

\subsection{Reviewer 3: major revision (Fix writing O1-O3 \&\& Clarify O4, O5)}
\begin{enumerate}
    \item \introparagraph{Clarify definitions}
    
    Even if overall, the paper is understandable, some definitions are unclear and there are parts of the paper that are hard to follow (see the specific comments that follow)
    
    \textit{Specific comments:}
    \begin{itemize}
        \item  Definition 5 (and 7): is the relationship semantics a symmetric relation? It looks like CS(C1,C2) can be different from CS(C2,C1). Please clarify. (O5) \aamod{Added description that we sent on author's feedback phase below \cref{eq:rel_match}.}
        
        \item Definition 9, Page 4: it is definitely not clear. Please, rewrite it in a more comprehensible way. It seems to be dependent on a "magic" semantic function that returns the "best" matching. This is too shallow, please specify the notion of matching in a more precise way. Finally, I would not expect in a definition a "is to find" locution (last sentence). You should rather use "is" or "is not". (O7)
        \item Section 7: Please, specify better all the tasks that are included in the "indexing" and in the "pre-processing" phases. (O13, O14)
        \aamod{Updated \cref{section:preprocessing_phase} and \cref{section:query_phase} to clarify the tasks during pre-processing and query phases.}
    \end{itemize}
    \item \introparagraph{Motivate restrictive hypothesis}
    
    Some hypotheses look rather restrictive and should be better motivated (see the specific comments that follow) (O2)
    
    \textit{Specific comments:}
    
    \begin{itemize}
        \item Page 4: the notion of Query Table is unclear. Should it contain a relevant number of tuples? How many? It seems that the overall technique is unreliable if it contains just a few tuples, as in the running example. Also, you restrict the approach to the case in which there is only one "intent column". I understand that this allows you to deal with trees only, but is it enough general? This choice should be better motivated. (O6)
        \aamod{Added a paragraph at the end of \cref{section:results_KB} to explain that SANTOS is effective because the number of rows is fairly large in the data lake tables.}
        
        \item Formula (2) in Section 4.2: Please, use a different and more precise notation for the number of entities that map to a. Also, how did you set the 10 threshold? (O9)
        \item Section 5.1: The hypothesis of the absence of homographs is rather strong and the impact of the adoption of tools for its discovery should be included in the overall cost of the search for unionable tables. You should discuss this point more. (O11)
        \aamod{Reported the time taken to find the homographs in REAL benchmark in \cref{section:results_effeciency} (to be completed by @Zixuan).}
    \end{itemize}
    
    \item \introparagraph{Explain complexity}
    \begin{itemize}
        \item The study of the complexity of the approach is missing and needs to be addressed. (O3) \aamod{Resolved the specific comments O(8) and O(10).}
        \item The performance of the indexing phase is rather poor, which makes hard the scalability of the approach in a dynamic environment in which data stores are progressively collected. Also, it seems that some needed pre-processing (e.g., the discovery of homographs and of FDs), has not been considered in the computation. This aspect should be discussed more. (O4)
        \aamod{Explained in \cref{section:results_effeciency} based on what we replied on author's feedback phase.}
    \end{itemize}
    \textit{Specific comments:}
    
    \begin{itemize}
        \item End of Section 4.1: the search of top-level types, which also involves the discovery of column and relationship semantics, seems a very complex task. You should clarify its complexity. (O8) \aamod{Added explanation at the end of \cref{subsection:csconfidence}}.
        \item Section 4.3: The computation of the relationship semantics seems another very complex task. Some words on its complexity should be said. (O10)
        \aamod{Added explanation at the end of \cref{subsection:relation_semantics}}.
        \item Section 8.4: It is not clear if the indexing time includes all the tasks described in Section 7 as well as all the activities that are strictly needed to create a viable index. Also, you should specify if and where the "pre-processing" step discussed in Section 7 is counted.
        \aamod{Explained in \cref{subsection:kb_details} that this is a one-time task and takes less than 20 minutes.}
    \end{itemize}
    
\end{enumerate}

\subsection{Reviewer 5: minor revision}
\begin{enumerate}
\item \introparagraph{Remove verbosity in \cref{subsection:theory_synthesized_cs}} \aamod{Resolved! Updated \cref{subsection:theory_synthesized_cs} and started directly at ``Generally,}

In some places, the paper appears a bit too lengthy. For instance, I think you can remove the beginning of Section 5.1, and start directly at "Generally, values..." (O1)

\item \introparagraph{In \cref{section:synthetic_knowledge_base}, write precisely that KB is not used}
\aamod{Resolved! Updated \cref{section:synthetic_knowledge_base} opening paragraph and rewrote the confusing portion in \cref{subsection:theory_synth_relationship}.}

In Section 5.2, you write "has value-pairs not found in an existing KB" and then again "RS was not found from the existing KB". This confused me: I thought Section 5 was not using an existing KB at all, but just "synthesizing" KB-style information. This is consistent with the material in Section 5. Can you explain/rephrase? (O2)

\item \introparagraph{Keep proposal outside of example 17}
\aamod{Resolved! Brought the proposal outside of the example.}

Example 17 contains: "Faced with such competing semantics... we propose a 2-step approach..." An example is not the right place to present/propose an idea/technique. It should be proposed before or after examples, interspersed with examples, as needed. (O3)

\item \introparagraph{Correct typo and change $\in$ to $=$ in \cref{section:semantic_union_search}}
\aamod{Corrected!}

 Under Example 17, let $a1,a2, ... \in (CS(Qc) \cap CS(Tc))$ : this is not very clear. The intersection $CS(Qc) \cap CS(Tc)$ is a set. Do you mean each of $a_i$ is a member of this set? but if $a1, a2, ...ax$ is the intersection itself, you should write $a1, a2, ..., ax = CS(Qc) \cap CS(Tc)$ , isn't it? (O4)
 
 \item \introparagraph{Update table in figure 6} \aamod{ resolved! Included the number of rows in (\cref{fig:benchmark_statistics}). Added description in benchmark details to explain the type of values they contain.}
 
  I would like the authors to say more about the types of values that are present in the benchmarks. All examples appear to be on strings; in some cases the text states that numbers are ignored. Are there numbers, dates, geographic coordinates, etc. in these experimets? If yes, how do the authors handle various types when comparing data from the tables to YAGO (casting, etc.)? (O5)
\end{enumerate}

==> sections/semantic_unionability_search.tex <==
\newcommand{\intent}{\mbox{intent }}
\section{Semantic Union Search}

%\aamod{10/20: Please feel free to visit and leave the comments on this section. I am still working to make it more precise. My intention is to first describe how we compute the scores for each triple i.e., multiplying the column semantics and relation semantics scores. After that, I thought of explaining how we compute the matching score between each triple pair i.e., by multiplying the individual triple scores. Finally, we find the weighted set containment of the query table's triples in the data lake table's triples, which gives us the final unionability score.}
%\aamod{10/20: I am looking for a suggestion on describing the inverted index. Shall we do it with an example before this section? I am not sure where to plug it in.}
%\zixuan{10/21: I'd like to keep it here. No need to describe the inverted index a lot since it's quite common.}

\label{section:semantic_union_search}
\begin{figure*}[h]
  \includegraphics[scale = 0.5]{figures/pipeline.pdf}
  \caption{Pipeline of SANTOS. (a) Preprocessing phase: data-lake tables are labeled with types from YAGO or {\em synthesized KB}. (b) Query phase: the query table is annotated, and we query the data lake to retrieve and rank unionable tables. Columns highlighted in yellow represent the (matching) intent column. The type hierarchy is omitted for simplicity.}
\label{fig:pipeline}
\end{figure*}
The SANTOS algorithm works in two steps, namely \emph{pre-processing} and \emph{query}. 
We summarize the former next, then discuss the computation of the unionability score
during the latter.

\subsection{Pre-Processing Phase}

In the offline pre-processing phase, shown in \cref{fig:pipeline}(a), data-lake tables are ingested to populate the
inverted indexes for both KB-derived and synthesized relationships
% and the synthesized relationship dictionary
, as discussed in Sections~\ref{section:unionability_components}-\ref{section:synthetic_knowledge_base}.%previously.

In the inverted index, the key is either a KB-derived relationship, e.g.,
\texttt{(person,birthplace,place)}, or a synthesized relationship, e.g., 
\texttt{RS(A,B)}. %between columns
% \texttt{A} and \texttt{B}.
% in a data lake table $D$ where the KB did not return any types for any of the pairs of (\texttt{A}, \texttt{B}) values in $D$.
For the synthesized case, the type of the involved columns like \texttt{A}
and \texttt{B} is implicitly set to NULL and their respective score to 1.
The corresponding value of an index entry is a set of tuples, each consisting of
a table ID
%the IDs of the two columns involved in the relationship, 
and the
corresponding relationship-semantics confidence score RS$_{\textsc{Conf}}$ (\cref{def:rscs}).
The set contains one tuple for each table whose semantic graph contains the
relationship defined by the index key.
If a table contains multiple column pairs with the same relationship semantics,
only the one with the highest score is recorded in the value list. For example, looking back at \cref{fig:running_examples_2}, if \texttt{Actor1} and \texttt{Actor2} were both assigned in a relationship with \texttt{Title}, the one with the higher confidence (RS$_{\textsc{Conf}}$) will be added.
\grace{3/25: Is it better to represent this paragraph as an example?} \aamod{03/31: This is just 1 sentence and has not been used again anywhere. So, let's leave it in the paragraph?}

% In the synthesized relation dictionary, the key is a pair of values
% such as mfa\_boston in \cref{fig:synthetic_kb}. The dictionary value component
% is a set of column pairs and the corresponding scores for all column pairs
% that either contain this value pair or do not directly contain it, but
% there is a non-empty intersection between their set
% of value pairs and a column pair that contains the value pair.
% (In \cref{fig:synthetic_kb}, mfa\_boston is associated with
% E\_F: 1.0, because column pair (E, F) contain (mfa, boston),
% and with C\_D: 1/3, because the intersection between the pairs in
% (C, D)---which does not contain (mfa, boston)---and in (E, F)
% is the pair (greenwich heritage, greenwich) out of 3 rows).

Using the inverted index as well as the other dictionaries
%shown in \cref{fig:indexes} 
allow for efficient search for candidate unionable tables and contain all scores needed
for ranking them at query time.

\subsection{Query Phase, Unionability Scoring Function}

In the query phase, shown in \cref{fig:pipeline}(b), the user provides a query table $Q$ in which the \intent column
is marked.\footnote{the user may also select a set of property columns to consider. In our experiments (\cref{section:experiments}), we simply assume that the user is interested in all property columns.} %along with a set of property columns. \grace{3/21: Does the user also mark the property columns?} \aamod{3/21: Not in the experiments. We simply consider other columns as property or property of a property}
We find the query table's relationship semantics between the \intent column
and each property column as discussed for data lake tables.
Note that
% \zixuan{multi-level query tables never defined before. Either we introduce that we call such table multi-level table here or we just use something like "some tables"}
% \roee{we may also want to define it in Section 3 if you think it is important}
some property column in $Q$ may not have a direct relationship with the \intent column,
but is a  property of one of the other property columns.
For instance, \texttt{Geo} in \cref{fig:running_examples}(c)
is a property of \texttt{Birthplace}, which %in turn 
is a property of
\intent column \texttt{Famous Person}.
Hence, SANTOS also finds the relationship semantics between all pairs of columns
where at least one of them does not have a direct relationship with the \intent column.

%\grace{3/21: Do we also find the column semantics for the QT?} \aamod{yes, we do} %Finally, we combine the computed semantics to form the triples as described in \cref{section:unionability_components}.
%If we get more than one relationship
%If there are unnormalized columns in the query table like actor columns in \cref{example:normalization_problem}, we get the same triple for multiple column pairs. 
%\rjm{10/31:  I don't understand the next sentence.  what is referrent of its?}
%To prevent double counting of such unnormalized attributes, we only keep the triple having maximum count and remove its duplicates. 
%We combine such columns pairs into a single pair with a single relation semantics.  
%\aamod{10/20: I will add an example once we merge the running example tables.} Note that the user latency of SANTOS is dependent only on the second step. 
% \roee{I also called the pre-processing step ``offline'' to clarify this}
Given the annotated semantics of the query table, SANTOS searches
for all data lake tables whose semantic graph contains the relationships in the semantic tree of the query table. 
It does so by %simply 
looking up those relationships in the inverted index and
retrieving the set of candidate tables and their respective confidence scores.
Then for each column pair in the query table's semantic tree, SANTOS computes the unionability score with column pairs of candidate tables based on RS$_{\textsc{Conf}}$ of different hierarchy levels. This allows us to find data-lake tables that are unionable in different granularities. The algorithm then selects the column pair with the maximum score with the query table.  
\begin{example}
For column pair \texttt{(Person, Place)} in Table (c) of \cref{fig:running_examples}, we have multiple RS$_{\textsc{Conf}}$ in our inverted index with varying granularities: \texttt{(person, birthplace, place)}, \texttt{(person, birthplace, city)}, \texttt{(singer, birthplace, city)}, etc. 

We return the RS$_{\textsc{Conf}}$ that has the maximum score with the query table. SANTOS can return \cref{fig:running_examples} (c) as a table unionable with a general query table about people and their birthplaces, or with a specific query table about singers and their birth cities.
%(selecting certain rows).
\end{example}
% For instance, we stored more than one RSCS (\texttt{(person, birthplace, place)}, \texttt{(person, birthplace, city)}, \texttt{(singer, birthplace, city)}, etc.) for column pairs \texttt{(Place, Famous Person)} in Table (f) of \cref{fig:running_examples}.

% \begin{example}
% \label{example:tbw}
% Some triples and their score for \cref{tab:city_and_details} are:
%  (place-birthPlace-person, 1.0), $\dots$, (physicist-hasOccupation-profession, 0.166).
% \end{example}
%We search the inverted index using the query table's relationships to find the matching data lake table relatioships. 
%Ideally, we would find a higher unionability score with higher number of matching triples.
%\roee{revisit after the definition is final:} 

A SANTOS unionable table shares relationship(s) from the same intent column with the given query table. 
% For SANTOS unionability, by %\cref{definition:santos_unionability}
% a unionable table
% %has as many attributes with the same relations as the query table. 
% only requires a single matching relationship between query and candidate table.
%each attribute's semantic type and relationship's confidence score. \roee{We may want to refer here to the trade-off between higher number of matching triples and the quality of each triple matching explicitly. Again, I think we need to do that once we fix the unionability and problem definition. My suggestion is to define that a query table and a data lake table are SANTOS unionable if they have the same intent/subject column and at least one of its properties. Then in the problem definition say that we aim to find the \intent column and a maximal amount of properties. Now, when we get to this section we refer to the trade-off that is created based on the quality of the matching subject and properties.} 
Ideally, we would like to rank candidate tables with more shared relationships higher, but this does not consider confidence scores, as well as attention to granularities. 
%\rjm{10/31: IMPORTANT example:tbw is missing!!!}
%aamod: resolved by using example 14.
For instance, considering \cref{example:column_semantics},
%\zixuan{This example is confusing. (place-geo, 1.0) is there but place-geo is not a triple.}, 
we cannot count the contribution of 
\texttt{city} and \texttt{country} equally as they have confidence scores of $0.6 * 0.2115$ and $0.2 * 0.2712$, respectively. 
Thus, we want to 
%rjm
balance the number of relationships matched with their confidence.
%find the probability and confidence that the semantic types and relationships in the query table triples are found in the data lake table.

% To do so, we find the probability that the data lake table 
%rjm triple 
%contains a column that matches the query table's subject column's semantic (same column semantics) and relations that match the relations in the query semantic tree.
%rjm property column's semantic type, and relationship between the two columns. 
%Recall that, based on \cref{definition:santos_unionability}, even if we only find one matching relation in a table (i.e., matching subject and at least one relationship), we consider that table unionable. 
%However, based on our problem definition, our scoring function should also capture the notion that a table has a higher unionability score if it has a higher number of matches.
%Thus, we find the sum of matching probabilities of each $RS(c_1c_2)$ and ranked the table using the sum.
%\wolf{10/21: So here, there a number of design decisions for the scoring functions, which may not be well justified. 
%In the formal setup, it maybe good to distinguish between:
%1. the parts of the framework that are generic steps that rely on certain quantified metrics that capture some goal,
%2. and particular design choices that quantify that intuition into one (exchangeable) metric}

% \subsection{Unionability Scoring Function}
% We search the inverted index using the query table's triples to find the matching data lake table triples. 
% We want to see how likely it is to find each query table's triple in the data lake table's triples.
% First, we compute the match score between the pair of triples from the query table and the data lake table. Once we get the match score for each triple pair, we combine them to get the final ranking score. As our definition says, we want the data lake table to have as many columns with same relations from the query table as possible. This is monotonically related with the number of triples. Therefore, we find the set containment of Query table's triple set in the Data lake table's triple set. Higher the number of query triples that are contained in the data lake table triples, better is the unionability score. However, we cannot rely only on the number of the triples because the confidence score for each triple can be different. For instance, considering triples from \cref{example:tbw}, we cannot count the contribution of 
% $physicist-hasOccupation-profession$ and $place-birthPlace-person$ equally as the former has a confidence score of 0.166 and the later has that of 1.0. Therefore, instead of using the normal set containment, we use weighted set containment where, the weight comes from the confidence score for each triple.

% My intention is to first describe how we compute the scores for each triple i.e., multiplying the column semantics and relation semantics scores. After that, I thought of explaining how we compute the matching score between each triple pair i.e., by multiplying the individual triple scores. Finally, we find 

%\rjm{10/31:  the triple section was removed, please update this to reflect the new definitions of column semantics and relation/ship semantics}
%\aamod{11/1: Updated!}

% To this end, we formally define SANTOS scoring based on %3 components:
% the following three components:
% (1) relationship semantics confidence score (RS$_{\textsc{Conf}}$) (see \cref{subsection:relation_semantics}),
% (2) relationship-matching score, and (3) unionability score.
% Let $Q$ be a query table with \intent column $I$ and semantics $CS(I)$. 
% Assume $Q$ has $m$ relationships with $I$, with scores
% $RS_{\textsc{Conf}}(Q.I,p_{IP_1}, Q.P_1)$, \ldots, $RS_{\textsc{Conf}}(Q.I, p_{IP_m}, Q.P_m)$ that best match with the 
% relationships in candidate table $D$ with scores
% $RS_{\textsc{Conf}}(D.c, p_{cc_1}, D.c_1)$, \ldots, $RS_{\textsc{Conf}}(D.c, p_{cc_m}, D.c_m)$. 
% % \grace{3/21: Is this different from \cref{def:rscs}?
% % \aamod{They are the same.}
% % }

% The \emph{relationship-based} score for each RS$_{\textsc{Conf}}$ of $Q$ (similarly for RS$_{\textsc{Conf}}$ of $D$) is given by,
% \begin{multline}
%     RS_{\textsc{Conf}}(Q.I, p_{I P_i}, Q.P_i) = CS_{\textsc{Conf}}(Q.I, CS(Q.I)) \\
%     \cdot RS_p(Q.I, p_{I P_i}, Q.P_i) \cdot CS_{\textsc{Conf}}(Q.P_i, CS(Q.P_i))  
% \end{multline}\noindent where $CS_{\textsc{Conf}}(Q.I, CS(Q.I))$ and $CS_{\textsc{Conf}}(Q.P_i, CS(Q.P_i))$ are column semantics confidence score for the intent and property column semantics, and $RS_p(Q.I, p_{I P_i}, Q.P_i)$ is the Relationship Predicate Confidence Score (see \cref{section:unionability_components}). 

% \grace{3/21: Substitute for the above explanation for relationship-based score:}
% \updated{
% To this end, we formally define SANTOS scoring based on 3 components:
% Relationship semantics confidence score (RS$_{\textsc{Conf}}$) (see \cref{subsection:relation_semantics}),
% relationship-matching score, and unionability score.
% Here, RS$_{\textsc{Conf}}$ follows the same logic as RS$_{\textsc{Conf}}$ (\cref{def:rscs}), but it only finds scores between relationships formed with the query table's \intent column, $Q.I$, where $CS_{\textsc{Conf}}(c_i, t_i)$ is $CS_{\textsc{Conf}}(Q.I, CS(Q.I))$ in the equation.}

To this end, we formally define SANTOS scoring based on the following three components:
(1) relationship semantics confidence score (RS$_{\textsc{Conf}}$) (see \cref{subsection:relation_semantics}), (2) relationship-matching score, and (3) unionability score.
RS$_{\textsc{Conf}}$ of a query table Q  is computed based on \cref{def:rscs}, finding scores between relationships formed with the query table's \intent column, $Q.I$, where $CS_{\textsc{Conf}}(c_i, t_i)$ is $CS_{\textsc{Conf}}(Q.I, CS(Q.I))$ in the definition.

\introparagraph{Relationship-matching Score:} Using RS$_{\textsc{Conf}}$, we compute the relationship-matching score for each matching relationship, between the relationship formed from query table's intent column ($Q.I$) and some property column ($Q.P_i$) with the relationship formed from a data-lake table's columns, $D.c$ and $D.c_j$ as
\begin{multline}
    \mathrm{matchScore}(RS_{\textsc{Conf}}(Q.I, p_{I P_i}, Q.P_i), RS_{\textsc{Conf}}(D.c, p_{c c_j}, D.c_j)) = \\
    RS_{\textsc{Conf}}(Q.I, p_{I P_i}, Q.P_j) \cdot RS_{\textsc{Conf}}(D.c, p_{c c_j}, D.c_j)
\end{multline}

\begin{example}
\label{example:inverted_index}
For instance in \cref{example:rscs} (table(c) of \cref{fig:running_examples}), let the
$RS_{\textsc{Conf}}$ value 0.0203 is stored in the inverted index in the value component for semantic relationship
\texttt{(person, birthplace, city)}.
%as shown in \cref{fig:indexes}
If a query table also has \texttt{(person, birthplace, city)} as one of its semantics, we compute the match score by multiplying two $RS_{\textsc{Conf}}$.
\grace{3/21: TODO: Update example. If we don't include an inverted index in section 3, should we form the example around a synthesized relationship from section 5?}
\aamod{3/21: let's assume we have an inverted index. Or we can use synth relationship too.}
\end{example}

%Using the triple-based score of a query table triple $Qs_{i}$ and a data lake table $Ds_{i}$ we can compute the \emph{triple-matching score} as follows
% \begin{equation}
%     s_{matching}(Qs_{i}, Ds_{i}) = s_{triple}(Qs_{i})\cdot s_{triple}(Ds_{i})
% \end{equation}
\introparagraph{Unionability Score:} Finally, these match scores are used to compute the \emph{unionability score} between $Q$ and $D$ as:
\begin{multline}
\label{eq:unionability_score}
    s_\mathrm{unionability}(Q, D) = \\\sum_{i,j = 1}^m \mathrm{matchScore}(RS_{\textsc{Conf}}(Q.I, p_{I P_i}, Q.P_i) \cdot RS_{\textsc{Conf}}(D.c, p_{c c_j}, D.c_j))
\end{multline}\noindent 
%where $Z$ is a normalization factor. In this work we set $Z=|\{Qs_{i}| s_{triple}(Qs_{i}) > 0\}_{i=1}^{m}|$, i.e., the number of query table triples with a non-zero triple-based score.\footnote{Note that since $Z$ considers only the query table triples, it does not change the ranking induced by unionability score}
In order to reduce computation cost at query time, notice in \cref{eq:unionability_score} that we calculate RS$_{\textsc{Conf}}$ for each data lake table during pre-processing and store them to the inverted index. 
%(\cref{fig:indexes}). 
At query time, we find RS$_{\textsc{Conf}}$ for query tables and compute the unionability score.
Intuitively, \cref{eq:unionability_score} addresses the trade-off between the number of matching relationships and the quality of their match in its computation. Higher matching quality is captured by the individual matching scores while the number of matches is addressed by the summation of such scores.
%\updated{below}
%\roee{The next definition should define the problem and not the state the solution ("ranked using the scores given by ${s_\mathrm{unionability}(Q, D_i)}$"). The final sentence may be replaced by something like: "... ranked by their *likelihood* [(replace by the property which the scoring function seeks)]of being unionable with $Q$"}
%\roee{Also, why do we need the intent column and the Knowledge Base for the definition?}
%\aamod{02/20: I agree. I am trying to make the definition precise. If we add unionable, we may have to define that again. I think mentioning the scoring function itself in the definition makes it clearer. I agree with KB part too, I removed that from the definition.}
\begin{definition}[Top-k SANTOS-Unionable Table Search]
\label{definition:santos_ranking}
Given a Query Table $Q$, the intent column of $Q$, $Q.I$, a set of Data lake tables $\mathcal{D}$,
%Knowledge Base $\mathcal{K}$,
a scoring function ${s_\mathrm{unionability}(Q, D)}$
and an integer $k$, the Top-k SANTOS-Unionable Table Search is to find the top-k Data lake tables $D_1$, $D_2$, $\dots$, $D_k \in \mathcal D$ that are
%SANTOS-Unionable with $Q$ and 
ranked using the scores given by ${s_\mathrm{unionability}(Q, D_i)}$.
\end{definition}

\grace{ I believe we need a concrete explanation / definition somewhere, whether in the top-k table search definition or elsewhere, that explains SANTOS-unionability and how it's different from other unionability definitions. When we reference it in the beginning of Section 7, or when other works cite our SANTOS-unionability formalization, it shouldn't be based on our scoring function. It should explain concretely what SANTOS-unionability means. This way, other works can easily use our unionability definition in their new approach, or even use it for other problems like joinable table search.

---

Given a query table $Q$ with a specified intent column $Q.I$, and a set of data-lake tables $\mathcal{D}$, we aim to find SANTOS-Unionable Tables from $\mathcal{D}$ that have the maximum number of relationships shared with $Q$ such that each matched relationship has a high confidence score, where the relationships are formed from $Q.I$ to the remaining property columns.

\begin{definition}[\textit{Alternative} SANTOS-Unionable
 Table Search]
\label{definition:santos_ranking}
To perform top-$k$ SANTOS-unionable table search, we find $k$ tables that have the maximum unionability scores, which is defined by \cref{eq:unionability_score}.
\end{definition}
}

\roee{
\begin{definition}[\textit{Yet another} Top-k Unionable Table Search]
\label{definition:santos_ranking}
Let $Q$ be a query table with an intent column $Q.I$, $\mathcal{D}$ be set of Data lake tables and $s_\mathrm{unionability}(Q, D)$ be a scoring function. Given $k\in \mathbb{N}$, the Top-k Unionable Table Search problem is to find $k$ tables in $\mathcal{D}$ with the highest score ${s_\mathrm{unionability}(Q, D)}$.
%$s(Q, D)$.
\end{definition}
}


Note that unionability between two tables is often viewed as a binary decision i.e., either the tables are unionable or not.
%unionable~\cite{}. 
In a traditional database setting, two tables are unionable if and only if they have compatible schemata.\footnote{one might also pre-process the tables for compatibility, for example, project out columns or rename attribute names}
% Ideally, two unionable tables do not only have exactly the same schema but also same relationships.
% In a data lake setting, which we follow in this work, due to heterogeneous nature, such strict constraints leads to a large amount of false negatives, or in other words a low recall while searching for the unionable tables. This is why, we relax these constraints and define a more realistic setting for data lakes.
%we formulate the unionability as a ranking problem. 
% Existing works~\cite{nargesian_18_TUS, 2020_bogatu_d3l} relax the unionability definition even further as they do not consider the relationships between attributes in the table.%modeled by pairs of attributes in a table and 
%  This, in turn, may lead to false positives as discussed in \cref{example:intent_column_importance}. In what follows, the main motivation of the newly suggested definition is to also consider such relationships. We will show the effectiveness of relationships and the importance of new definition empirically in \cref{section:experiments}.
%  \grace{3/21: The last two paragraphs: is this too repetitive with the related work / beginning? Rewrite below:}
%  \aamod{I think we need this in some way because last time also reviewers never noticed that previous approaches consider the match between just one column. We need to explain why one intent and one more property is enough. These paragraphs are about the same.}
In the data-lake setting, the constraint of aligning a unionable table's schema exactly with that of a query table is not practical. Existing works~\cite{nargesian_18_TUS, 2020_bogatu_d3l} have relaxed this in their unionability definitions. However, they solely consider column unionability without considering the relationships and the preservation of the query table's topics. Thus, by introducing SANTOS-unionability, we aim to show the importance of considering relationships when searching for unionable tables that share the same intent as the query table. Next, we empirically show the effectiveness of relationships and the importance of new definition.
 %This is the main motivation behind our new definition. 
% Note that,  \cref{definition:santos_unionability} sets the minimal conditions for unionability as we envision it and is used to shortlist the candidate data lake tables wrt to a query table.
% After this step, we use a scoring function (\cref{eq:unionability_score}) that considers column/relationship semantics match and confidence scores to rank how unionable the shortlisted data lake tables are. Therefore, a table fulfilling the minimum condition still may not exist in the top-k ranking if there are other better tables. We will define top-k SANTOS-Unionable Table Search problem and related scoring function in details in \cref{section:semantic_union_search}. 


% % \roee{\textbf{OLD}: Let us consider that m triples from a Query Table Q's triple set are contained in the data lake table D's triple set. Let
% % $(qs_1, ds_1)$, $(qs_2, ds_2)$ \dots $(qs_m, ds_m)$
% % be the pair of confidence scores for the matching triples.
% % Let, n be the total number of query table's triples with confidence score greater than 0 where, $m \leq n$. 
% % The unionabilty score between Tables Q and D is given by:

% \begin{equation}
%     Unionability(Q, D) = \frac{\sum_{i = 1}^m qs_i * ds_i}{n}
% \end{equation}
% }
% \aamod{10/20: I am sorry for abusing some notations like m, n in this section. I will update to make everything consistent from the beginning.}

==> sections/synthetic_KB.tex <==
\section{Synthesized Knowledge Bases}\label{section:synthetic_knowledge_base_old}
% \aamod{10/31: Using synthesized knowledge base instead of synthetic knowledge base}

%\wolf{11/1: replacing textit and em with emph}
%\aamod{sure, thanks!}
% \wolf{11/1: replacing occasional use of texttt with standard text (because sometimes it was used, sometimes not)}
% \wolf{11/1: I see inconsistent use of relation vs relationships and did not change in my pass}

    % \begin{figure*}[h]
    %   \includegraphics[scale = 0.5]{figures/synthetic_kb.pdf}
    %   \caption{Creation of synthesized knowledge base to capture the column relationships. The data lake tables are about museums and their location. Only column values are given and the knowledge base is not available. The synthesized relationships (\texttt{A\_B, C\_D} and \texttt{E\_F}) are assigned to the column pairs in Table 1. Table 2 and Table 3 respectively. Ranking in query phase is based on \cref{eq:unionabilty_score}}
    % \label{fig:synthetic_kb}
    % \end{figure*}

% \begin{figure*}[h]
%   \includegraphics[scale = 0.53]{figures/Fig_synthetic_kb}
%   \caption{Creation of synthesized knowledge base to capture the column relationships. The data lake tables are about museums and their location. Only column values are given and the knowledge base is not available. The synthesized relationships (\texttt{A\_B, C\_D} and \texttt{E\_F}) are assigned to the column pairs in Table 1. Table 2 and Table 3 respectively. Ranking in query phase is based on \cref{eq:unionability_score}. Note that here we only have a pair of columns. For more column pairs, we compute the score in same way for each pair and integrate using \cref{eq:unionability_score}.}
% \label{fig:synthetic_kb}
% \end{figure*}

% \begin{table}[t]
% \caption{Example tables for synthetic knowledge base creation}
% \label{tab:synth_kb_tables}
% \begin{tabular}{ccl}
% \toprule
% $A_1$ & \dots \\
% \midrule
% a & \dots\\
% b & \dots\\
% c & \dots\\
% d & \dots\\
% e & \dots\\
% \bottomrule
% \end{tabular}
% \hspace{3em}
% \begin{tabular}{cl}
% \toprule
% $B_1$ & \dots\\
% \midrule
% c & \dots\\
% d & \dots\\
% e & \dots\\
% f & \dots\\
% \bottomrule
% \end{tabular}\end{table}


% \begin{table}[t]
% \caption{\wolf{10/21: I suggest to use tables that make it a bit more explicit that those are relational tables with explicitly delineated cells. Among the two below, the left one I think strikes the right balance:}
% \aamod{10/21: I agree! Actually, these are only the placeholder tables, I will remove them and use intuitive examples.}
% }
% % \label{tab:synth_kb_tables}
% \begin{tabular}{|c|c|l|}
% \hline
% $A_1$ & \dots \\
% \hline
% a & \dots\\
% b & \dots\\
% c & \dots\\
% d & \dots\\
% e & \dots\\
% \hline
% \end{tabular}
% \hspace{3em}
% \begin{tabular}{|c|l|}
% \hline
% $B_1$ & \dots\\
% \hline
% c & \dots\\
% \hline
% d & \dots\\
% \hline
% e & \dots\\
% \hline
% f & \dots\\
% \hline
% \end{tabular}
% \end{table}

%rjm: added
Knowledge bases (KBs) may have limited coverage
of data values found in real data lakes.
Hence, using an existing KB (even a set of KBs) as the only source for finding column and relationship semantics 
% in unionability search
can lead to low coverage (recall).  
%Generic and pre-populated knowledge base may not contain data lake entities and their relationship.
%This, in turn, can impact the efficacy of our technique as we may not get enough edges for the semantic graph.
To solve this problem, we propose a novel 
data-driven approach for creating KBs from the actual data lake tables. 
We thus call the resulting KB a \emph{synthesized knowledge base}.
% , that is a KB that is created from the data lake itself.
%rjm resolved
%\wolf{10/21: ``using the very data lake tables we are also using to expand the query table. We call this approach `data lake synthesized knowledge bases' [or something more fancy, it warrants a short discussion as this is quite innovative and may go beyond the way people normally think about knowledge base].'' }
Our goal is to assign a
\emph{synthesized semantic relationship}
to those column pairs within a data lake table having a relationship that is not covered by a KB. We do it in a way
that fits our overall unionability framework. 
Intuitively, we will create a synthesized KB of 
%types and 
\emph{unnamed binary relationships} that can be used like a regular KB relationship, 
even if we don't know their names.
%of these
%types or 
%relations.  
%We will also not create a type hierarchy over synthetic types.
% For convenience, we ignore the type hierarchy and conceptually, only assign \emph{Top Level Types}.


To create a synthesized KB, we start by assuming that all the \emph{value pairs} in a \emph{column pair} 
%with a functional dependency
% \wolf{11/1: ``with a function dependency'' or ``of interst'' [because not every pair is considered; please choose here the formulation that fits the remainder]}
have the same semantic relationship 
%\wolf{11/1: is it `relationship' or `relation'?}
between them. 
%value pairs of the columns from two columns are of same semantic type inherently.
For example, consider the table of \cref{fig:relation_parks_films}:
%the value pairs of column pair \texttt{Film Title} and \texttt{Film Director} i.e.,
The tuples in $\Pi_{\mathrm{Film Title, Film Director}}$ (e.g., 
\textrm{\{Bee Movie, Simon J. Smith\}}, \textrm{\{Coco, Pixar\}}), 
should have the same semantic meaning (relationship)
%\wolf{11/1: `relationship' or `relation'}
, in this case, \textit{directedBy}.
%\wolf{11/1: `\textit{directedBy}' []Just a quick check for Zixuan. Are trriples usually declared in that way?
%Thus if the arrow points from film to the director, then is the relationship name either
%1) `directedBy' or 2) `directorOf'?]}
%rjm done
%\aamod{10/30: Can we write above example as a projection of two columns or something more clearly?}
% \wolf{10/21: semantic meaning or just type. I am a bit confused about the use of semantics for a single column without reference to the context, thus other columns}
%However, our assumption can be violated due to co-existence of \textit{property column pairs}.
As we have discussed however, some binary relationships are not meaningful without additional contextual information and are rather indirect.
%\wolf{11/1: `some binary relationships are not meaningful without additional contextual information, and are thus \emph{not} relevant binary relationships.'}
For example, the \emph{value pairs} in 
$\Pi_{\mathrm{Film Title, Park Location}}$ 
(e.g., \textrm{\{Bee Movie, 6748 N. Sacramento Ave.\}}, \textrm{\{Coco, 5210 W. $64^{\mathrm{th}}$ St.\}}) 
%in \textit{column pairs} \texttt{Film Title} and \texttt{Park Location} 
in \cref{fig:relation_parks_films} have a tenuous relationship at best (film was shown in a park with this address).
%do not have any semantic relationship between them. 
Hence, when constructing the synthesized KB, we will
%Hence, we revise our assumption and state that the \textit{value pairs} between the "related" \textit{column pairs} have same semantic relationship.
%Now in absence of knowledge base, we 
only consider
%\wolf{11/1: `only consider'}
columns that are \emph{in a functional relationship} (thus the value in one column functionally determines the value in the other column).  
For example, the \textrm{ParkName} functionally determines the \textrm{ParkLocation} 
indicating a possible semantic relationship (even if the KB does not contain \textit{parkLocations}).  
%rjm added 10/31
Our hypothesis is that column pairs in a functional relationship are more likely to contain an interesting relationship that also exists in other tables and is useful in union search. 
This has the benefit of limiting the number of column pairs we analyze, 
yet has the potential downside of missing many-many relationships 
(like actors playing in movies) unless they are already modeled in an existing KB.  
%to each other using the second component of our relationship oracle i.e., \textit{functional dependency}.
%We assume that two columns have a relationship between them if they have a functional dependency between them in any direction.

%rjm 10/31 this is incorrect
%SANTOS uses an existing (approximate) functional dependency discovery algorithm to find \textit{property columns} that functionally depend on the user's chosen \textit{subject column} in the query table.  At query time, we also find functional dependencies from columns in data lake tables that match (meaning have the same column semantics) as the query subject column.
%\grace{10/20: we may need to change the name} and store their relationships.
SANTOS uses an existing (approximate) functional dependency (FD) 
discovery algorithm 
called FDEP~\cite{1999_flach_database_dependency_discovery} 
to find unary FDs (FDs with a single column determinant).
% Specifically, we use FDEP~\cite{1999_flach_database_dependency_discovery} to discover the functional dependencies.
%an induction algorithm of dependencies. 
%FDEP induces a set of valid FDs from a set of general dependencies by performing pairwise comparisons between all tuples. 
%The resulting set must be complete and minimal.
More precisely, we run their bottom-up variant 
that starts by considering all pairwise relationships, and checking if a given dependency satisfies or violates an FD.
Notice that since we are only considering binary relationships, we only compute unary FDs.
% (FDs where the left-hand-side is a single attribute).  
%Also notice that we only consider column pairs with an empty KB relationsho semantics.  

%rjm do we need this as we are only doing unary FDs
%Compared to other FD algorithms, FDEP is memory efficient and scales the best when a dataset has a large number of columns, which is suitable for data lake tables \cite{2015_papenbrock_fdep_comparison}.
%To solve this problem, we assume that the columns are pre-processed and the homographs and incorrect entries are removed before creating the synthetic knowledge base \cite{21_leventidis_homograph_detection}.


%\wolf{11/1: there are 3 subsections. It may be better to start here witha quick overview of teh 3 steps, but not yet discuss the actual example, which is discussed in the example box in 5.1 below}
As example, consider data lake tables (1), (2) and (3) of \cref{fig:synthetic_kb}.
All these tables are about museums and their locations 
and we discover the FDs between the given column pairs.
Unlike web tables,  data lake tables are generally large enough that we can more reliably find non-spurious FDs (meaning, FDs that are likely to hold in the domain, not just this one instance).  We show only few rows and two columns in the example tables in the figure.


%\rjm{10/31:  I agree, let's leave this out}
%\aamod{10/31: We do not have experiments for sampling. Is it good to write? However, it is doable until the deadline. I would prefer to say it in future works}
%\subsubsection{Reducing the number of value pairs in the synthesized knowledge base}
%Let there are $\mathcal{D}$ tables in the data lake having $n$ rows and $m$ columns in average.  
%If there are functional dependencies between all column pairs, the number of keys in the synthesized knowledge base is $ \mathcal O [\mathcal{D} m^2 n]$. To reduce this number, we propose a sampling strategy where, we sample a number of rows in each data lake table and create the synthesized knowledge base based on the sampled data.
%In our experiments, SANTOS scaled well and therefore, we create the synthesized knowledge base without using this optimization.

%resolved!
%\rjm{I don't think I understand.  Is the assumption that the KB doesn't know about museums?  Why are we assuming FDs?  I thought we were discoverying if there is an FD?}
%\aamod{10/30: updated! we discover FD. Yes, we assume that the KB is not available or is not covering the entities in this case. Shall we update example to something that is really not found?}

\subsection{Synthesized Relationship}

We start by assigning each functionally
dependent column pair in the data lake tables with a unique synthesized relationship.
%rjm repetitive
%For instance, we assigned synthesized relations \texttt{A\_B}, \texttt{C\_D} and \texttt{E\_F} to the column pairs of Table 1, Table 2 and Table 3 in \cref{fig:synthetic_kb} respectively.

\begin{example}\label{ex:synKB}
%Here, \texttt{Title} from (a), \texttt{Name} from (b) and \texttt{Museum} from (d) are all about the museums. 
% Let us consider columns $A_1$ and $B_1$ in \cref{tab:synth_kb_tables} as an example. 
% \wolf{10/21: one table or two tables? I think replacing all table environments with figure environments will make the references and the paper reading simpler}
%rjm:  saying this in fewer words
%Using our assumption and 
%considering absence of the knowledge base, 
Consider the table fragments 1, 2, 3 in the left of \cref{fig:synthetic_kb}.
Assume no relationship was found in the KB for any of these table fragments, and that there is an FD in each.
%we first assume the tuples within a table represent a single semantic relationship.
%the \textit{value pairs} \{\emph{Freud Museum, Camden}\}, \{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\} from Table (1) have same semantic relationship.
%Similarly, the column value pairs from Table (2) i.e., \{\emph{Wallace Collection, City of Westminster}\}, \{\emph{Wellcome Collection, Camden}\} and \{\emph{Greenwich Heritage, Greenwich}\} also have same semantic relationship. 
We first give a synthetic name to each relationship (e.g., A\_B) and store the value pairs in a synthesized lookup dictionary (middle top of figure).
Note that, if \textit{value pair} belongs to two (or more) column pairs, it will be assigned  two (or more) synthesized relationships.
For example, the \textit{value pair} \{\emph{Wellcome Collection, Camden}\} has \texttt{A\_B} and \texttt{C\_D} as synthesized relationships.
%Furthermore, the overlap between A\_B and C\_D hints that these might be the same relationship.  In this example,  \{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\} appear in both tables.
%Therefore, using transitive closure, we can say that \{\emph{Freud Museum, Camden}\} and \{\emph{Greenwich Heritage, Greenwich}\} should also be of same semantic relationship even though they are not under the same \textit{column pair}.
%Rather than creating a unique synthetic relation for each column pair, we discuss below how relations might be combined. 
%Hence, we design a probabilistic model that assigns each \textit{value pair} a score for each synthetic relationship.
%\wolf{10/21: so here I cannot follow because of the notation. a column of cities can have the semantic type "birth place" as predicate or be just be "towns" if a subject column. Shouldn't the use of the word "semantics" be restricted to when relations come into play?}
%\aamod{10/26: We call that relationship semantics. Next option is column Semantics. If we look from types vs properties, semantic types are related to columns and  properties are related to the relationship between the columns.}
\end{example}
%\wolf{11/1: shouldn't this be `relationships' instead of `relations'?}
%aamod: resolved

%rjm not sure "transitive closure" is good description
%However, one should be careful in deciding how similar they are and how far shall we go using the transitive closure.
%For this, we design a probabilistic model that assigns each \textit{value pair} with a score for each synthetic relationship.
%In summary, we assume that every \textit{value pairs} are likely to be of all semantic types we assigned.

%\subsection{Assigning synthesized relationship}
%Considering above concepts, we start creating the synthesized knowledge base by assigning each functionally
%dependent column pairs in the data lake tables with a unique synthesized relationship.
%For instance, we assigned synthesized relationships \texttt{A\_B}, \texttt{C\_D} and \texttt{E\_F} to the column pairs of Table 1, Table 2 and Table 3 in \cref{fig:synthetic_kb} respectively.


%Apart from direct assignment as discussed above, we use the transitive closure to assign the semantic relationship.

%\rjm{I think this is all said already, I suggest removing it and calling the lookup table a "Synthesized relation dictionary" to use the same terminology as in KB section.}
%
%\subsection{Lookup Table Creation}
%Next, using our assumption, we assign each \textit{value pair} with a synthesized relationship that is assigned to its respective \textit{column pair}. For example,  \{\emph{Freud Museum} and \emph{Camden}\} are considered to have a synthesized relationship \texttt{A\_B}.
%We record the synthesized relationship provided to each \emph{value pair} in Lookup Index. Note that, if \textit{value pair} belongs to two (or more) column pairs, it will be assigned with two (or more) synthesized relationship.
%For example, the \textit{value pair} \{\emph{Wellcome Collection, Camden}\} has \texttt{A\_B} and \texttt{C\_D} as synthesized relationships.
%Recall that we are using co-occurrence information between the value pairs to determine if the column pairs have same relationship. 
%To do so, we need to know where each \textit{value pair} exist.
%The \textit{lookup index} records the \textit{value pairs} as key and the list of their synthesized relationships as value as shown in \cref{fig:synthetic_kb}.
%Lookup index works like \textit{relation dictionary} in \cref{section:unionability_components}.

%\wolf{10/21: Interesting. Do you see a conceptual connection to a topic model? The topics here are all the column, and each word gets a stochastic vector assignment to topics. The unusual connection is that a column in your model is both a topic and a text document *at the same time*. Would you agree? If yes, you could make the connection and also use a lot of the notation from topic models. 
%interestingly, you just have a binary graph instead of a ternary graph as in topic models :)}
%\aamod{10/30: I tried to explore that but I am sorry that I am not able to use that to describe synthetic kb.}

\subsection{Creating Lookup Relationship Dictionary}
As we do not have a knowledge base available to process the data lake tables, we go through all of them and record the value overlap in a lookup relationship dictionary. The lookup dictionary records the occurrence of each value pair in the data lake. For instance, in \cref{fig:synthetic_kb}, 
as the pair
(wallace collection, city of westminster) 
% \{\emph{wallace collection\_\_city of westminster}\} 
appears in two column pairs,
thus the lookup relationship dictionary records 
the pair
% \{\emph{wallace collection\_\_city of westminster}\} 
as a key for two values:
\textit{A\_B} and \textit{C\_D}.\footnote{Notice that we normalize capitalization to lower case.}
\subsection{Processing Data Lake Tables}
Once we create this lookup relationship dictionary, we use it similar to the \textit{relationship dictionary} (\cref{section:unionability_components}) to process the data lake tables. Note that, lookup index is only for processing the data lake tables and we do not need it at query time. For query time, we create the
%lookup index, 
synthesized relationship dictionary and use it similar to the KB \textit{relationship dictionary}. It has same keys as the lookup relationship dictionary but updated values that captures the co-occurrence. Note that the values in synthesized relationship dictionary is updated after processing each column pair.
%as a synthesized knowledge base to get the relationship between the column pairs in the data lake table.
%at query time, just as we use the KB relation dictionary, however, 
%Also, we use the synthesized relationship dictionary only for column pairs with an empty relationship semantics.  
%For each value pair, we search the lookup index and get the synthesized relationships.

\begin{example}
For example, suppose we are processing Table 1 of \cref{fig:synthetic_kb} as data lake table after creation of lookup relationship dictionary. All three values have synthesized relationship \texttt{A\_B} as they belong to the same column pair. Here, \{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\} also have synthesized relationship \texttt{C\_D}.
Therefore, we assign both \texttt{A\_B} and \texttt{C\_D} as the synthesized relationship (that is, the \emph{ synthesized relationship semantics} (synthesized RS)) with a confidence score which is the fraction of unique value pairs mapped in the synthesized RS to the total number of unique value pairs in the column pairs. For example in Table 1 of \cref{fig:synthetic_kb}, the confidence score for \texttt{A\_B} is 1.0 and \texttt{C\_D} is 0.66.  With these confidence scores we define the Synthesized RSCS.
\end{example}
Once we find the synthesized relationship for data lake tables (shown below each table in the example), we also need to record the data lake tables containing those relations. This helps us to find them quickly during the query phase.
Therefore, we use an inverted index having the synthesized relationship as key and the tuple of \textit{(table name, column pair index, confidence score)} as value as shown in \textit{Synthesized Inverted Index} of \cref{fig:synthetic_kb}.
%Synthetic inverted index, synthetic relation dictionary and lookup index are three different things. Lookup table captures the overlap between the values and we use lookup index as a knowledge base for the data lake tables. Using lookup relation index, we create the synthetic relation dictionary that we use for the query tables.

%As we assume that the \textit{value pairs} in same column pair (eg.\{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\} ) should have same semantic relationships, we add each \textit{value pair} as a key and the synthesized semantics assigned to the \textit{column pair} as its value to the \textit{synthesized knowledge base} as shown in \cref{fig:synthetic_kb}.

%aamod: resolved
%\rjm{10/31:  This needs to be made analogous to the KB.  Where is the RSCS?}
% aamod : The above sentence is about the inverted index that we use during the query time to search for the data lake tables.

%\aamod{10/31: A\_B, C\_D and E\_F are Relationship semantics (RS). RSCS(A, B, A\_B) is stored in the syntesized inverted index. For example: for table1's column pair 0\_1, 1.0 is the confidence score. Synthesized relationship dictionary is analogous to the relationship dictionary. We also have inverted index for yago part where we store RSCS as the key and the tables and columns containing them as a value.}
We follow the same procedure for all data lake tables and update the synthesized inverted index and synthesized relationship dictionary. 
%Also, if a \textit{value pair} in the synthesized knowledge base gets a synthesized relationship that already exists as its value, it updates the confidence score with maximum of new confidence score and old confidence score.

%\rjm{10/31: above sentence makes no logical sense in English.  How can a value pair have a relationship as its value? I don't understand.}
%aamod : Resolved. It seems like off-the-context here.
%\aamod{10/31: Like in relation dictionary, we have entity pairs as a key and the relationship between them as a value, similarly, we have value pairs (eg. freud museum\_\_camden) are keys and their synthetic relationships, eg. A\_B as values.}
\begin{example}
Let us consider data lake tables in \cref{fig:synthetic_kb} as an example. 
After the processing of Table 1, the synthesized KB contains the following three keys:  \emph{freud museum\_\_camden}, \emph{wallace collection\_\_city of westminster} and \emph{wellcome collection\_\_camden}. All of them have value: \{A\_B: 1.0, C\_D: 0.66\}.  After processing the second table, we get greater value of C\_D (1.0) for \emph{wallace collection\_\_city of westminster} and \emph{wellcome collection\_\_camden} than before (0.66). 
%rjm get an update on their values. 
%are updated.
Therefore, the values of both of them in synthesized relationship dictionary change to: \{A\_B: 1.0, C\_D: 1.0, E\_F: 0.33\}. Also, greenwich heritage\_\_greenwich is added to the synthesized knowledge base with value: \{A\_B: 0.66, C\_D: 1.0, E\_F: 0.33\}. Similarly, after processing Table 3, the synthesized knowledge base contains the keys and values as shown in the figure. We can see that \emph{freud museum} and \emph{camden} from Table 1 are not in Table 2. Still our algorithm is able to capture that they also have a semantic relationship with Table 2.
%However, by using our transitive closure, we provide them with a synthesized semantic type from Table 2.
%\rjm{10/31:  what is "our transitive closure".  Define this formally.  Or leave this out if it is a minor detail.  I suggest the latter given that we don't have time to introduce new concepts this late. }
%\aamod{10/31: Yes, that just means co-occurrence with neighbooring tables. It's a minor detail. Removed}
After processing all data lake tables, we store the synthesized knowledge base and synthesized relationship index which are both used during the query phase. 
\end{example}
%We use the synthesized knowledge base 
%rjmas a backup to YAGO during the query phase.
%for column pairs with no KB relationship semantics.
In Query phase, we use \textit{Synthesized relationship dictionary} to find the relationship between the column pairs like we do in \cref{subsection:relation_semantics} using the regular knowledge base. For example, for Query table in \cref{fig:synthetic_kb}, we find two value pairs in the \textit{synthesized relationship dictionary}. Once we find the relationship semantics using all the value pairs, we average the score for each value pairs to get the relationship semantics of the column pair. Finally, we lookup the synthesized inverted index to find out the tables that are unionable with the query table. Note that, we only use one semantic relationship to match between each query and data lake table column pairs. For example, during score computation, we only used the score provided by \texttt{C\_D} although there were two semantics (also \texttt{A\_B}) matching between Query table and Table 1. Note that the example only shows the cases for a single column pair. We repeat the same procedure for each column pair and finally aggregate them using the scoring function (\cref{eq:unionability_score}) which we will discuss in \cref{section:semantic_union_search}.
%\rjm{10/31:  do you mean Query Processing?  I also suggest removing the entire subsection below.  Above you defined Synthesized KB "procedurally", you don't need an opaque declarative definition.}
%\aamod{10/31:  Agree!}

% \subsection{Processing Query Table}
% %\aamod{10/30:  May be we need to move it to next section}
% Let us continue with our assumption that a knowledge base is unavailable and user provides us with a query table and a subject column marked on it. Now we use the synthesized knowledge base that we created during the offline phase to get the synthesized relationship between the subject column and property columns. As shown in \cref{fig:synthetic_kb}, we lookup each \textit{value pair} in the synthesized knowledge base and find the synthesized relationships. In this example, we find the value pairs \textit{Salar Jung Museum} and \textit{Hyderabad} in the synthesized knowledge base. As done in the data lake tables, we compute the confidence score for each synthesized relationship. Then we search each synthesized relationship to search the synthesized inverted index and find all the tables that have at least one synthetic semantics matching with the query table. Finally we use our ranking function \cref{eq:unionabilty_score} to rank the unionable tables.
% % \aamod{10/31: I feel it would have been easier to explain with an algorithm and going through the running examples.}
% % \aamod{10/30: Leaving the definition here. I am not sure where to move it, may be after section 5.1?}
% % \begin{definition}[Synthetic KB]
% % If \{$A_1 B_1$, $A_2 B_2 \dots$ ,$A_pB_p$\} $\in \mathcal W_D$ are the unique column pairs having a functional dependency, \{$A_1\_B_1$, $A_2\_B_2 \dots $ ,$A_p\_B_p$\} are the respective synthesized relationships assigned to them and
% % \{$a_1b_1$, $a_2b_2$ \dots $a_qb_q$\} $\in \mathcal U_D$ are the unique column value pairs
% % % \wolf{10/21: I could not follow when reading. Only later realized you mean the A's are the column of type text?}
% % in the entire data lake,
% % the synthesized knowledge base for the given data lake is a key-value pair having $a_i\_b_i$  for each $a_ib_i \in \mathcal U_D$ as a key and $\forall key$, a vector $(g_{i1} A_1\_B_1, g_{i2} A_2\_B_2, \dots g_{ip} A_p\_B_p)$as value.
% % \aamod{10/30: Let's say simply list instead of vector?}
% % \wolf{10/21: I am not familiar with this notation, it's like a named perspective of the entries of a vector. Is this a standard notation? Maybe, I just have not seen yet. Just in case, maybe formally mention in the early formal setup.}
% % \aamod{10/30: I tried to find some but could not fine other standard notations. For vectors, the best way is to represent with arrow over. Should we go for that?}
% % \end{definition}
% % For instance, for a data lake having column pairs \{$A_1B_1$, $A_2B_2$\} and value pairs \{$a_1b_1$, $a_2b_2$ $a_3 b_3$\} , 
% % the synthetic KB contains the key-value pairs: $\{a_1\_b_1: (g_{11} A_1 B_1, g_{12} A_2 B_2)\}$, 
% % $\{a_2\_b_2: (g_{21}A_1 B_1, g_{22}A_2 B_2\}$,
% % $\{a_3\_b_3: (g_{31}A_1 B_1 g_{32}A_2 B_2\}$ respectively.

% %Next, we will discuss how we assign values to the coefficients $\{g_{i1}, g_{i2}, \dots g_{im}\}$ step-by-step.

% %\rjm since we have a single optimization, let change name
% %\subsection{Optimization}
\subsection{Reducing the Number of Relationships}
%\aamod{10/31: trying to start positively :) ! We will move this to discussion or some other sections at the end}

The synthesized knowledge base stores: 
%mainly stores two information: 
the \textit{value pairs} and \textit{synthesized relationship semantics}. %Therefore, there are mainly two areas in which we can optimize our synthetic knowledge base.
%\subsubsection{Reducing the number of synthesized relationships}
As shown in \cref{fig:synthetic_kb}, the number of synthesized relationship is equal to the total number of \textit{column pairs} with a functional dependency between them that are not represented in the KB. However, one can merge certain relationships based on  available information. If all value pairs of a smaller column pair are contained in a large column pair, we assign both a single synthesized relationship. For example, in the absence of row \{\emph{Freud Museum, Camden}\}, we would assign a single synthesized relationship, say \texttt{C\_D}, to the column pair in Table (1) and Table (2).
A step ahead from containment, if two column pairs have high overlap between them, we can merge their synthetized relationships. Precisely, given two column pairs $c_{11} c_{12}$ and $c_{21} c_{22}$ having $n_1$ and $n_2$ $(n_1 \leq n_2)$ unique value pairs respectively. Let there are $g$ unique value pairs that appear in both column pairs. Then,
%we remove $c_{11} c_{12}$'s synthesized relationship and assign it $c_{21} c_{22}$'s synthesized relationship
if $\frac{g}{n_1} \geq \eta$, we can assign them a single synthesized relationship. Here, $\eta$ ranges from $0$ to $1$. This optimization would be applied just after the creation of lookup table in offline phase.

\begin{example}
For example, let us revisit the column pairs of Table 1 and Table 2 of \cref{fig:synthetic_kb}. We see that there are two value pairs:\{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\}
overlapping between them. If we consider $\eta = 0.66$, the column pairs in Table 1 and Table 2 will be identified with a single synthetic relationship \texttt{C\_D}.
\end{example}

%\rjm{10/31:  I agree, let's leave this out}
%\aamod{10/31: We do not have experiments for sampling. Is it good to write? However, it is doable until the deadline. I would prefer to say it in future works}
%\subsubsection{Reducing the number of value pairs in the synthesized knowledge base}
%Let there are $\mathcal{D}$ tables in the data lake having $n$ rows and $m$ columns in average.  
%If there are functional dependencies between all column pairs, the number of keys in the synthesized knowledge base is $ \mathcal O [\mathcal{D} m^2 n]$. To reduce this number, we propose a sampling strategy where, we sample a number of rows in each data lake table and create the synthesized knowledge base based on the sampled data.
%In our experiments, SANTOS scaled well and therefore, we create the synthesized knowledge base without using this optimization.

==> sections/synthetized_kb_updated.tex <==
\section{Synthesized Knowledge Bases}
\label{section:synthetic_knowledge_base}
% \updated{Aamod: I did not change old synthesized KB section and started a new section for its revision. The old section has been removed from main.tex file.}
\begin{figure*}[h]
  \includegraphics[scale = 0.52]{figures/synthesized_index.pdf}
  \caption{Data-Lake Tables and Synthesized Relationship Dictionary (S), made up of synthesized relationship types of each value-pair. Value-pairs highlighted in blue appear in Tables 1 and 2, and the value-pair highlighted in green appear in Tables 2 and 3.}
\label{fig:synthetic_kb}
\end{figure*}
% \begin{figure*}[h]
%   \includegraphics[scale = 0.53]{110821_POST_VLDB_Submission/figures/synthetic_kb.png}
%   \caption{Creation of synthesized knowledge base to capture the column relationships. The data lake tables are about museums and their location. Only column values are given and the knowledge base is not available. The synthesized relationships (\texttt{RS(A,B), RS(C,D)} and \texttt{RS(E,F)}) are assigned to the column pairs in Table 1. Table 2 and Table 3 respectively. Ranking in query phase is based on \cref{eq:unionability_score}. Note that here we only have a pair of columns. For more column pairs, we compute the score in same way for each pair and integrate using \cref{eq:unionability_score} \aamod{02/18: todo: replace png file with pdf.}}
% \label{fig:synthetic_kb}
% \end{figure*}

Knowledge bases (KBs) have limited coverage over the 
%of 
data values found in real data lakes. The types returned for columns and especially relationships tend to be sparse.
Hence, using an existing KB (even a set of KBs) as the only source for finding column and relationship semantics 
can lead to low coverage (recall). \roee{Update:} As an example, our experimental study (see Section~\ref{section:experiments}) indicate that YAGO covers only a XX\% over UK open data and XX\% over Canada open data. 
%Generic and pre-populated knowledge base may not contain data lake entities and their relationship.
%This, in turn, can impact the efficacy of our technique as we may not get enough edges for the semantic graph.
To solve this problem, we propose a novel 
data-driven approach for creating a synthesized KB using the data lake itself. %from the  data lake tables. 
This way, we can mine a data lake for column and relationship semantics, and fill in the gaps created from the existing KB.
%We thus call the resulting KB a \emph{synthesized knowledge base}.
% , that is a KB that is created from the data lake itself.
%rjm resolved
%\wolf{10/21: ``using the very data lake tables we are also using to expand the query table. We call this approach `data lake synthesized knowledge bases' [or something more fancy, it warrants a short discussion as this is quite innovative and may go beyond the way people normally think about knowledge base].'' }

Recall that we create \textit{entity dictionary, inheritance dictionary, type dictionary and relationship dictionary} using YAGO.
For synthesized KB, we directly use the cell values as entities. Hence, a synthesized entity dictionary is not needed. %we do not create \textit{synthesized entity dictionary}. 
%Also, we found the requirement of external knowledge to infer the type hierarchy. Therefore, 
To keep the synthesized KB entirely data-driven, we also do not create the inheritance dictionary, which requires an external type hierarchy. We focus primarily on the \textit{Synthesized Relationship Dictionary}. A type dictionary can also be similarly generate; yet, following our data driven approach we simply set  set the synthesized CSCS to 1 in synthesized RSCS (see Definition~\ref{def:rscs}).
%One can easily use the same technique (taking columns instead of column pairs) to create \textit{Synthesized Type Dictionary} %However, as the type hierarchy is not available and we directly work with cell values, we only create synthesized relationship dictionary and set the synthesized CSCS to 1 in synthesized RSCS. 
\grace{3/17: The paragraph above is a bit wordy, and readers can get lost trying to follow it. Can we instead say, we use the synthesized KB to mine for relationship semantics, especially considering the sparsity of the relationships returned by an external KB? Instead of talking about why we don't create the other dictionaries?} \roee{I revised the paragraph to be (much) less wordy. let me know what you think.}
%Though it may slightly impact the effectiveness due to absence of synthesized column semantics, it eliminates the computation and storage cost of \textit{Synthesized Type Dictionary} giving similar effectiveness.

We create a \textit{Synthesized Relationship Dictionary} for \textit{value-pairs} (values in a \textit{column pair}) that cannot find relationship semantics from the existing KB. For data-lake tables, and especially relationship tables made up of several entities, relationships are difficult to retrieve from the existing KB. Thus, we assign the binary relationship between the value-pair a \emph{synthesized semantic relationship}, and these relationships are stored in the synthesized relationship dictionary. We keep the structure of the dictionary consistent with the others in order to query them all in a uniform manner. Furthermore, we make sure to only store relationships between values in columns that have a unary functional dependency (further explained below). This way, the size synthesized relationship dictionary is manageable.

\roee{I think it is too early for an example here. Maybe only introduce the table and say we assume that we were not able to map the values using a standard KB:}
\begin{example}
\label{example:synth_kb_concept}
Consider the column pairs in Tables 1, 2, 3 of \cref{fig:synthetic_kb}, about parks and films shown in these parks at the same showtime on the same day. We are unable to find their relationships from an existing KB, so we store the value pairs in an inverted index, along with their synthesized relationship type and associated confidence score. Note that only one film is showing at a given park at a certain time, so these two columns form a functional dependency. Tables 1 and 2 have direct value-pair overlaps, indicating that they have similar relationship semantics. The same is seen in tables 2 and 3, with their shared value (Union Park, Black Panther). However, Tables 1 and 3 do not have an overlap, but both have overlaps with table 2, so they indirectly overlap.  
% Consider the column pairs in Table 1, Table 2 and Table 3 of \cref{fig:synthetic_kb} about 
% %rjm the 
% museums and their addresses where only a few tuples of the tables are shown. 
% Assume that columns A, C, and E are unionable, as are B, D, and F.
% %rjm this isn't true
% %These tables fulfill the SANTOS unionability definition and should be considered as unionable with each other. Although we do not have external KB available, 
% The value overlap between tuples
% %\rjm{tuples} 
% in Table 1 and Table 2 may be 
% %\rjm{may be}
% %is a good 
% an indication that they have same semantic relationship--both tables have (\textit{Wallace Collection, City of Westminster}) and (\textit{Wellcome Collection, Camden}). Similarly, Table 2 and Table 3 contain the tuples
% %have 
% %\rjm{contain the tuples} 
% (\textit{Greenwich Heritage, Greenwich}) 
% %as an overlapping value
% which may be
% %\rjm{maybe}
% %is 
% a signal that they model the same
% %\rjm{maybe} 
% %have column pairs having same 
% %\rjm{model the same} 
% semantic relationship. However, Table 1 and Table 3 do not have any overlapping values. 
% %even though they are SANTOS unionable with each other. 
% In such a scenario, we use the information in Table 2 to find a link between Table 1 and Table 3. Precisely, as Table 2 has overlapping tuples
% %rjm values 
% %\rjm{tuples}
% with both Table 1 and Table 3, this is a weaker, but good indication that Table 1 and Table 3 have the same semantic relationship although they do not have direct overlap of tuples.
% %rjm values.
% %\rjm{tuples}.
\end{example}

\renee{you've lost me here.  this makes it sound like we are processing all pairs of columns in the lake.}
Taking the observation in \cref{example:synth_kb_concept} into account, we first consider that all the \emph{value pairs} in a \emph{column pair} 
%with a functional dependency
% \wolf{11/1: ``with a function dependency'' or ``of interst'' [because not every pair is considered; please choose here the formulation that fits the remainder]}
have the same semantic relationship 
%\wolf{11/1: is it `relationship' or `relation'?}
between them. 
%value pairs of the columns from two columns are of same semantic type inherently.
%the value pairs of column pair \texttt{Film Title} and \texttt{Film Director} i.e.,
For instance, the tuples \textrm{(Brands Park, Moana)}, \textrm{(Kells Park, Spider-Man)}) and \textrm{(Eckhart Park, Avengers)} in Table 1 of \cref{fig:synthetic_kb} should have the same semantic meaning (relationship)
, in this case, \textit{containedInPlace}. \grace{3/17: I thought it was given a synthesized relationship. Why do we name it?}
%\wolf{11/1: `\textit{directedBy}' []Just a quick check for Zixuan. Are trriples usually declared in that way?
%Thus if the arrow points from film to the director, then is the relationship name either
%1) `directedBy' or 2) `directorOf'?]}
%rjm done
%\aamod{10/30: Can we write above example as a projection of two columns or something more clearly?}
% \wolf{10/21: semantic meaning or just type. I am a bit confused about the use of semantics for a single column without reference to the context, thus other columns}
%However, our assumption can be violated due to co-existence of \textit{property column pairs}.
As we have discussed however, some binary relationships are not meaningful without additional contextual information and are rather indirect.
%\wolf{11/1: `some binary relationships are not meaningful without additional contextual information, and are thus \emph{not} relevant binary relationships.'}
For example, the \emph{value pairs} in 
$\Pi_{\mathrm{Film Title, Park Location}}$ 
(e.g., \textrm{(Bee Movie, 6748 N. Sacramento Ave.)}, \textrm{(Coco, 5210 W. $64^{\mathrm{th}}$ St.)}) 
%in \textit{column pairs} \texttt{Film Title} and \texttt{Park Location} 
in \cref{fig:running_examples}(c) have a tenuous relationship at best (film was shown in a park with this address).
%do not have any semantic relationship between them. 
Hence, when constructing S, we will
%Hence, we revise our assumption and state that the \textit{value pairs} between the "related" \textit{column pairs} have same semantic relationship.
%Now in absence of knowledge base, we 
only consider
%\wolf{11/1: `only consider'}
columns that are \emph{in a functional relationship} (thus the value in one column functionally determines the value in the other column).  
For example, the \textrm{ParkName} functionally determines the \textrm{ParkLocation} 
indicating a possible semantic relationship (even if the KB does not contain \textit{parkLocations}).  
%rjm added 10/31
Our hypothesis is that column pairs in a functional relationship are more likely to contain an interesting relationship that also exists in other tables and is useful in union search. 
This has the benefit of limiting the number of column pairs we analyze.
% yet has the potential downside of missing many-many relationships 
% (like actors playing in movies) unless they are already modeled in an existing KB.  
%to each other using the second component of our relationship oracle i.e., \textit{functional dependency}.
%We assume that two columns have a relationship between them if they have a functional dependency between them in any direction.

%rjm 10/31 this is incorrect
%SANTOS uses an existing (approximate) functional dependency discovery algorithm to find \textit{property columns} that functionally depend on the user's chosen \textit{subject column} in the query table.  At query time, we also find functional dependencies from columns in data lake tables that match (meaning have the same column semantics) as the query subject column.
%\grace{10/20: we may need to change the name} and store their relationships.
SANTOS uses an existing (exact) functional dependency (FD) 
discovery algorithm 
called FDEP~\cite{1999_flach_database_dependency_discovery} 
to find unary FDs (FDs with a single column determinant).
% Specifically, we use FDEP~\cite{1999_flach_database_dependency_discovery} to discover the functional dependencies.
%an induction algorithm of dependencies. 
%FDEP induces a set of valid FDs from a set of general dependencies by performing pairwise comparisons between all tuples. 
%The resulting set must be complete and minimal.
More precisely, we run their bottom-up variant 
that starts by considering all pairwise relationships, and checking if a given dependency satisfies or violates an FD.
Notice that since we are only considering binary relationships, we only compute unary FDs.
% (FDs where the left-hand-side is a single attribute).  
%Also notice that we only consider column pairs with an empty KB relationsho semantics.  

%rjm do we need this as we are only doing unary FDs
%Compared to other FD algorithms, FDEP is memory efficient and scales the best when a dataset has a large number of columns, which is suitable for data lake tables \cite{2015_papenbrock_fdep_comparison}.
%To solve this problem, we assume that the columns are pre-processed and the homographs and incorrect entries are removed before creating the synthetic knowledge base \cite{21_leventidis_homograph_detection}.


%\wolf{11/1: there are 3 subsections. It may be better to start here witha quick overview of teh 3 steps, but not yet discuss the actual example, which is discussed in the example box in 5.1 below}
Unlike web tables, the data lake tables are generally large enough (in \cref{fig:synthetic_kb}, we show only few rows and two columns for conciseness) that we can more reliably find non-spurious FDs (meaning, FDs that are likely to hold in the domain, not just this one instance).

%resolved!
%\rjm{I don't think I understand.  Is the assumption that the KB doesn't know about museums?  Why are we assuming FDs?  I thought we were discoverying if there is an FD?}
%\aamod{10/30: updated! we discover FD. Yes, we assume that the KB is not available or is not covering the entities in this case. Shall we update example to something that is really not found?}




%-------------------------------------
%-------------------------------------
%-------------------------------------

%\subsection{Formalization of Synthesized KB}
%\updated{Grace 2/15: 5.1, 5.2 are a draft of the formalization of synthesized KB for revisions}
%\aamod{2/16: We will remove this subsection and add text here to section 5.0.}
Formally, for Columns $c_1, c_2, \dots c_n \in$ Table $T_i$, each unique column pairs, $(c_i, c_j)$ in a Functional relationship is assigned a synthesized relationship semantics $RS(c_i, c_j)$. For values $u_1, u_2, \dots u_m \in c_i$ and $v_1, v_2, \dots v_m \in c_j$, $(u_{ki}, v_{kj})$ of the same tuple k in a unique column pair is also assigned synthesized relationship $RS{(c_i, c_j)}$.
%\aamod{we need to define KB confidence score too. Here the score is KB confidence score.}
Each synthesized relationship of $(u_{ki}, v_{kj})$ is assigned a confidence score that indicates how likely $(u_{ki}, v_{kj})$ has that type. Since $u_{ki} \in c_i$ and $v_{kj} \in c_j$, $(u_{ki}, v_{kj})$ has relationship semantics $RS{(c_i, c_j)}$ with confidence score of 1. $(u_{ki}, v_{kj})$ also adopts synthesized RS of relationship pairs consisting of $(c_i, c_j) \setminus (u_{ki}, v_{kj})$ with RS confidence scores computed as 
\grace{3/17: Does anyone know how to have this as a formula or some kind of formalization, that we can reference elsewhere?}

$$\dfrac{|(c_i, c_j) \setminus (u_{ki}, v_{kj})| \in T_i \cap T_j}{|(c_i, c_j)|}$$
where $|(c_i, c_j) \setminus (u_{ki}, v_{kj})| \in T_i \cap T_j$ represents the number of value-pairs belonging in the same tuple from $c_i$ and $c_j$, other than $(u_{ki}, v_{kj})$, in table $T_i$ that are found in table $T_j$, and $|c_i, c_j|$ represents the total number of value-pairs in unique column pair $(c_i, c_j)$. 
%If there are conflicting confidence scores for a synthesized type, we take the maximum score.

\begin{example}
\label{example:synth_kb_scores}
Consider Synthesized relationship dictionary ($S$) and Tables 1, 2 and 3 in \cref{fig:synthetic_kb}. We assigned value-pairs in the column pairs (A,B), (D,E) and (F,G) with synthesized relationship semantics $RS_{(A,B)}, RS_{(D,E)}$ and $RS_{(F,G)}$ respectively.
$S$ stores the value pairs as key and the set of synthesized RS with confidence scores assigned to them as value.
As \textrm{(Brands Park, Moana)} belongs to the column pairs having synthesized RS $RS_{(A,B)}$ and two out of three total value pairs in Table 1 i.e., \textrm{(Kells Park, Spider-Man)}) and \textrm{(Eckhart Park, Avengers)} also belong to the column pairs in Table 2 having synthesized RS $RS_{(D,E)}$, 
S[(Brands Park, Moana)] = \{RS_{(A,B)} : 1, RS_{(D,E)} : $\frac{2}{3}$\}.
\end{example}
Next, we explain the steps involved in creating S.
\subsection{Creating Synthesized Knowledge Base} 
First, we iterate through the data lake tables and store occurrences of all value-pairs in column-pairs in a \textit{Lookup Dictionary}. Then, we iterate through this dictionary to annotate each value-pair with relationship semantics and associated confidence scores.

\introparagraph{Lookup Dictionary Creation} At first, for each data lake table, identify the column pairs in a functional relationship and assign them a synthesized RS. In the meantime, we also record the occurrence of value pairs (not covered by the existing KB) from those column pairs in Lookup relationship dictionary ($L$). L has the value-pairs as key and the set of synthesized RS as value. For example, \textrm{(Kells Park, Spider-Man)}) is a key in L. Also, as it appears in two column pairs having synthesized semantics $RS_{(A,B)}$ and $RS_{(D,E)}$, it has value \{$RS_{(A,B)}$, $RS_{(D,E)}$\}. 
\grace{3/17: Should we include an in-line example of a lookup dictionary?}

\introparagraph{Synthesized Relationship Dictionary Creation} 
Once we create the lookup dictionary, we use it similar to the relationship dictionary (\cref{section:unionability_components}) and annotate the column pairs.
\begin{example}
For example, suppose we are processing Table 1 of \cref{fig:synthetic_kb} as data lake table after creation of lookup relationship dictionary. All three values have synthesized relationship $RS_{(A,B)}$ as they belong to the same column pair. Here, (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}) also have synthesized relationship $RS_{(D,E)}$.
Therefore, we assign both $RS_{(A,B)}$ and $RS_{(D,E)}$ as the synthesized relationship (that is, the synthesized RS) with confidence scores, calculated by Formula x. \grace{TODO: reference formalization above}
% which is the fraction of unique value pairs mapped in the synthesized RS to the total number of unique value pairs in the column pairs. 
For Table 1, the confidence score for $RS_{(A,B)}$ is 1.0 and $RS_{(D,E)}$ is $\frac{2}{3} = 0.66$. 
%With these confidence scores, we define the Synthesized RSCS.
\end{example}
Recall that, we assume all \textit{value pairs} in the same \textit{column pair} have the same semantic relationship between them. Also, recall relationship dictionary from \cref{section:unionability_components} (\cref{fig:indexes}) that contains entity pairs as key and the set of tuples of (binary relationships, confidence score) as values. Similarly in synthesized relationship dictionary, we add each value pair in the column pair as keys and the set of tuples of (synthesized relationships, confidence score) assigned to the column pairs as values. If a synthesized relationship already exists in $S$ for a \textit{value pair}, we take the maximum score.

\begin{example}
Again consider data lake tables in \cref{fig:synthetic_kb} as an example. 
After processing Table 1,
$S$ contains the following three tuples as keys:  (\emph{Brands Park, Moana}),
(\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}).
All value-pairs now have values: \{$RS_{(A,B)}$: 1.0, $RS_{(D,E)}$: $\frac{2}{3}$\}.

Next, we process Table 2 in a similar manner, and add/update its value pairs
(\emph{Kells Park, Spider-Man}), (\emph{Eckhart Park, Avengers}), (\emph{Union Park, Black Panther}), (\emph{Chopin Park, Trolls}) as keys
and \{$RS_{(A,B)}$: $\frac{2}{4}$, $RS_{(D,E)}$:1, $RS_{(F,G)}$: $\frac{1}{4}$\} as their values to $S$.
However, as (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}) already have values for $RS_{(A,B)}$ and $RS_{(D, E)}$, we take the maximum scores. 

So, after processing Table 2, the value for both (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}) is 
$\{RS_{(A,B)}$: 1, $RS_{(D,E)}$:1, $RS_{(F,G)}$: $\frac{1}{4}$\}
%rjm get an update on their values. 
%are updated.

Table 3 is processed in the same way. At the end, the synthesized relationship dictionary is shown in the figure.

%However, by using our transitive closure, we provide them with a synthesized semantic type from Table 2.
%\rjm{10/31:  what is "our transitive closure".  Define this formally.  Or leave this out if it is a minor detail.  I suggest the latter given that we don't have time to introduce new concepts this late. }
%\aamod{10/31: Yes, that just means co-occurrence with neighbooring tables. It's a minor detail. Removed}
\end{example}
In  the example, we only show one column pair for each table. For more column pairs, we process each of them in the same way.

After processing all data lake tables, we append \textit{synthesized relationship dictionary} to the (YAGO) \textit{relationship dictionary}, which we use during the query phase. \grace{3/17: TODO: edit the transition into section 6}
As mentioned before, we set synthesized CSCS to 1 and hence, the confidence score of synthesized RS forms synthesized RSCS.  %\aamod{02/18: todo: add the figure showing dictionaries}.
On what follows, we add each synthesized RSCS to the inverted index as shown in \cref{fig:indexes}. It is interesting to see that although Query table in \cref{fig:synthetic_kb} does not have any value overlap with Table 1, Table 1 still has a non-zero ranking score because of indirect overlap. We will discuss about the query phase in detail in \cref{section:semantic_union_search}.

%Similar to RSCS in \cref{section:unionability_components}, we store synthesizd RSCS to the main Inverted Index (S) with synthesized RSCS as key and the tuple of (table name, confidence score) as value as shown in the \cref{fig:synthetic_kb} \aamod{02/18: update the figure reference}.


% \subsection{Reducing the Number of Relationships}
% %\aamod{10/31: trying to start positively :) ! We will move this to discussion or some other sections at the end}

% The synthesized knowledge base stores: 
% %mainly stores two information: 
% the \textit{value pairs} and \textit{synthesized relationship semantics}. %Therefore, there are mainly two areas in which we can optimize our synthetic knowledge base.
% %\subsubsection{Reducing the number of synthesized relationships}
% As shown in \cref{fig:synthetic_kb}, the number of synthesized relationship is equal to the total number of \textit{column pairs} with a functional dependency between them that are not represented in the KB. However, one can merge certain relationships based on  available information. If all value pairs of a smaller column pair are contained in a large column pair, we assign both a single synthesized relationship. For example, in the absence of row (\emph{Freud Museum, Camden}), we would assign a single synthesized relationship, say \texttt{C\_D}, to the column pair in Table (1) and Table (2).
% A step ahead from containment, if two column pairs have high overlap between them, we can merge their synthetized relationships. Precisely, given two column pairs $c_{11} c_{12}$ and $c_{21} c_{22}$ having $n_1$ and $n_2$ $(n_1 \leq n_2)$ unique value pairs respectively. Let there are $g$ unique value pairs that appear in both column pairs. Then,
% %we remove $c_{11} c_{12}$'s synthesized relationship and assign it $c_{21} c_{22}$'s synthesized relationship
% if $\frac{g}{n_1} \geq \eta$, we can assign them a single synthesized relationship. Here, $\eta$ ranges from $0$ to $1$. This optimization is applied just after the creation of lookup table in offline phase.

% \begin{example}
% For example, let us revisit the column pairs of Table 1 and Table 2 of \cref{fig:synthetic_kb}. We see that there are two value pairs:\{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\}
% overlapping between them. If we consider $\eta = 0.66$, the column pairs in Table 1 and Table 2 will be identified with a single synthetic relationship \texttt{C\_D}.
% \end{example}

%Therefore, we use an inverted index having the synthesized relationship as key and the tuple of \textit{(table name, column pair index, confidence score)} as value as shown in \textit{Synthesized Inverted Index} of \cref{fig:synthetic_kb}.


%\aamod{02/15: This is the old Synthesized KB definition. Grace, please feel free to use it if it makes sense in someway to expand column based definition to the relation-based.}
% \begin{definition}[Synthesized KB]
% If \{$A_1 B_1$, $A_2 B_2 \dots$ ,$A_pB_p$\} $\in \mathcal W_D$ are the unique column pairs having a functional dependency, \{$A_1\_B_1$, $A_2\_B_2 \dots $ ,$A_p\_B_p$\} are the respective synthesized relationships assigned to them and
% \{$a_1b_1$, $a_2b_2$ \dots $a_qb_q$\} $\in \mathcal U_D$ are the unique column value pairs in the entire data lake,
% the synthesized knowledge base for the given data lake is a key-value pair having $a_i\_b_i$  for each $a_ib_i \in \mathcal U_D$ as a key and $\forall key$, a vector $(g_{i1} A_1\_B_1, g_{i2} A_2\_B_2, \dots g_{ip} A_p\_B_p)$as value.
% \end{definition}
% For instance, for a data lake having column pairs \{$A_1B_1$, $A_2B_2$\} and value pairs \{$a_1b_1$, $a_2b_2$ $a_3 b_3$\} , 
% the synthetic KB contains the key-value pairs: $\{a_1\_b_1: (g_{11} A_1 B_1, g_{12} A_2 B_2)\}$, 
% $\{a_2\_b_2: (g_{21}A_1 B_1, g_{22}A_2 B_2\}$,
% $\{a_3\_b_3: (g_{31}A_1 B_1 g_{32}A_2 B_2\}$ respectively.

==> sections/synthetized_kb_updated_roee.tex <==
\section{Synthesized Knowledge Bases}
\label{section:synthetic_knowledge_base}
\begin{figure*}[h]
  \includegraphics[scale = 0.52]{figures/synthesized_index.pdf}
  \caption{Data-Lake Tables and Synthesized Relationship Dictionary (S), made up of synthesized relationship types of each value-pair. Value-pairs highlighted in blue appear in Tables 1 and 2, and the value-pair highlighted in green appear in Tables 2 and 3. %\aamod{03/19: @Grace, Should we change the dark blue and dark green colors to something light while highlighting the text? In monochrome print, text having dark backgrounds are difficult to read.}
  %\grace{Done! Is this okay?}
\wolf{3/22: 1. Suggestion to put Table 1-3 on top of the tables at same horizontal height /
keep formatting of tables consistent with the one from Figure 1 throughout (same cell height for value cell and attribute name cell / same text font and size /
same color for background of text of entire background of cell) 
2. Should the right table have a name `S'?
3. Is `type: confidence score' the appropriate name? It seems it should be just `semantics' (relationship mapped to its semantics). But then a RS is not a pair, but rather a `set of weighted (ordered) pairs' (the order matters too!)
4. Link to both example 18 and 19 (the numbers and arrows are not clear before)}
  } 
\label{fig:synthetic_kb}
\end{figure*}

Knowledge bases (KBs) have limited coverage over the data values found in real data lakes especially, the relationships returned tend to be sparse.
Hence, using an existing KB (even a set of KBs) 
as the only source for determining column and relationship semantics can lead to low coverage (recall). %\roee{Update:} 
% \wolf{3/22: ``determining'' instead of finding? `determining the column type and relationship semantics across columns can ...'}
% \aamod{I agree. updated}
As an example, our experimental study (see Section~\ref{section:experiments}) indicate that YAGO, a well-known and maintained KB, covers only a 41.81\% string values over UK open data and 33.92\% string values over Canada open data. 
% \wolf{3/22: this means that 42 percent of the column names can be identified? 
% Or that 42 of the pairwise relations can be identified?
% Or that 42 of the relationship between the non-key and the key columns can be identified?}
% \aamod{This means 42 \% of cell values can be mapped to the entities in the KB. We have also reported this for each column in the experiment section. However, we do not have the ground truth for the relationships i.e., we don't know how many relationships should exist. therefore, we have not reported for the relationships}

To solve this problem, we propose a novel
data-driven approach for creating a \emph{synthesized KB} using the data lake itself. Specifically, we directly mine meaningful relationship semantics from the data lake tables and fill in the gaps left by the existing KB.
% \wolf{3/22: `gapes left by the existing'}\
% \aamod{updated :)}

When using YAGO, we create four different dictionaries, namely, for entities, inheritance, types and relationships (see \cref{subsection:knowledge_base}).  
% \wolf{3/22: I started reading here. Was it explained earlier what those 4 categories exactly mean?}
Following an entirely data-driven approach, for the case of synthesized KB we focus primarily on relationships, creating a \textit{Synthesized Relationship Dictionary}. Since we directly use the cell values as entities, an entity dictionary is not needed and inheritance requires external type hierarchy which does not exist in this case. A type dictionary can also be generated fairly easily; yet, following our data-driven approach we simply set a dummy column semantics with synthesized CS$_{\textsc{Conf}}$ of 1
and focus on finding synthesized RS.
%in synthesized RS$_{\textsc{Conf}}$ (see \cref{def:rscs}).
%\wolf{3/22: use shortcut CREF \cref{def:rscs} instead of REF \ref{def:rscs}}
% \wolf{3/22: This past paragraph contains a lot of likely useful information. Is this clear for a reader who started earlier? 
% E.g. why a type hierarchy does not exist `in this case' /
% `since we can use the cell values as entities' /
% is the type hierarchy easy to create, or it does not exist?}
 
% To keep the synthesized KB entirely data-driven, we also do not create the inheritance dictionary, which requires an external type hierarchy. We focus primarily on the \textit{Synthesized Relationship Dictionary}. A type dictionary can also be similarly generate; yet, following our data driven approach we simply set  set the synthesized CSCS to 1 in synthesized RSCS (see Definition~\ref{def:rscs}).
%One can easily use the same technique (taking columns instead of column pairs) to create \textit{Synthesized Type Dictionary} %However, as the type hierarchy is not available and we directly work with cell values, we only create synthesized relationship dictionary and set the synthesized CSCS to 1 in synthesized RSCS. 
% \grace{3/17: The paragraph above is a bit wordy, and readers can get lost trying to follow it. Can we instead say, we use the synthesized KB to mine for relationship semantics, especially considering the sparsity of the relationships returned by an external KB? Instead of talking about why we don't create the other dictionaries?} \roee{I revised the paragraph to be (much) less wordy. let me know what you think.}
%Though it may slightly impact the effectiveness due to absence of synthesized column semantics, it eliminates the computation and storage cost of \textit{Synthesized Type Dictionary} giving similar effectiveness.

The synthesized relationship dictionary is created based on \textit{value-pairs} (values in a \textit{column pair}) for which relationship semantics were not found in the existing KB. 
% \wolf{3/22: What is a nice word to contrast synthesized KB against: here `existing KB' / or `pretrained KB' or `external KB' or ... Whatever it is, best to decide then consistently use}
% \aamod{3/23: we are using "existing kb" everywhere}
For each such value pair, we assign a binary \emph{synthesized semantic relationship} which is stored in the synthesized relationship dictionary. Intuitively, a synthesized semantic relationship is a distribution of column pairs in the data lake in which a particular pair of values appears. 

% A binary relationship between the value-pair a \emph{synthesized semantic relationship}, and these relationships are stored in the synthesized relationship dictionary. 


%For data-lake tables, and especially relationship tables made up of several entities, relationships are difficult to retrieve from the existing KB. Thus, we assign the binary relationship between the value-pair a \emph{synthesized semantic relationship}, and these relationships are stored in the synthesized relationship dictionary. We keep the structure of the dictionary consistent with the others in order to query them all in a uniform manner. Furthermore, we make sure to only store relationships between values in columns that have a unary functional dependency (further explained below). This way, the size synthesized relationship dictionary is manageable.

% \roee{I think it is too early for an example here. Maybe only introduce the table and say we assume that we were not able to map the values using a standard KB:}
% \begin{example}
% \label{example:synth_kb_concept}
% To illustrate the setup for the synthesized KB, consider the column pairs in Tables 1, 2, 3 of \cref{fig:synthetic_kb}. The tables hold information about films presented in parks at a given day and time. We assume that only one film is showing at a given park at a certain time, so the columns form a functional dependency. 
% %\wolf{3/22: suggestion to remove the footnote because it does not show well and include as standard text.}
% %resolved
% For sake of example, assume we were unable to find their relationships from an existing KB. Thus, these value pairs will be stored in the synthesized relationship dictionary, each with synthesized semantic relationships. 
% % \wolf{3/22: here best to give some intuition behind the `semantic relationship', what is it. Is this true?
% % ``Intuitively, a synthesized semantic relationship is a distribution of column pairs in the data lake in which a particular pair of values appears. This information (or index) forms the basis of a quantitative analysis similar in nature to topic models given represent a distribution over source documents''}
% These relationships are later associated with their type scores which can be ignored for the time being. For example the value pair \textrm{(Brands Park, Moana)} from Table 1 will be added to the synthesized relationship dictionary (shown on the right of the figure) with a synthesized semantic relationship $RS(A,B)$ (see \cref{def:rs}).
% % \wolf{3/22: explain that RS is Relationship Semantics. 
% % So according to the last sentence, a RS is just a pair of columns from the same table? Isn't it instead a set of pairs?}
% % \aamod{3/23: RS is defined in \cref{def:rs}}
% %  Tables 1 and 2 have direct value-pair overlaps, indicating that they have similar relationship semantics. The same is seen in tables 2 and 3, with their shared value (Union Park, Black Panther). However, Tables 1 and 3 do not have an overlap, but both have overlaps with table 2, so they indirectly overlap.  
% \end{example}

\subsection{Creating a Synthesized Relationship Dictionary} 

%Considering the observation in \cref{example:synth_kb_concept}, w
We first assign all value pairs in a column pair with the same synthesized semantic relationship. 
% \wolf{3/22: so this gets confusing. Suggestion:
% 1. keep a motivating example first as you do. But then 2. here give a clear formal definition: what is a RS? Is it a pair, or a set of pairs, or a set of weighted column pairs? With weight determination open to different instantiations. But however one determines (with iteration or not), it will still be a set of weighted pairs, right?}
For instance, the value-pairs \textrm{(Brands Park, Moana)}, \textrm{(Kells Park, Spider-Man)} and \textrm{(Eckhart Park, Avengers)} in Table 1 of \cref{fig:synthetic_kb} are assigned with the same synthesized relationship semantics $RS{(A, B)}$. %$RS\roee{change the notation $R_{(A, B)}$ to $RS{(A, B)}$}{(A,B)}$.
% \wolf{3/22: suggestion to define a pair of columns as RS, but rather some statistics over pairs.}

% are not meaningful without additional contextual information and are rather indirect.
As we have discussed however, some binary relationships between columns in a data lake are not meaningful and may be indirect. For example, going back to \cref{fig:running_examples}, the value-pairs in $\Pi_{\mathrm{Film Title, Park Location}}$ 
(e.g., \textrm{(Bee Movie, 6748 N. Sacramento Ave.)} and
\textrm{(Coco, 5210 W. $64^{\mathrm{th}}$ St.)}) in Table (c) 
have a tenuous relationship at best (film was shown in a park with this address). In what follows, aiming to capture only meaningful relationships, we will only consider pairs of columns whose relationship is functional (one of them functionally determines the other). %(thus the value in one column functionally determines the value in the other column).  
% \wolf{3/22: ...``only consider pairs of columns whose relationship is function (one of them functionally determines the other)''}  
For example, in \cref{fig:running_examples}(b), \textrm{ParkName} functionally determines the \textrm{ParkLocation} indicating a possible relationship, 
%semantic relationship, 
% \wolf{3/22: is a SR formally defined before in section 4?}  
even if a KB does not cover it. 
We hypothesize that column pairs in a functional relationship are more likely to contain a \emph{meaningful} relationship that also exists in other tables and is useful in union search. 
% \wolf{3/22: So this last sentence is important. This is something that is good to bring early:
% 1. here is our observation (with an example)
% 2. then here is our formalism motivated by these earlier observations}  
As a side-effect, this also has a benefit of reducing the synthesized relationship dictionary size. 

\begin{example}
\label{example:synth_kb_concept}
To illustrate the setup for the synthesized KB, consider the column pairs in Tables 1, 2, 3 of \cref{fig:synthetic_kb}. The tables hold information about films presented in parks at a given day and time. We assume that only one film is showing at a given park at a certain time, so the columns form a functional dependency. 
%\wolf{3/22: suggestion to remove the footnote because it does not show well and include as standard text.}
%resolved
For sake of example, assume we were unable to find their relationships from an existing KB. Thus, these value pairs will be stored in the synthesized relationship dictionary, each with synthesized semantic relationships. 
% \wolf{3/22: here best to give some intuition behind the `semantic relationship', what is it. Is this true?
% ``Intuitively, a synthesized semantic relationship is a distribution of column pairs in the data lake in which a particular pair of values appears. This information (or index) forms the basis of a quantitative analysis similar in nature to topic models given represent a distribution over source documents''}
These relationships are later associated with their type scores which can be ignored for the time being. For example the value pair \textrm{(Brands Park, Moana)} from Table 1 will be added to the synthesized relationship dictionary (shown on the right of the figure) with a synthesized semantic relationship $RS(A,B)$ (see \cref{def:rs}).
% \wolf{3/22: explain that RS is Relationship Semantics. 
% So according to the last sentence, a RS is just a pair of columns from the same table? Isn't it instead a set of pairs?}
% \aamod{3/23: RS is defined in \cref{def:rs}}
%  Tables 1 and 2 have direct value-pair overlaps, indicating that they have similar relationship semantics. The same is seen in tables 2 and 3, with their shared value (Union Park, Black Panther). However, Tables 1 and 3 do not have an overlap, but both have overlaps with table 2, so they indirectly overlap.  
\end{example}

We use an existing 
%(exact) 
\emph{functional dependency} (FD) discovery algorithm called FDEP~\cite{1999_flach_database_dependency_discovery} to find unary FDs (FDs with a single column determinant, considering only binary relationships).
% Specifically, we use FDEP~\cite{1999_flach_database_dependency_discovery} to discover the functional dependencies.
%an induction algorithm of dependencies. 
%FDEP induces a set of valid FDs from a set of general dependencies by performing pairwise comparisons between all tuples. 
%The resulting set must be complete and minimal.
More precisely, we run their bottom-up variant that starts by considering all pairwise relationships, and checking if a given dependency satisfies or violates an FD. It is also worth noting that, unlike web tables, data lake tables are generally large enough where we are more likely to find non-spurious FDs (FDs that are likely to hold in the domain, not just in an instance). In what follows, we filter out all column pairs that are not functional, which, in turn, might present some issues. First, FDEP time complexity is quadratic, which can be a bottleneck if applied in query time. However, we only use it in the offine phase and benefit from an important improvement in space complexity. Second, some observed FDs can be spurious (contains false positives). We only consider FDs as a proxy for meaningful relationships; yet, even if we add a non-meaningful relationship to the synthesised KB, it may not affect the output of our algorithm rather slightly increase the running time. 
% \wolf{3/22: so this discussion on FDs is important and a crucial assumption. It merits a whole separate paragraph, perhaps with separate bold intro word. What you like to bring:
% 1. semantic relationships only make sense if they are functional;
% give a quick motivation (you can give with counterexample, and example, whatever it is, it should scrutiny)
% 2. so you first need to filter column pairs down to those that are functional
% 3. problem is that 
% a. you only learn FD based on observed FDs, and those can be spurious (false positives)
% b. the complexity.
% 4. shortly explain why a) and b) are not problems (e.g. even false positives, thus some that are not functional, will not screw up your algorithm: at least I think so. But that is important to point out: usually we need 100\% correctness in FDs, but your approach is likely also ok with 50\% correctness, correct?)
% }  
% \roee{add a sentence about time-space complexity for FD discovery and its correctness.}

\subsubsection{Overview}
To this end, the key idea is to model (and store) relationships between pairs of values as a weighted distribution  over exiting columns that exhibit some meaningful relationships. A similar idea also exists, for example, in topic modeling~\cite{papadimitriou2000latent}, where some latent topic of a document (pair of values) is represented by a distribution over other documents (pair of columns). 

Generally, different weighting schemes can be designed. In this work, we assume that the highest weight is assigned to a RS created from the value pair origin, that is the pair of columns under which it appears in a table. Note that a single pair of values may be assign with more than one highest weight if it appears in more than one table (first pass, \cref{sec:firstpass}). Once we cover these, we also want to assign some indirect relationships to value-pairs. We do so by looking into the overlaps between the column pairs. For example, the value-pair \textrm{(Brands Park, Moana)} in Table 1 in \cref{fig:synthetic_kb} does not appear in the column pair $(D,E)$; however, since $(A,B)$ and $(D,E)$ share information (\textrm{(Kells Park, Spider-Man)} and \textrm{(Eckhart Park, Avengers)}, \textrm{(Brands Park, Moana)} should also be assigned with some, lower, weight with respect to $(D,E)$. 

\subsubsection{First Pass}\label{sec:firstpass}
To generate our synthesized relationship dictionary, we first iterate over the data lake tables and identify the column pairs (which were not covered by the existing KB) in a functional dependency and generate a synthesized relationship semantics that represents it. 
% \wolf{3/22: 1. what is the sequence: first identify the undocumented pairs (which can be quadratic in average table column number), or identify the FD pairs (which are more likely not quadratic in general)?
% 2. at this point it is not yet clear what exactly the outcome, thus what ``a synthesized RS'' actually is
% }
In the same pass, we also perform the first pass over the value-pairs in these column-pairs and add the respective relationship semantics with the type score of 1. 
% \wolf{3/22: stop. these here seems to explain in words an algorithm. But please first explain the intuition. Something like
% 1. RS are intuitively a weighted set of pairs
% 2. we create these in two steps: first we get the pairs, then we iteratively calculate the scores.
% The calculation is such that [explain here the motivation of the updates / what the desired outcome is].
% Once the reader knows what you try to achieve, it is easier to follow along the individual steps}
\begin{example}
Using example \cref{fig:synthetic_kb}, at this point we generate the synthesized relationship semantics \{$RS{(A,B)}$, $RS{(D,E)}$, $RS{(F,G)}$\} and add the value-pairs \textrm{(Brands Park, Moana)}, \textrm{(Kells Park, Spider-Man)}, etc. with their respective relationship semantics. 
% \wolf{3/22: what are respective RS here? 
% Also should this be part of an example environment?}
In this pass, for example, the value-pair \textrm{(Kells Park, Spider-Man)} will be already assigned with two relationships, namely, $RS{(A,B)}$, $RS{(D,E)}$. We refer to the dictionary after the first pass as a \emph{lookup dictionary}.
\end{example}



% \wolf{3/22: what seems to be going on:
% The intuition seems to be a bit like in topic modeling: there you model a document as a distribution over other documents (or a distribution of topics, which are themselves a distribution of documents or so / maybe good to look up exactly and to draw the connection).

% Here you try to model the directed relationship of a pair of cells by a weighted distribution over existing columns.
% Full stop here. That is the key idea. That is *very nice* and merits itself a detailed discussion(e.g. the connection to topic modeling, or possibly latent semantic indexing, etc.). People will understand and appreciate this idea.

% Then you describe one particular instance of the weights. Before you describe the iterations, describe what the intuition is that you try to capture with the calculations. So without this, I can't follow at all everything below.}


%Notice that since we are only considering binary relationships, we only compute unary FDs.
% (FDs where the left-hand-side is a single attribute).  
%Also notice that we only consider column pairs with an empty KB relationsho semantics.  

%rjm do we need this as we are only doing unary FDs
%Compared to other FD algorithms, FDEP is memory efficient and scales the best when a dataset has a large number of columns, which is suitable for data lake tables \cite{2015_papenbrock_fdep_comparison}.
%To solve this problem, we assume that the columns are pre-processed and the homographs and incorrect entries are removed before creating the synthetic knowledge base \cite{21_leventidis_homograph_detection}.


%\wolf{11/1: there are 3 subsections. It may be better to start here witha quick overview of teh 3 steps, but not yet discuss the actual example, which is discussed in the example box in 5.1 below}
% Unlike web tables, the data lake tables are generally large enough (in \cref{fig:synthetic_kb}, we show only few rows and two columns for conciseness) that we can more reliably find non-spurious FDs (meaning, FDs that are likely to hold in the domain, not just this one instance).

%resolved!
%\rjm{I don't think I understand.  Is the assumption that the KB doesn't know about museums?  Why are we assuming FDs?  I thought we were discoverying if there is an FD?}
%\aamod{10/30: updated! we discover FD. Yes, we assume that the KB is not available or is not covering the entities in this case. Shall we update example to something that is really not found?}




%-------------------------------------
%-------------------------------------
%-------------------------------------

%\subsection{Formalization of Synthesized KB}
%\updated{Grace 2/15: 5.1, 5.2 are a draft of the formalization of synthesized KB for revisions}
%\aamod{2/16: We will remove this subsection and add text here to section 5.0.}
\subsubsection{Second Pass (assigning type scores to value-pairs)}

Using the lookup dictionary, we now find the confidence scores of relationship types that each value-pair has. 
Currently, for Columns $c_1, c_2, \dots c_n \in$ Table $T_i$, consider unique column pairs, $(c_i, c_j)$.
% has a synthesized relationship semantics $RS(c_i, c_j)$. Then, 
A value-pair $(u_{ki}, v_{kj})$ such that $u_{ki}\in c_i$ and $v_{kj}\in c_j$ has been assigned synthesized relationship $RS{(c_i, c_j)}$.
%For values $u_1, u_2, \dots u_m \in c_i$ and $v_1, v_2, \dots v_m \in c_j$, $(u_{ki}, v_{kj})$ of the same tuple k in a unique column pair is also assigned synthesized relationship $RS{(c_i, c_j)}$.
%\aamod{we need to define KB confidence score too. Here the score is KB confidence score.}
Now, for each synthesized relationship of $(u_{ki}, v_{kj})$, we need to assign a type score that indicates how likely it is for $(u_{ki}, v_{kj})$ to be in a relationship. Firstly, $(u_{ki}, v_{kj})$ is assigned type $RS{(c_i, c_j)}$ with type score of 1. However, we also wish to propagate the generated relationships. To do so, we use the overlap between value-pairs appearing in different tables in the data lake. In what follows, a value-pair $(u_{ki}, v_{kj})$ now also adopts synthesized relationship that overlap with its initial relationship $RS{(c_i, c_j)}$. In the example of \cref{fig:synthetic_kb}, the value-pair \textrm{(Brands Park, Moana)} is also assigned with the synthesized relationship semantics $RS{(D, E)}$ since Table 1 and 2 and their respective synthesized relationship semantics $RS{(A, B)}$ and $RS{(D, E)}$ share the value pairs \textrm{(Kells Park, Spider-Man)}) and \textrm{(Eckhart Park, Avengers)}. 

The assigned type score is computed with respect to this overlap, as follows
% also adopts synthesized RS of relationship pairs consisting of $(c_i, c_j) \setminus (u_{ki}, v_{kj})$ with RS confidence scores computed as 
% Since $u_{ki} \in c_i$ and $v_{kj} \in c_j$, $(u_{ki}, v_{kj})$ has relationship semantics $RS{(c_i, c_j)}$ with confidence score of 1. 
% $(u_{ki}, v_{kj})$ also adopts synthesized RS of relationship pairs consisting of $(c_i, c_j) \setminus (u_{ki}, v_{kj})$ with RS confidence scores computed as 
% \grace{3/17: Does anyone know how to have this as a formula or some kind of formalization, that we can reference elsewhere?}
\begin{equation}\label{eq:confidence2pass}
    \dfrac{|(c_i, c_j) \setminus (u_{ki}, v_{kj})| \in T_i \cap T_j}{|(c_i, c_j)|}
\end{equation}
where $|(c_i, c_j) \setminus (u_{ki}, v_{kj})| \in T_i \cap T_j$ represents the number of value-pairs in $T_i$ (except $(u_{ki}, v_{kj})$) that also exist in $T_j$. $|c_i, c_j|$ represents the total number of value-pairs in unique column pair $(c_i, c_j)$. We clarify the computation using the following example.

% in the same tuple from $c_i$ and $c_j$ except $(u_{ki}, v_{kj})$, in table $T_i$ that are found in table $T_j$, and $|c_i, c_j|$ represents the total number of value-pairs in unique column pair $(c_i, c_j)$. 
%If there are conflicting confidence scores for a synthesized type, we take the maximum score.

% \begin{example}
% \label{example:synth_kb_scores}
% Consider Synthesized relationship dictionary ($S$) and Tables 1, 2 and 3 in \cref{fig:synthetic_kb}. We assigned value-pairs in the column pairs (A,B), (D,E) and (F,G) with synthesized relationship semantics $RS_{(A,B)}, RS_{(D,E)}$ and $RS_{(F,G)}$ respectively.
% $S$ stores the value pairs as key and the set of synthesized RS with confidence scores assigned to them as value.
% As \textrm{(Brands Park, Moana)} belongs to the column pairs having synthesized RS $RS_{(A,B)}$ and two out of three total value pairs in Table 1 i.e., \textrm{(Kells Park, Spider-Man)}) and \textrm{(Eckhart Park, Avengers)} also belong to the column pairs in Table 2 having synthesized RS $RS_{(D,E)}$, 
% S[(Brands Park, Moana)] = \{RS_{(A,B)} : 1, RS_{(D,E)} : $\frac{2}{3}$\}.
% \end{example}

\begin{example}
\label{example:synth_kb_scores}
Consider Tables 1, 2 and 3 and an example synthesized relationship dictionary given at the right part of \cref{fig:synthetic_kb}. 
The first pass assigns all value-pairs with their synthesized relationship semantics $RS{(A,B)}, RS{(D,E)}$ and $RS{(F,G)}$ with respect to their consisting table with a type score of 1. 

For the second pass, consider \textrm{(Brands Park, Moana)}. Since Table 1 ($RS{(A,B)}$) and 2 ($RS{(D,E)}$) share the value-pairs \textrm{(Kells Park, Spider-Man)} and \textrm{(Eckhart Park, Avengers)}, the value-pair \textrm{(Brands Park, Moana)} is also assigned with $RS{(D,E)}$. Specifically, using \cref{eq:confidence2pass}, we assign a type score of $\frac{2}{3}$ to the value-pair \textrm{(Brands Park, Moana)} for the type $RS{(D,E)}$, since Table 1 that contains the pair has two other value-pairs that overlap with Table 2, out of a total of three value-pairs.

Now consider Table 2. Table 2 shares two value-pairs with Table 1 (\textrm{(Kells Park, Spider-Man)}, \textrm{(Eckhart Park, Avengers)} and one value-pair with Table 3, namely \textrm{(Eckhart Park, Avengers)} out of the four value-pairs it consists. In what follows, the value-pair \textrm{(Chopin Park, Trolls)} will be assigned with $RS{(A,B)}$ with a type score of $\frac{2}{4}$ = 0.5 and $RS{(F,G)}$ with a type score of $\frac{1}{4}$ = 0.25 in addition to it's original assignment to $RS{(D,E)}$ with type score = 1.
\end{example}

% Next, we explain the steps involved in creating S.


% \subsection{Creating The Synthesized Knowledge Base Details} 
% In practice, we first iterate over the data lake tables and identify the column pairs (which were not covered by the existing KB) in a functional dependency and generate a synthesized relationship semantic that represents it. In the same pass, we also perform the first pass over the value-pairs in these column-pairs and add the respective relationship semantics with the confidence score of 1. Using example \cref{fig:synthetic_kb}, at this point we generate the synthesized relationship semantics \{$RS{(A,B)}$, $RS{(D,E)}$, $RS{(F,G)}$\} and add the value-pairs \textrm{(Brands Park, Moana)}, \textrm{(Kells Park, Spider-Man)}, etc. with their respective relationship semantic. In this pass, for example, the value-pair \textrm{(Kells Park, Spider-Man)} will be already assigned with two relationships, namely, $RS{(A,B)}$, $RS{(D,E)}$. We refer to the dictionary after the first pass as a \emph{lookup dictionary}.

% In the second pass we use \cref{eq:confidence2pass}, assigning indirect relationships to value-pairs that already exist in the lookup dictionary. At this pass, the value-pair \textrm{(Brands Park, Moana)} will also be assigned with $RS{(D,E)}$ with a confidence value of $\frac{2}{3}$ as described before. After this pass, the lookup dictionary becomes a synthesized relationship dictionary. 

% we use it similar to the relationship dictionary (\cref{section:unionability_components}) and annotate the column pairs.

% Recall that, we assume all \textit{value pairs} in the same \textit{column pair} have the same semantic relationship between them. Also, recall relationship dictionary from \cref{section:unionability_components} (\cref{fig:indexes}) that contains entity pairs as key and the set of tuples of (binary relationships, confidence score) as values. Similarly in synthesized relationship dictionary, we add each value pair in the column pair as keys and the set of tuples of (synthesized relationships, confidence score) assigned to the column pairs as values. If a synthesized relationship already exists in $S$ for a \textit{value pair}, we take the maximum score.

% \begin{example}
% We now provide an additional example using Table 2 in \cref{fig:synthetic_kb} to make the creation of the synthesized relationship dictionary clearer. 

% Table 2 shares two value-pairs with Table 1 (\textrm{(Kells Park, Spider-Man)}, \textrm{(Eckhart Park, Avengers)} and one value-pair with Table 3, namely \textrm{(Eckhart Park, Avengers)} out of the four value-pairs in consists. In what follows, the value-pair \textrm{(Chopin Park, Trolls)} will be assigned with $RS{(A,B)}$ with a confidence of $\frac{2}{4}$ = 0.5 and $RS{(F,G)}$ with a confidence of $\frac{1}{4}$ = 0.25 in addition to it's original assignment to $RS{(D,E)}$ with confidence 1.
% \end{example}
We merge synthesized relationship dictionary to Relationship dictionary built using YAGO.
% (\cref{fig:yago_indexes}). 
Now using the updated Relationship Dictionary, we can cover all data lake tables and ready to turn our efforts of finding unionable tables given a query table in the next Section.

% In  the example, we only show one column pair for each table. For more column pairs, we process each of them in the same way.

% After processing all data lake tables, we append \textit{synthesized relationship dictionary} to the (YAGO) \textit{relationship dictionary}, which we use during the query phase. \grace{3/17: TODO: edit the transition into section 6}
% As mentioned before, we set synthesized CSCS to 1 and hence, the confidence score of synthesized RS forms synthesized RSCS.  %\aamod{02/18: todo: add the figure showing dictionaries}.
% On what follows, we add each synthesized RSCS to the inverted index as shown in \cref{fig:indexes}. It is interesting to see that although Query table in \cref{fig:synthetic_kb} does not have any value overlap with Table 1, Table 1 still has a non-zero ranking score because of indirect overlap. We will discuss about the query phase in detail in \cref{section:semantic_union_search}.


% iterate through the data lake tables and store occurrences of all value-pairs in column-pairs in a \textit{Lookup Dictionary}. 


% Then, we iterate through this dictionary to annotate each value-pair with relationship semantics and associated confidence scores a

% \introparagraph{Lookup Dictionary Creation} At first, for each data lake table, identify the column pairs in a functional relationship and assign them a synthesized RS. 

% In the meantime, we also record the occurrence of value pairs (not covered by the existing KB) from those column pairs in Lookup relationship dictionary ($L$). 

% L has the value-pairs as key and the set of synthesized RS as value. For example, \textrm{(Kells Park, Spider-Man)}) is a key in L. Also, as it appears in two column pairs having synthesized semantics $RS_{(A,B)}$ and $RS_{(D,E)}$, it has value \{$RS_{(A,B)}$, $RS_{(D,E)}$\}. 
% \grace{3/17: Should we include an in-line example of a lookup dictionary?}

% \introparagraph{Synthesized Relationship Dictionary Creation} 
% Once we create the lookup dictionary, we use it similar to the relationship dictionary (\cref{section:unionability_components}) and annotate the column pairs.
% \begin{example}
% For example, suppose we are processing Table 1 of \cref{fig:synthetic_kb} as data lake table after creation of lookup relationship dictionary. All three values have synthesized relationship $RS_{(A,B)}$ as they belong to the same column pair. Here, (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}) also have synthesized relationship $RS_{(D,E)}$.
% Therefore, we assign both $RS_{(A,B)}$ and $RS_{(D,E)}$ as the synthesized relationship (that is, the synthesized RS) with confidence scores, calculated by Formula x. \grace{TODO: reference formalization above}
% % which is the fraction of unique value pairs mapped in the synthesized RS to the total number of unique value pairs in the column pairs. 
% For Table 1, the confidence score for $RS_{(A,B)}$ is 1.0 and $RS_{(D,E)}$ is $\frac{2}{3} = 0.66$. 
% %With these confidence scores, we define the Synthesized RSCS.
% \end{example}
% Recall that, we assume all \textit{value pairs} in the same \textit{column pair} have the same semantic relationship between them. Also, recall relationship dictionary from \cref{section:unionability_components} (\cref{fig:indexes}) that contains entity pairs as key and the set of tuples of (binary relationships, confidence score) as values. Similarly in synthesized relationship dictionary, we add each value pair in the column pair as keys and the set of tuples of (synthesized relationships, confidence score) assigned to the column pairs as values. If a synthesized relationship already exists in $S$ for a \textit{value pair}, we take the maximum score.

% \begin{example}
% Again consider data lake tables in \cref{fig:synthetic_kb} as an example. 
% After processing Table 1,
% $S$ contains the following three tuples as keys:  (\emph{Brands Park, Moana}),
% (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}).
% All value-pairs now have values: \{$RS_{(A,B)}$: 1.0, $RS_{(D,E)}$: $\frac{2}{3}$\}.

% Next, we process Table 2 in a similar manner, and add/update its value pairs
% (\emph{Kells Park, Spider-Man}), (\emph{Eckhart Park, Avengers}), (\emph{Union Park, Black Panther}), (\emph{Chopin Park, Trolls}) as keys
% and \{$RS_{(A,B)}$: $\frac{2}{4}$, $RS_{(D,E)}$:1, $RS_{(F,G)}$: $\frac{1}{4}$\} as their values to $S$.
% However, as (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}) already have values for $RS_{(A,B)}$ and $RS_{(D, E)}$, we take the maximum scores. 

% So, after processing Table 2, the value for both (\emph{Kells Park, Spider-Man}) and (\emph{Eckhart Park, Avengers}) is 
% $\{RS_{(A,B)}$: 1, $RS_{(D,E)}$:1, $RS_{(F,G)}$: $\frac{1}{4}$\}
% %rjm get an update on their values. 
% %are updated.

% Table 3 is processed in the same way. At the end, the synthesized relationship dictionary is shown in the figure.

% %However, by using our transitive closure, we provide them with a synthesized semantic type from Table 2.
% %\rjm{10/31:  what is "our transitive closure".  Define this formally.  Or leave this out if it is a minor detail.  I suggest the latter given that we don't have time to introduce new concepts this late. }
% %\aamod{10/31: Yes, that just means co-occurrence with neighbooring tables. It's a minor detail. Removed}
% \end{example}
% In  the example, we only show one column pair for each table. For more column pairs, we process each of them in the same way.

% After processing all data lake tables, we append \textit{synthesized relationship dictionary} to the (YAGO) \textit{relationship dictionary}, which we use during the query phase. \grace{3/17: TODO: edit the transition into section 6}
% As mentioned before, we set synthesized CSCS to 1 and hence, the confidence score of synthesized RS forms synthesized RSCS.  %\aamod{02/18: todo: add the figure showing dictionaries}.
% On what follows, we add each synthesized RSCS to the inverted index as shown in \cref{fig:indexes}. It is interesting to see that although Query table in \cref{fig:synthetic_kb} does not have any value overlap with Table 1, Table 1 still has a non-zero ranking score because of indirect overlap. We will discuss about the query phase in detail in \cref{section:semantic_union_search}.

%Similar to RSCS in \cref{section:unionability_components}, we store synthesizd RSCS to the main Inverted Index (S) with synthesized RSCS as key and the tuple of (table name, confidence score) as value as shown in the \cref{fig:synthetic_kb} \aamod{02/18: update the figure reference}.


% \subsection{Reducing the Number of Relationships}
% %\aamod{10/31: trying to start positively :) ! We will move this to discussion or some other sections at the end}

% The synthesized knowledge base stores: 
% %mainly stores two information: 
% the \textit{value pairs} and \textit{synthesized relationship semantics}. %Therefore, there are mainly two areas in which we can optimize our synthetic knowledge base.
% %\subsubsection{Reducing the number of synthesized relationships}
% As shown in \cref{fig:synthetic_kb}, the number of synthesized relationship is equal to the total number of \textit{column pairs} with a functional dependency between them that are not represented in the KB. However, one can merge certain relationships based on  available information. If all value pairs of a smaller column pair are contained in a large column pair, we assign both a single synthesized relationship. For example, in the absence of row (\emph{Freud Museum, Camden}), we would assign a single synthesized relationship, say \texttt{C\_D}, to the column pair in Table (1) and Table (2).
% A step ahead from containment, if two column pairs have high overlap between them, we can merge their synthetized relationships. Precisely, given two column pairs $c_{11} c_{12}$ and $c_{21} c_{22}$ having $n_1$ and $n_2$ $(n_1 \leq n_2)$ unique value pairs respectively. Let there are $g$ unique value pairs that appear in both column pairs. Then,
% %we remove $c_{11} c_{12}$'s synthesized relationship and assign it $c_{21} c_{22}$'s synthesized relationship
% if $\frac{g}{n_1} \geq \eta$, we can assign them a single synthesized relationship. Here, $\eta$ ranges from $0$ to $1$. This optimization is applied just after the creation of lookup table in offline phase.

% \begin{example}
% For example, let us revisit the column pairs of Table 1 and Table 2 of \cref{fig:synthetic_kb}. We see that there are two value pairs:\{\emph{Wallace Collection, City of Westminster}\} and \{\emph{Wellcome Collection, Camden}\}
% overlapping between them. If we consider $\eta = 0.66$, the column pairs in Table 1 and Table 2 will be identified with a single synthetic relationship \texttt{C\_D}.
% \end{example}

%Therefore, we use an inverted index having the synthesized relationship as key and the tuple of \textit{(table name, column pair index, confidence score)} as value as shown in \textit{Synthesized Inverted Index} of \cref{fig:synthetic_kb}.


%\aamod{02/15: This is the old Synthesized KB definition. Grace, please feel free to use it if it makes sense in someway to expand column based definition to the relation-based.}
% \begin{definition}[Synthesized KB]
% If \{$A_1 B_1$, $A_2 B_2 \dots$ ,$A_pB_p$\} $\in \mathcal W_D$ are the unique column pairs having a functional dependency, \{$A_1\_B_1$, $A_2\_B_2 \dots $ ,$A_p\_B_p$\} are the respective synthesized relationships assigned to them and
% \{$a_1b_1$, $a_2b_2$ \dots $a_qb_q$\} $\in \mathcal U_D$ are the unique column value pairs in the entire data lake,
% the synthesized knowledge base for the given data lake is a key-value pair having $a_i\_b_i$  for each $a_ib_i \in \mathcal U_D$ as a key and $\forall key$, a vector $(g_{i1} A_1\_B_1, g_{i2} A_2\_B_2, \dots g_{ip} A_p\_B_p)$as value.
% \end{definition}
% For instance, for a data lake having column pairs \{$A_1B_1$, $A_2B_2$\} and value pairs \{$a_1b_1$, $a_2b_2$ $a_3 b_3$\} , 
% the synthetic KB contains the key-value pairs: $\{a_1\_b_1: (g_{11} A_1 B_1, g_{12} A_2 B_2)\}$, 
% $\{a_2\_b_2: (g_{21}A_1 B_1, g_{22}A_2 B_2\}$,
% $\{a_3\_b_3: (g_{31}A_1 B_1 g_{32}A_2 B_2\}$ respectively.

==> sections/unionability_components.tex <==
\section{Creating Semantic Graph}
\label{section:unionability_components}
% \begin{figure*}[h]
%   \includegraphics[scale = 0.6]{figures/indexes.png}
%   \caption{Examples of different indexes built by SANTOS. Relationship Dictionary, Type Dictionary and Inheritance Dictionary are built using YAGO. Synthesized Relationship Dictionary is appended to Relationship Dictionary. Inverted Index stores Relationship Semantics found in the data lake tables along with their confidence Scores. \aamod{02/18: todo: replace png file with pdf. Also fill rows related to synthesized KB and YAGO with different colors.}}
% \label{fig:indexes}
% \end{figure*}


  

%In the next sections, 
We now introduce two methods that
%the major  annotation components used by SANTOS. 
SANTOS uses to discover relationships. 
%First we discuss in this section how we use an existing knowledge base.  %$This method is described in this section.  
%In this section, we will assume the knowledge-base covers all columns and relationships in the query table and data lake.  
%rejm resolved
%\wolf{10/21: so here it is super crucial to be very precise about how you think about a KB representing relationships (can this all be mapped to the triple formalism?). 
%And how you think about relations being expressed in tables. 
%And how both map to each other.
%In particular, how do the concepts of relations in this paper relate to the definitions in this highly cited survey:
%\url{https://arxiv.org/pdf/2003.02320.pdf}}
%In the next section, we will relax this unrealistic assumption and present a comprehensive annotation solution
%that makes use of a knowledge-base together with the knowledge embedded in the data lake -- an approach we call a {\em synthesized knowledge-base}.  
%\wolf{10/21: emphasize here that the overall approach stays the same (the framework is unchanged), you just instantiate the component of an external knowledge base with a data-driven approach. Thus ideally separate the overall steps that will be followed by *any* future approach you can think of, from particular instantiations in that instantiation of that framework. now, of course, future framework can always extend the supposedly generic framework developed here in some way, but then it is just yet another dimension to that framework here that was discovered later.}
First, 
%\wolf{3/23: In this section,}
we explain how we use an existing knowledge base (KB) \cite{21_hogan_knoweledge_graph_survery} to 
create a semantic graph for a table in this section.
Specifically, we describe how we use a KB to annotate the nodes of the semantic graph 
with a (set of) semantic types from the KB and %to annotate 
the edges of the semantic graph with properties from the KB.  
Then later in \cref{section:synthetic_knowledge_base},
%\wolf{3/23: Then later in \cref{section:synthetic_knowledge_base}, ...}
we introduce a {\em synthesized knowledge base}.
%that we describe in \cref{section:synthetic_knowledge_base}.  
%We also explain how we combine them to obtain the triples for each column pair.
%rjm Aamod is doing this
%\wolf{10/21: suggestion: to create an end-to-end figure that shows the ultimate instantiation of that framework. 
%In particular, what aspects / steps / components are developed in the offline phase, and which in the online phase?
%E.g. I assume the synthesized KB is done offline before a search query is specified}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\linewidth]{figures/cs_and_rs.png}
%   \caption{An illustrative figure showing the information encapsulated by Column Semantics (CS) and relationship semantics (RS) in a table.}
%  %rjm:  what is a "table use"?  As I understand there is a single interpretative for a single KB.
%  %\wolf{10/21: Is the relationship semantics of a table independent of its use? or is the semantics (or reading order) dependent on the use?
% %  Thus, does the same table allow different interpretations? If the latter, you could define the query table as unambiguous with regard to its reading (because you constrain the input enough to avoid ambiguities). But the same datalake table may allow different interpretations.}}
%   \label{fig:cs_and_rs}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[scale =0.6]{figures/Fig_RS_semantics}
%   \caption{An illustrative figure showing the information encapsulated by Column Semantics (CS) and relationship semantics (RS) in a table.}
%   \label{fig:cs_and_rs}
% \end{figure}




% \begin{table*}[t]
% \caption{Table illustrating famous people born in different places and the geographical coordinates}
% \label{tab:city_and_details}
% \begin{tabular}{cccl}
% \toprule
% Place & Geo & Famous Person & Occupation\\
% \midrule
% Boston &42.358333,-71.0625 & James Taylor & Singer\\ 
% Barnet &51.644444,-0.199722 &Anthony Pelissier & Film Director\\
% Qatar &25.26954,51.21277 &Moayad Hassan & Football Player\\
% NYC &40.67,-73.94 &Ivan A. Getting & Physicist\\
% Boston & 42.358333,-71.0625 &Abby May & Social Worker\\
% Dallas &32.779166,-96.808888&Stevie Ray Vaughan & Singer \\
% \bottomrule
% \end{tabular}
% \end{table*}

\input{sections/KB_details}

\subsection{Column Semantics}
\label{section:column_semantics}
% \begin{figure}[t]
%     \includegraphics[scale = 0.55]{figures/sem_illustration.pdf}
%   \captionof{figure}{Column Semantics (CS) and relationship semantics (RS) in a given table
%   \wolf{3/23: best to draw the RS as directed edges, it's an ordered relationship S-P-O}}
% \label{fig:sem_illustration}
% \end{figure}

%Column semantics is one of the important unionability features in SANTOS.
%It is the list of knowledge base types that represent the semantics of the data values in a column.
For determining table unionability,
%inferring the semantics of a table, 
it is very important to understand the semantics 
of its columns.
For this, we seek to associate a set of KB types to each column.
% ~(\cref{fig:sem_illustration}).
%label each text column of table using the KB types as shown in \cref{fig:cs_and_rs}. 
Associating columns with types from a KB is a 
%Labeling a table column is 
well-studied problem~\cite{venetis_11_recovering_semantics,ritze_15_matching_tables_to_dbpedia,zhang_17_tableminer+,hulsebos_19_sherlock,zhang_20_sato}.
%Column semantics are the nodes in the semantic graph.
%rjm right, fixed
%\wolf{10/21: aren't the columns the nodes, but their semantics the interpretation of the relationshipships (may depend on whether you like to formalize in terms of S-P-O triple, or just S-P pairs}
Like previous work on unionability~\cite{nargesian_18_TUS} and column semantic type detection~\cite{hulsebos_19_sherlock,2020_ota_d4}, we are only using values within a column to determine the associated KB types.
However, unlike other approaches in the literature, we make the use of both KB type and the KB type hierarchy to find the column semantics.
Intuitively, we want to assign a type distribution to each column based on the aggregate of the types of individual values in the column. This is based on three objectives: 
(i) \textit{Semantic consistency} i.e., we assign multiple types to a column but all assigned types should be semantically consistent. For example, if a column is assigned a type \textit{place}, it can also be assigned another granular type \textit{city} but not \textit{movie}, which is semantically inconsistent.
(i) \textit{Monotone in input weight} i.e., if a type gets assigned to more values in the column, it should be prioritized over a type assigned to less values. (iii) Rare types in the knowledge base are more informative and hence, should be prioritized over the frequent types (see \cref{section:knowledge_base}). Now we discuss how we fulfill these objectives.

\wolf{3/24: I see, so you use ``semantics'' as synonym for ``type distribution''? 
I'd still suggest to be clear: your idea is to deviate from prio work that determines a mapping froma column to a type (type detection), the goal of this approach is to determine a type distribution. What is a good name (other than semantics):
probabilistic type detection (only if the weights have a clear probabilistic interpretation),
weighted type detection,
type distribution detection,
type distribution assignment,
assigning each column a type distribution
}
\aamod{03/30: Yes, if we say column type detection only, it sounds like we are annotating each column with 1 type with full confidence. However, this is not the case. Therefore, we want to name it differently.}
For a given column, 
%rjm editted
%first we map each column value to the knowledge base 
we first use the \textit{entity dictionary} to map each column value to entities in the KB. Next, we use the \textit{type dictionary} to find a set of types associated with these entities. 
%and find its types.
%In the mean time, 
We then count the number of unique values mapped to each type. 
\wolf{! 3/24: stop here. This becomes a description of a particular algorithm. Please first describe the intuition, the goal of what the algorithm tries to achieve. Some axioms. Something like:

1. we want to assign a type distribution to each column.
2. the idea is do this based on the aggregate values their individual types. 
3. intuitively each value has a distribution, the problem then becomes to somehow aggregate those.
Intuitively, the aggregation should follow certain desiderata:

1. monotone in appearance: If a type appears more often, then higher weight
2. monotone in input weight: if a type gets assigned more for a value, then also the aggregate value higher
3. types that are more discriminative (appear less frequently, or are more specific) should be given higher weight.
4. ???
5. ???

Next we show a `weight distribution assignment' that fulfills all of these 5 desiderata.
}
\aamod{03/30: updated the section and added the objectives before the algorithm. I would be happy to update further.}

Note that the same cell might be mapped to multiple types due to homographs~\cite{21_leventidis_homograph_detection} and the inheritance hierarchy.
%No matter how many types a column value is mapped, each type will get its count increased by 1.
%rjm addressing below \wolf{10/21: this is a design decision that needs to be justified. Currently, a very generic word (with many meanings, say ``the'') can gives many votes, one for each context it appears in.
%The design decision in random walks is that nodes with high outdegree (homographs) can get one total weight vote, but each context gets one over the number of contexts. What is the reason to give homographs basically more votes; shouldn't it the opposite?}
%\wolf{10/21: somewhere early, and ideally with some figures, explain that ''aggregation process''.
%1. each cell, 2. gets aggregated into the column. 3. then the columns relative to each other at the aggregate level get compared for the semantics. An alternative decision could have been that the semantics is determined *for each row* before being aggregated. I agree with the current aggregation, intuitively. Is there a good justification though? Efficiency, or avoidance of ambiguities?}
%Notice, 

%\introparagraph{Assigning Top Level Types}
Next, we shortlist all the top level types that we get from the KB.
Assuming all the top-level types are semantically disjoint \cite{tanon_20_yago}, we argue that a column should have only one top level type.
%\grace{TODO: cite the YAGO paper that claims this} 
%aamod: done!
Ideally, we assume that the KB returns a single top-level type for each column.  However, due to homographs and the deep heterogeneity in data lakes that may lead to a value being mapped to an incorrect entity, we may get multiple top-level types for the same column.
Therefore, we use an unweighted
voting strategy and select only one top-level type that has maximum count among all top level types of the column \footnote{\label{footnote:no_ties} In our experiments, we never encountered "ties" on real data.}.
\wolf{3/24: I see, so this particular algorithm does not assign a distribution but the goal is to determine the most likely (one single) top level domain. I am not exactly sure why this works better in practice / experimentally as suggested below.
Is it that keeping around a (90/10) distribution would introduce more noise than information because the 10\% are more likely to be spurious than useful?}
Thus selected type is considered as a Top-Level Column Semantics (TL$_{CS}$) for that column.
%We experimented with different type selection strategies and found that this unweighted one was the best and that we never encountered "ties" on real data.  

\begin{example}
\label{example:top_type_explanation }
Let us consider, the \texttt{Birthplace} column in Table (c) of \cref{fig:running_examples} having 5 unique values.
%\cref{tab:city_and_details}.
In YAGO type hierarchy, "place" and "creative work" are among the top level types. The value "Boston" is associated with both types.  Hence, the KB returns both types for {\tt Birthplace} column.
%will have both KB types associated with it.  
Notice the majority of the values are only associated with the place type, hence, we will select this as the TL$_{CS}$ for the {\tt Birthplace} column and discard "creative work".
%Also, "administrative area" is the children type of "place" and "film" and "musicComposition" are the children types of "creative work".
%When querying this column in the KB, we recieve the following types excluding the KB root type: \{place, administrative area,  city, country, sovereign state, emirate, creative work, film, musicComposition\}. 
%\wolf{10/21: I found it a bit complicated to follow. What about using the space to the right of Table 4 and showing the relevant excerpt of the hierarchy from Yago. You can draw it in PPTX and make nice highlights and annotations}
%We omitted some granular types like "singleMusic" in this example to keep things simple. 
%However, we handle them in our experiments.
%One can call that this column is about "place" as well as "administrative area" at the same time because "administrative area" is semantically a granular type of "place".
%\wolf{10/21: adm are being a granular type of place, does this mean: place is a more general concept? Place is a super concept? Should it be a more or less granular?}
%However, it cannot be considered as a "creative work" column concurrently 
%even if Boston and New York City are the name of songs and Barnet and Dallas are the name of films.
%Conversely, if one considers this as a "creative work" column, 
%then it is reasonable to call it as a "musicComposition" or a "film" column too but it does not make sense to call it as a "place" column at the same time.
%Hence, assuming we have a well-curated KB type hierarchy, we do not assign multiple top level types to the same column, which the simple counting algorithms in the literature do.
\wolf{3/24: make his a full example:
1. we have 5 different values (I assume you ignore duplicates, please mention).
2. one of them (Boston) maps to two: place and cw. All the other ones mape to place. Thus we get votes:
place 4.5, cw: 0.5 (you giving each value the same number of total votes, right?).
3. thus the algorithm determines place as the top level.

Question: why do you only focus on the top level type, not the more fine-grained ones? You likely would not want to union towns with countries. Alice born in Boston, Bob born in Canada. Leads to union countries with cities.}
\end{example}

%Ideally, we assume that the KB returns a single top-level type for each 
%cell of a 
%column. However, due to homograph and incorrect entity mapping, we get multiple top level types for the same column.
%Therefore, we use 
%\wolf{10/21: a simple unweighted} 
%voting strategy and select only one top level type that has %maximum count among all top level types of the column.
%Thus selected type is considered as a Top Level Column Semantics (TL$_{CS}$) for that column.

\begin{definition}[Top-Level Column Semantics]
Let $T_c \subseteq T$ be the set of types for any column c such that $t \in T_c$ is the type of at least one column data value 
%rjm - let's use data value
%\wolf{10/21: cell value in that column?}
$v \in c$.
\wolf{3/24: Let me clarify: if the value is Boston, then will this value be assigned both place and city, or just city, based on the dictionary? Assume the transitive closure up the hierarchy is *not* encoded in the dictionary (it would be a waste).
But do you then still do find the top one? Thus $t$ is the set of top level hierarchies mapped to by some value? How do you exactly calculat the weight?}
\aamod{03/29: We get boston's type as place, city, state\_capital, creative\_work, movie, etc. However, we only keep the semantics that belongs to the top level type place i.e., this column will be annotate with place, city, state, etc. but not with createive work and movie. We first explained the top-level semantics assignment. Then we talk about how we assign the children types.}
Now, among all $t \in (T_c \cap T_{\mathit{top}})$, $t$ is said to be the Top-level Column Semantics (TL$_{CS}$) for $c$ 
if it is the top level type for the highest number of unique values in $c$.
%rjm right you are and we experiment with this and discussed it at length as you recall - using a TF/IDF inspired score
% since the choice was empirical, let's discuss it in eperiments.
%\wolf{10/21: yet another choice would be weights for each vote in proportion to how often a value appears. So there is a range of possible design choices. It will really pay off to shortly explain the various realistic options you see, and then explain *why* you choose one particular one (or keep two as alternatives, and then let the experiments decide for you? E.g., you could introduce a weighted vote with some log of counts, and let the exponent be learned from data...)}
%\wolf{10/21: suggestion: separate the problem (find out which of several possible top level types is ``the right one") from the actually particular choice you have here (unweighted majority vote).}
For a column c, there can be at most one TL$_{CS}$ and it is represented by TL$_{CS}$(c).
%\wolf{10/21: what if two types have the same vote count? Or more general, if the chosen voting scheme (here majority vote) assigns the same top score to two columns?}
\grace{We can do TL$_{CS}$ or CS$_{TL}$ or Top$_{CS}$}
\end{definition}

%rjm point taken, but let's not change this terminology so late
%\wolf{10/21: I find the use of ``semantics'' in above definition confusing. What is called ``semantics" appears to just be the "most likely type" for an individual column. No semantics = relationshipships between columns used yet. Comes later.}
%\introparagraph{Assigning Children Types}
Once TL$_{CS}$ is determined, we discard all the types that are neither TL$_{CS}$ nor the children of TL$_{CS}$ -- the remaining types
%The rest of the types, together with TLCS 
are the column semantics for the column. This fulfills our first objective.
%rjm no, they will form a tree (DAG depending on KB if it has multiple inheritance) rooted at the TLCS
%\wolf{10/21: so ``semantics'' are here a set of types that form a possibly disconnected subgraph of the knowledge base?}
%rjm I think this is explained clearly above so "recap" not needed
%In summary, for any column c, first we shortlist a set of candidate types $T_c$, where $T_c \subseteq T$.
%Here, any $t \in T_c$ is the type of at least one column value $v \in c$. Next, we find the Top Level Column Semantics TLCS(c). If TLCS(c) = t, we discard any $u \in T_c$ such that u is not a children of t.
%The remaining types are the column semantics of c.

%\rjm{Be consistent, you define TLCS of a column and column semantics of an column!  Why the difference.}

\begin{definition}[Column Semantics]
For a column $c$, a type $t \in T_c$ is said to be in the column semantics for 
%column A 
$c$ if it is either TL$_{CS}$(c) or a descendant  of TL$_{CS}$(c) in the type hierarchy. We represent column semantics for 
%column A by $CS(A)$.
column $c$ using $CS(c)$.
% , as shown in \cref{fig:sem_illustration}.
\wolf{3/24: I am confused: is the focus only on top hierarchies, or any hierarchy? 
I think the explanation so far allows both interpretations}
\end{definition}

\begin{example}
%rjm In \cref{tab:city_and_details}, 
In~\cref{fig:running_examples} (c), the column semantics for the column \texttt{Birthplace} are the set of types:
\emph{\{place, administrative area, city, country, sovereign state, emirate\}}.  The top-level type is {\em place} and all other types are specializations (children) of {\em place}.
\end{example}

Within the column semantics, there may be types with more support (that is, more values associated to them) than others.  This is complicated by inheritance hierarchy (a value that is associated with a type is also associated with all of its supertypes).  In our unionability search, we need to take this into account.  
%\updated{changed example and paragraph below after adding tfidf penalizing.}


\begin{example}
\label{example:confidence_explanation }
Let us return to the {\tt Birthplace} column in~\cref{fig:running_examples}(c).
%\cref{tab:city_and_details}.  
The column semantics includes both city and country.  
% \wolf{3/24: I am confused: didn't Example 5 also include creative work?} \aamod{03/29: No, it was discarded. We only select 1 top level type for each column. Then, the children of only the selected top level types will be assigned to the column with different confidence scores.}
These are siblings in the KB and both children of type {\em place}. Notice however, that only one data value is associated with country while three are associated with city (Barnet is mapped to neither city nor country).
To model this difference, we assign a confidence score to each type in the column semantics by using \textit{type score} and using the type statistics returned by KB.
\wolf{3/24: here I am completely confused: the details here contradict everything what was said before:
1. is the focus on just top or not?
2. why 4 values and not 5? where is creative work?}
\aamod{03/29: There are 5 values. We have one value (Barnet) that is neither country nor city. It is only mapped up to administrative area.}
\end{example}

%rjm rewrote in the example above.
%However, it will be misleading if we consider the column in \cref{example:top_type_explanation } as type "city" and "country" with equal importance because there is just 1 value having type "country" whereas, 3 are of type "city".
%One can easily consider this as a "city" column and discard "country".
%But doing so, we miss few information we have about "country" in the column and we do not want to do so.
%Hence, to tackle with this trade-off and retrieve the granular type 
%\wolf{10/21: more granular, or less granular? or to be less ambiguous: the more specific, or the more general term}
%information in a systematic manner, 
%we assign a probabilistic score to each column semantics that quantifies 
%the wealth of information a column contains about each type.
We name this score Column Semantics Confidence Score, CS$_{\textsc{Conf}}$, and it ranges from 0 to 1.
\wolf{3/24: why not column type score? To be consistent with type detection. 
Conceptually, it is still a type detection, yet with a more careful intermediate aggregation step, and as output a weighted type.}
We start by assigning CS$_{\textsc{Conf}}$ to TL$_{CS}$, which is the ratio of the total number of 
unique column values mapped to TL$_{CS}$ to the total number of unique column values mapped to the knowledge base multiplied by its \textit{type score}.
\wolf{3/24: I can't follow that description of the particular algorithm in text, without first a high-level description of where the journey goes.}
Next, for each children type, we get CS$_{\textsc{Conf}}$ by dividing its count by the total number of unique column values mapped to the knowledge base and multiplying it by the respective \textit{type score}.
Here, count refers to the number of unique column values each type is mapped to.

\begin{definition}[Column Semantics Confidence Score]
Let $CS(c)$ be the column semantics of $c$.
For a type $t \in CS(c)$, 
the column semantics confidence score  (CS$_{\textsc{Conf}}$) of
%a column semantics s of a column c 
$t$ is the ratio of the number of unique data values associated to type $t$ 
%(and none of its subtypes) 
to the number of unique data values in this column that are mapped to the knowledge base multiplied by ts(t).
We represent CS$_{\textsc{Conf}}$ for a type $t$ of column $c$ using CS$_{\textsc{Conf}}$($c,t$).
\end{definition}
\begin{example}
\label{example:column_semantics}
In Table (c) of \cref{fig:running_examples}, the column semantics with their confidence score for all columns are:
[{\tt Person}: \{ person: 1.0 * 0.1605, human: 1.0 * 0.1605 \},
{\tt Occupation}: \{ occupation: 1.0 * 0.2728, profession: 1.0 * 0.3118 \},
{\tt Birthplace}: \emph{ \{ place: 
1.0 * 0.1633, administrative\_area: 1.0 * 0.1720, city: 0.6 * 0.2115, country: 0.2 * 0.2712, sovereign\_state: 0.2 * 0.434, emirate: 0.2 * 0.72 \} , 
}].
Recall that we do not compute the column semantics for numerical columns like {\tt Geo}. 
\end{example}
The assignment of CS$_{\textsc{Conf}}$ to each type fulfills our second and third objectives.
%\wolf{10/21: this would really benefit from a figure that illustrates this process, it is all part of the same running example, thus one figure showing the hierarchy, the counts, the count aggregation, and the final decision and scores}
%\rjm{agreed but let's see if we have time for this.  Zixuan?  Could you do this?}

%rjm:  agree and resolved
%\wolf{10/21: Does the following paragraph belong into the next section?}
%We also take the help of relationship semantics for better entity mapping that eliminates some homographs from the equation.
%For example, we have another column providing the geographical coordinates for the places in \cref{tab:city_and_details}. When we look for the relationship semantics in the KB with Place column values as subjects and Geo column values as objects, only URIs related to the places from the first column would be able to find a relationshipship with the second column.
%This way, we can easily discard URIs that are related with "creative work".
%This increases the gap between the counts of candidate top level types and makes it easier to select one among them.
%Like relationship semantics, we compute the column semantics for both data lake and query tables.

\wolf{! 3/24: An essential idea that appears to be missing in the scoring algorithm is the idea of downweighting ambiguous types.
Say there are 1000 values that are assigned type A. 
And there are other 1000 values that are assigned both B and C.
Then if I understand correctly, the current math gives all three types A, B, C the same weight (the weight is only determined by how often those appear). But shouldn't A have a clearly higher weight? Whenever you assign B, it could also be C and v.v.
So it is less discriminating}
\aamod{03/29: Thinking about this possibility, we experimented with the scoring idea that you suggested. However, we did not find such cases in the real data. Instead we found opposite case in almost all tables as discussed in the example below:
Consider a column about cities having 9 values that are cities and let 1 value is a random noise value that maps to a noisy type, say Arson cases. Now since 9 other are famous cities, they are also the name of movies, products, organizations, etc. For example, Boston is the name of movie (creative work), place, organization, product, etc. Let it maps to 10 such top level types. Consider all other 8 cities map to place but also to 9 other top level types (may be same as Boston or different). Due to this, we get score for place = (0.1 * 9)/10 = 0.09. However, as arson case, although is a noise, maps to a single top level type, it gets a score of 1.0/ 10 = 0.1. In this way, instead of considering the top level type of the column as place, we considered it as Arson cases. To avoid this, we count each type equally first. Later, we select a top level type and handle the hierarchy.
}
\subsection{Relationship Semantics}
\label{subsection:relation_semantics}
%rjm this is arguing from the negative, let's turn this into a positive
%As discussed in \cref{example:intent_column_importance}, the false table unioning occurs when we do not determine the relationshipship between the columns in a table. 
%Furthermore, knowing the column pairs and understanding who are related to one another helps to marginalize the false column unioning.
Given the column semantics, we now present how we compute the SANTOS  
%\wolf{10/21: row semantics suggests at the level of cell values within one row. That is now what is meant here, right?}
relationship semantics (RS).
%\wolf{10/21: ``column relationshipships'' or ``column relationshipship semantics''}
The relationship semantics models binary relationships between columns in a table and are represented as 
%serves as the 
edges in the semantic graph.
%and helps to identify the relationship between columns.
%Given a pair of columns from a table, we map the first column value of each row to the subject and second column value of same row to the object of knowledge base triples.
%Thus obtained predicate is the relationship semantics between two columns.
%Ideally, for an column pair, we assume that each row is mapped to the same predicate in the KB.
%However, in practice, we may get multiple predicates for rows of the same column pair due to homographs \cite{21_leventidis_homograph_detection} and incorrect entity mappings.
%Therefore, we select the predicate that is mapped for the maximum number of rows as a relationship semantics for the given pair of columns.
%\wolf{10/21: hmmm, this paragraph suggests that aggregation first on rows, then aggregation. 
%but before description suggested the aggregation of cell values into columns, and then the semantics. 
%Do you want to use both in parallel and then vote across those two aggregation schemes?}
We begin our discussion with an example.

% \wolf{3/24: Just to get an early intuition: is the RS at the end a forest, or a weighted forest?}
% \aamod{03/29: RS is an edge in the semantic graph.}

\begin{example}
Consider again the table (b) in 
\cref{fig:running_examples} about park and films. We would like to understand if there are binary relationships (properties) in the KB that represent the semantics captured by a pair of columns in a table.  For example, given that the column semantics of {\tt Park Name} includes the KB type {\tt park}, and the column semantics of {\tt Film Director} includes {\tt movie director}, does the KB have a relationship between the types {\tt park} and {\tt movie director} that models the same relationship as the table?  In this example, this is unlikely.  However, the KB may well have a relationship between {\tt movies} (a KB type in the column semantics of {\tt Film Title}) and {\tt movie director}.  In this section, we discuss how we determine if the relationship modeled by a pair of columns in a table likely has the same semantics as a binary relationship in a KB.
\end{example}

%We also take the help of relationship semantics for better entity mapping that eliminates some homographs from the equation.
%F%or example, we have another column providing the geographical coordinates for the places in \cref{tab:city_and_details}. When we look for the relationship semantics in the KB with Place column values as subjects and Geo column values as objects, only URIs related to the places from the first column would be able to find a relationship with the second column.
%This way, we can easily discard URIs that are related with "creative work".
%T%his increases the gap between the counts of candidate top level types and makes it easier to select one among them.
%L%ike relationship semantics, we compute the column semantics for both data lake and query tables.


We compute relationship semantics for every binary pair of string (non-numeric) columns.
%rjm resolved
%columns 
%\wolf{10/21: columns?}
%of the table provided that the column mapped to subject is a string column.
%This is because the relationship with numerical value as a subject is ambiguous and generally not found in the KB. 
%rjm mentioned earlier in column semantics
%rjm resolved
%\wolf{10/21: this limitation (or restricted focus) comes a bit late. Better to very early classify columns as one of two types: string or numerical (is there a third? Likely yes: example: URLs, or pictures, etc.; just classify those as other). And state early as justifiable limitation = the focus of your work on strings (not in later sections)
%}
%If both columns are string columns, we find the predicates in both direction.
The relationship semantics is computed for both query and data lake tables. Note that many pairs of columns (like {\tt Park Name} and {\tt Film Director}) may not have a semantic relationship represented in the KB.  Intuitively, there is at least an indirect relationship between all columns in a table (in this case, the director of a film shown in the park), but in this section, we are only interested in relationships represented in the KB.
%every pair of columns may not have a semantic relationship between them. They may be the properties of other columns. For such column pairs, we do not get any relationship semantics.
Suppose columns $c_1$ and $c_2$ in table $D$ have non-empty column semantics, meaning some of their values have been associated with entities in the KB.
To determine relationship semantics, we determine if a pair of values in $\Pi_{c_1,c_2}(D)$ are associated with entities $(e_1,e_2)$ that are in a KB relationship $p$.


\begin{definition}[Relationship Semantics]
\label{def:rs}
Let $P$ be  the set of all binary relations (or predicates) in the KB.
%rjm No, it has properties between relations - YAGO actually has some ternary relations too, but we aren't using them yet!
%\wolf{10/21: I thought the KB only consists of types and their IsA relationships to instances?}
%a pair of columns $A_1$ and $A_2$ having
Let $p \in P$ be a relationship between types $t_1$ and $t_2$.  Let 
$c_1$ and $c_2$ be columns in a table whose column semantics include $t_1$ and $t_2$, respectively.
%values $v_1, v_2 \dots v_n$ and $w_1, w_2 \dots w_n$ respectively 
%\wolf{10/21: since here set semantics is assumed (ignoring duplicates), two columns may have different numbers of elements.
%What you like is DISTINCT(A1, A2), thus the distinct pairs}
%where, 
%$n$ is the number of rows in the table, 
%rjm resolved by removing n
%\wolf{10/21: wasn't $n$ used as number of tables earlier? It would be good to have a small notation table at the very end.}
% Suppose
%$p \in P$ is said to be 
%the relationship semantics for $c_1$ and $c_2$ 
%rjm it is not symmetric, but it is not directed
%\wolf{10/21: since you assume a non-symmetric, directional semantics, maybe better to call 
%``semantics from $A_1$ to $A_2$ (shown as $A_1 \xrightarrow{p} A_2$)''}
%if the maximum number of rows in \{$A_1, A_2$\} 
%rjm:  I've done this, resolved.
%\wolf{10/21: introduce this (or a variant thereof you have seen in a different paper) early as notation for projection on a subset of columns}
If there exists a pair of data values in $\Pi_{(c_i,c_2)}(D)$ where the values map to entities $(e_1,e_2)$ in $t_1$ and $t_2$, respectively, and the pair $(e_1,e_2) \in p$, then we say the $p$ is in the relationship semantics of $\Pi_{(c_i,c_2)}(D)$.
%are mapped to the KB with $A_1$ being a string column, $v_i \in A_1$ as a subject, $w_i \in A_2$ as an object and $p \in P$ as a predicate. 
	% or in the opposite direction
	% i.e., $A_2$ being a string atribute, $w_i \in A_2$ as a subject, $v_i \in A_1$ as an object and $p \in P$ as a predicate.
%rjm resolved
%\wolf{10/21: removed the opposite direction, that's redundant. You can always relabel A1 and A2}
%We represent relationship semantics between $A_1$ and $A_2$ by $RS(A_1, A_2)$. 
%\wolf{10/21: shouldn't the notation also include $p$? Like $p(A_1, A_2)$, or $RS(A_1, A_2, p)$}
%For a pair of columns, there can be at most two relationship semantics-- one in each direction.
%\wolf{10/21: suggestion to define everything in terms of a directed pair $(A_1, A_2)$ instead of a set $\{A_1, A_2\}.$}
If there is more than one KB relationship $p$ that qualifies, then  $p$ with the most associated pairs is used as the relationship semantics. We denote the Relationship Semantics between column pair $(c_1, c_2)$ using $RS(c_1, c_2)$.
% , shown in \cref{fig:sem_illustration}.
\end{definition}
%\updated{aamod 02/19: \cref{def:brcs} is added to fill the void in \cref{eq:unionability_score}. Accordingly, \cref{def:rscs} is updated.}
\begin{definition}[Relationship Predicate Confidence Score]
\label{def:brcs}
The Relationship Predicate Confidence Score (RS$_p$) for binary relationship p of $\Pi_{(c_i,c_2)}(D)$ is the fraction of the number of unique rows in $\Pi_{c_1,c_2}$ mapped to type RS($c_1,c_2$) 
to the total number of unique rows in $\Pi_{c_1,c_2}$. We denote it using $RS_p(c_1,p,c_2)$.
%rjm resolved
%\wolf{10/21: ``is the fraction of the number of unique rows in $\Pi_{A_1,A_2}$ that are mapped to type RS($A_1,A_2$). ''}
%We represent RSCS for $RS(A_1,A_2) = R$ using $RSCS({A_1,A_2})_R$.
\end{definition}
\begin{example}
\label{example:rscs}
In Table (c) of \cref{fig:running_examples}, the Relationship Semantics for (\texttt{Person}, \texttt{Birthplace}) is $RS(\texttt{Person}, \texttt{Birthplace})$ = \texttt{birthplace} and RS$_p$(\texttt{Famous Person}, \texttt{birthplace}, \texttt{Birthplace}) = 1.0.
\end{example}
Finally, we combine CS and RS to get Relationship Semantics Confidence Score (RS$_{\textsc{Conf}}$) as we define next.
\begin{definition}[Relationship Semantics Confidence Score]
\label{def:rscs}
The Relationship Semantics Confidence Score, RS$_{\textsc{Conf}}$, of a column pair $\Pi_{(c_i,c_j)}(D)$ with $CS(c_i) = t_i$, $CS(c_j) = t_j$ and $RS(c_i, c_j) = p_{ij}$ is given by $CS_{\textsc{Conf}}(c_i, t_i) * RS_p(c_i, p_{ij}, c_j) * CS_{\textsc{Conf}}(c_j, t_j)$. It is denoted using RS$_{\textsc{Conf}}$($c_i.t_i, p_{ij}, c_j.t_j$).
%rjm resolved
%\wolf{10/21: ``is the fraction of the number of unique rows in $\Pi_{A_1,A_2}$ that are mapped to type RS($A_1,A_2$). ''}
%We represent RSCS for $RS(A_1,A_2) = R$ using $RSCS({A_1,A_2})_R$.
%The pair containing the relationship and confidence is called $RSCS(c_1,p,c_2)$.
\end{definition}
\begin{example}
\label{example:rscs}
In Table (c) of \cref{fig:running_examples}, {\tt (person, birthplace, city)} is RS$_{\textsc{Conf}}$ for ({\tt Person}, {\tt Place}) and RS$_{\textsc{Conf}}$({\tt person, birthplace, city}) = $1.0 * 0.1605 * 1.0 * 0.6 * 0.2115$.
%we get for \{Place, Geo\} 
%i.e., $\Pi_{0,1}$ 
%\wolf{10/21: mention somewhere early in the formal setup that you may change algebra between named an unnamed perspective if opportune from the context}
%is "geo",
%\{Place,Famous person born\} i.e., $\Pi_{0,2}$ is "birthPlace" and for \{Famous person born, Occupation\} i.e., $\Pi_{2, 3}$ is "hasOccupation".
%We do not find relationship semantics for \{Place, Occupation\} as they are not related to each other semantically.
%Although we query in both directions, we found the relationship semantics for each pair in single direction only. As same relationship was found for all rows, 
%$RSCS(0,1)_{geo}$ = 1.0, $RSCS(0,2)_{birthPlace}$ = 1.0 and $RSCS(2, 3)_\mathit {hasOccupation}$ = 1.0.
%\wolf{10/21: never write text in match directly. But rather use $\mathit{hasOccupation}$ instead of $hasOccupation$, it looks nicer}
%In summary, for \cref{tab:city_and_details}, the relationship semantics with their confidence score are : \{geo-1.0, birthPlace-1.0, hasOccupation-1.0\}.
%\wolf{10/21: this last sentence is strange because it does not mention the pairs and the direction of those ``relationships''}
\end{example}
We compute RS$_{\textsc{Conf}}$ for both data lake tables and query tables. For data lake tables, we store RS$_{\textsc{Conf}}$ in an inverted index
%as shown in \cref{fig:indexes} 
where, ($c_i.t_i, p_{ij}, c_j.t_j$) is key and the set of tuples of (table name, RS$_{\textsc{Conf}}$($c_i.t_i, p_{ij}, c_j.t_j$)) is value. Recall that, a column may have more than 1 Column Semantics. Hence, there may be multiple RS$_{\textsc{Conf}}$ for a column pair. We store all of them in the inverted index and use one that contributes maximum score during query time which we will discuss in \cref{section:semantic_union_search}. Before we do this, 
%we the following sections 
we detail the computation of relationships that are not in the KB.
 
%\rjm{I've removed 4.4 on subject column semantics since this was covered in Sec 3.1 - it is just a column selected by a user in the query table and its column semantics, right?}
%\aamod{10/30: Yes!}
%rjm - yes i would add c-unionability!
%\aamod{10/21: Regarding definition, shall we also include the unionability scenarios anymore?  The diagram that was showing the importance of relationship by differentiating between crime name and museums (crime name to be changed). Also, let's define c-unionability for SANTOS too?}

%rjm added 10/31
% Given the column and relationship semantics, we can now define SANTOS unionability.  We say that two columns with the same column semantics {\em match} and similarly, two relationships between matching columns whose relationship semantics are the same also {\em match}.  So any data lake table with a column matching the query table's intent column and  at least one matching relationship that includes the intent column is considered to be SANTOS unionable.

% \begin{definition}[SANTOS Table Unionability]
% \label{definition:santos_unionability}
% Let $Q$ be a Query Table with intent column $Q.I$ and 
% property columns $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ having relationship semantics $RS(Q.I, Q.P_1)$, $RS(Q.I, Q.P_2)$ \dots $RS(Q.I, Q.P_m)$ respectively. 
% In addition, let $D$ be a data lake table with columns $D.c_1$, $D.c_2$ $\dots$ $D.c_d$. 
% $D$ is \emph{SANTOS unionable} with $Q$ if $D$ (1) contains a column $D.c_i$ such that $D.c_i$ has the same column semantics of $Q.I$, (2) has at least one column $D.c_j$ ($i\neq j$) such that $D.c_j$ has a column semantics of some property $Q.P_k$ and (3) has $RS(D.c_i, D.c_j) = RS(Q.I, Q.P_k)$.
% \end{definition}

%ak added on 1/21/22 (after vldb):
%\updated{Aamod 03/09: Whole paragraph below is new text. Also, I remove old definition completely and moved the paragraph below definition to section 6 just below santos top -k search definition.}


%rjm added 10/31
% Later, we present a scoring function that uses not just the column/relationship semantics, but also the confidence scores to rank how unionable different data lake tables are.  The scoring function will favor tables with more matching relations.  Before we do this, we consider how to compute column (relationship) semantics for columns (relationships) that are not in the KB.

% \begin{definition}
% A Data lake Table $\mathcal{D}$ is SANTOS unionable with a Query Table $\mathcal Q$ having a subject column $Q.S$ and its properties $Q.P_1$, $Q.P_2$ \dots $Q.P_m$ if $\mathcal{D}$ contains the a column having same column semantics of $Q.S$ and at least one property column 
% \end{definition}
% In simple words, \emph{a Data Lake Table D is \emph{SANTOS Unionable} with a Query Table Q if D contains the subject column of Q and at least one property column of Q having same relationship with the subject column.}
%\subsection{Subject Column Semantics}
%Since we do not have subject 
%\wolf{10/21: intent or subject?}
%column marked in the data lake tables, the subject column semantics is computed for the query tables only.
%
%\begin{definition}[Subject Column Semantics]
%A column semantics $t \in CS(A)$ for an column A of the query table Q is said to be a subject column semantics if column A is the subject column. We represent subject column semantics for subject column I using IS(I). 
%\wolf{10/21: why change in notation from A to I? And why does the column semantics for a particular column need a separate formal definition?
%Column semantics seem to be defined (in the current definition) just based on the column, not the relative relationships? }
%\end{definition}
%
%Note that each subject column semantics is provided with a confidence score similar to CSCS. 
%We call such score as Subject Column Confidence Score (SCCS). 
%For a subject column I, we represent SCCS for subject column semantics t by SCCS($I_t$).

%\subsection{Triple Formation}\label{section:triples}
%\rjm{I don't understand this subsection, there is no definition of a triple, can we remove this subsection?}
%After we compute relationship semantics and column semantics for a data lake table, we combine them to get the triples for each column pair having relationship semantics. Note that we form the triples of semantics on meta data level. These triples will be used to construct the semantic graph for the data lake table on query time. As the column pairs from the query table and the data lake table can match in different granular levels, we want to form the triples at every granular levels so that we do not miss any matches on the query time.
%Conceptually, to compute the triples of column pairs ($A_1$, $A_2$), we have a three-columned table with $A_1$'s column semantics in the left column, relationship semantics between $A_1$ and $A_2$ in the middle column and $A_2$'s column semantics in the right column. 
%Now, we take the cartesian product between these three columns, which gives all the triples for that pair of columns. 
%Another way of combining these triples will be to take the cartesian product between the semantics from same levels only. 
%However, since we may not find the semantics up to same level for every columns, we form the triples in all levels.
%Furthermore, each triple is provided with a confident score which is the product of the column semantics and relationship semantics scores of the individual components.
%We will explain the intuition behind this score in \cref{section:semantic_union_search}.

%\aamod{10/12: Alternatively, we can also form the triples in specific levels taking the cartesian products on the specific levels only. For example, keep: person-birthplace-location and president-birthplace-city but not person-birthplace-city or president-birthplace-location}.

% \aamod{The tuple of bag of words in not required anymore as we already formed the triples in pre-processing phase}
% \subsection{Tuple of bag of Words}
% After we compute relationship semantics, column semantics and intent column semantics for a table, we store them in a bag of words which we call as Tuple of Bag of Words (TBW).
% TBW is the semantic summary of a Table.
% It contains two sub-bags for the data lake tables namely Column semantics Bag containing the column semantics along with CSCS and relationship semantics Bag containing the relationship semantics.
% For query table, we have an extra sub-bag called Intent Column Bag that contains the intent column semantics along with SCCS.
%\begin{example}
%\label{example:tbw}
%Some triples and their score for \cref{tab:city_and_details} are:
%(place-geo, 1.0), (administrative\_area-geo, 1.0), $\dots$, (emirate-geo, 0.2), (place-birthPlace-person, 1.0), $\dots$, (physicist-hasOccupation-profession, 0.166). Since we do not compute the column semantics for the numerical columns, the triples formed between columns Place and Geo has only two semantic tokens in the triple. As we compute triples in same manner for both query and data lake tables, it will not make a difference while we make the comparison.
%\end{example}
%\wolf{10/21: I can't follow here. Maybe the shortened notation that leaves out the triples explicitly? Maybe a figure would really help here}

%After processing each data lake table, we store the triples in an inverted index having triple as a key and the list of tuples containing table name, related column pair and the confidence score as a value.
%e use these triples in the query time to generate the semantic trees for the data lake tables.
%Hence, the top-k unionable tables for a Query table Q is obtained by comparing its TBW with that of each data lake table.
%We will discuss about the comparison and ranking details in \cref{section:semantic_union_search}.

==> sections/unionability_definition.tex <==
\subsubsection{Unionability Definition Revisited}

We now revisit the definition of unionability and introduce \unionability. 

\begin{definition}[SANTOS Table Unionability]
\label{definition:santos_unionability}
Let $Q$ be a Query Table with the semantic tree $T$ containing a subject attributes $Q.S$, and additional 
property columns $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ having relations $Q.r_1$, $Q.r_2$ $\dots$ $Q.r_m$ with $Q.S$ respectively. %resolved
%\wolf{10/27: what are those relations? Q.S entry is S, Q.Pi header %is P, Q.Pi values is O?
%What about using m for the number of columns, and thus $P_{m-1}$ being the max?}
In addition, let $D$ be a data lake table with columns $D.A_1$, $D.A_2$ $\dots$ $D.A_n$. 
\wolf{10/27: you also use $n$ later for number of tables; best here to use $k$ or so. Also would $T$ easier than $D$ for table?} \aamod{10/28: T is used later on for the set of KB types.}
$D$ is \emph{SANTOS unionable} with a Query Table $Q$ if $D$ (1) contains a column $D.A_i$ such that $D.A_i$ is unionable with $Q.I$, (2) has at least one column $D.A_j$ ($i\neq j$) such that $D.A_j$ is unionable with some property $Q.P_k$ and (3) has relation between $D.A_i$  and $D.A_j$ that corresponds to $Q.r_k$.
\end{definition}

%resolved
%\wolf{10/27: above definition relies on an earlier definition of what it means for two columns to be unionable.
%It also requires a formal definition of relation.}


In simple words, \emph{a Data Lake Table D is \emph{SANTOS Unionable} with a Query Table Q if D contains the subject column of Q and at least one property column of Q having same relationship with the subject column.}

Our definition naturally provides a way of ranking the tables with a continuous unionability score that we will discuss later in \cref{section:semantic_union_search}.

% \begin{definition}[SANTOS Table Unionability]
% Let, $Q$ denotes a Query Table and $D$ denotes a Data Lake Table. Let, $Q.I$ be the subject column of $Q$ and $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ be its properties having relations $Q.r_1$, $Q.r_2$ $\dots$ $Q.r_m$ with $Q.I$ respectively. A data lake table D is SANTOS unionable with a Query Table Q if D contains a column $D.I$ such that  $D.I$ is unionable with $Q.I$ and has at least one $D.P_i$ such that $D.P_i$ is unionable with $Q.P_i$ and has relation $r_i$ with $D.I$ where, $i = 1, 2, \dots m$.
% \end{definition}
% Our definition naturally provides a way of ranking the tables with a continuous unionability score that we will discuss later in \cref{section:semantic_union_search}.



% \subsection{\unionability}\label{section:unionablity_def}
% \roee{shouldn't this be included in the next subsection? I think that this section should contained processing information of data lake tables (above) and query tables (here) without referring to the way we account for their unionability, which is introduced in the next section: Then Q and D are considered unionable only if the D's semantic tree (1) contains a node of the same type as the intent column and
% (2) there is a large number of matches between their children as well.}

% In order to solve the problems seen in searching for the unionable tables, we introduce a notion of \unionability.
% We now revisit the definition of unionability and introduce \unionability. 
% \wolf{10/21: what about calling this just ``semantic unionability'' to separate the approach (using relationships = semantics of tables) from the name of one particular instantiation of a system that uses semantics (SANTOS)} \roee{The reason we need a ``new'' name is that the TUS paper uses the term ``semantic unionability'' and it is diffrent from what we describe in this paper}



% \begin{definition}[\unionability]
% A data lake table D is unionable with Query Table Q if D contains the subject column of Q and as many property columns of Q with same relations as possible. 
% \wolf{10/21: what are ``relations'' here exactly? 
% You see, S-P-O are between instances: S and O are usually cell values, P are either 1. column names (or if missing the abstract concept for which there are instances, or 2. table names as a whole [like in a binary table]. }
% In worst case, 
% \wolf{10/21: better no ``worst cases" for formal definitions: better to define concepts binary: yes or now}
% D must contain the intent column of Q and at least one property column from Q with the same relation.
% \zixuan{as many property as possible here looks confusing. I prefer to rewrite this to: "A data lake table D is unionable with a Query Table Q if D contains the intent column of Q and at least one property column from Q with the same relation." Then if we want to show the concept of unionability score which is if D contains more property columns of Q, then D gets higher unionability score, we may need to propose a new definition.}
% \end{definition}

% \roee{suggested definition:
% \begin{definition}[\unionability]
% Let $Q$ be a query table with the subject column $Q.S$ and set of its properties $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ having relationship with $Q.S$. A data table $D$ is SANTOS unionable with $Q$ is it has the same subject column as $Q.S$ with at least one property from $Q.P$.
% \end{definition}}
% \aamod{10/22: @Roee, this definition looks good and we were using it before. But it missed the relation semantics part. This will consider president-birthplace-city and president-deathplace-city as same which we don't want. We need to somehow preserve the relationship between the columns.}

Hereafter, whenever we say unionablity, we mean \unionability \ unless mentioned otherwise. The formal definition refer to the minimal conditions for \unionability. However, in practice, we wish to find unionable tables that contain the same subject column as the query table and \emph{as many properties with same relation as possible}.

\aamod{10/25: I would advocate to move the definition of SANTOS Problem below either to \cref{section:semantic_union_search} so that we can also include the scoring function details or to section 1 and make it generic.}

Next, we define the problem of searching for the unionable tables formally.

\begin{definition}[Semantic Table Union Search (SANTOS) Problem]
Given a set of Data lake Tables $\mathcal{D}$ = \{$D_1$, $D_2$, \dots $D_n$\}, 
% \wolf{10/21: better replace x as variable with m or n for a constant}
a Query Table $Q$ with a subject column $Q.S$, a knowledge base $\mathcal{K}$, a positive integer $k$ and a scoring function $f(\mathcal D, Q, Q.S, \mathcal K , k)$ such that $k\leq n$, SANTOS problem is to search for the top-k Data lake Tables that are unionable with $Q$.
\end{definition}

\wolf{10/27: Above definition requires a scoring function by which one can rank}


% \begin{definition}[Semantic Table Union Search (SANTOS) Problem]
% Given a set of Data lake Tables \{$D_1$, $D_2$, \dots $D_x$\}, 
% \wolf{10/21: better replace x as variable with m or n for a constant}
% a Query Table Q, an intent column I marked in the Query Table and a positive integer k such that $k \leq x$, SANTOS problem is to search for the top-k Data lake Tables that are unionable with Q.
% \end{definition}

\wolf{10/21: suggestion: would it makes sense to first define early the table union search problem, without any mentioning of concepts from this paper. E.g. table union search is defined as INPUT: query table, repository, k. OUTPUT: top-k tables that are 1. most unable 2. independently (thus they are not integrated together, just added independently: that seems to be the definition here. Then explain that 1. they key problem is to design a good metric of ``most unable''. Earlier work tried to do this just based on pairwise column comparisons and then aggregating those individual pairwise comparisons into an overall score. This work suggest and *improved* measure that also takes into account the relative relations among columns (thus input is not just sets (or bags) of words = column independently: a table is a set of columsn, but rather, the 2nd dimensions: rows}
\roee{I think we can go either way. Have an intuitive discussion about unionability and why earlier work is different and formally define it here.} \roee{In addition, the problem definition here is different since we require a subject column being annotated in the query table}

\aamod{10/19: In the definition of SANTOS problem above, Should we also consider knowledge base as a given entity?}

\roee{In the reminder of the Section we can decide if we want to elaborate more on the way we solve the problem before we actually solve it (n the populated text), have a more formal discussion with respect for example to the semantic web community or provide steps for actually applying the unionability (second comment be Wolfgang). @Aamod, after reading the section again, try to say what is expected here. It may also be a short description of what we aim to do in the reminder of the paper in this context: `` In the following sections we suggest KB to generate semantic trees for tables, then we..."}

Once a user provides \emph{Q} marked with subject column \emph{I} and its properties, 
we represent it in the form of a semantic tree as discussed before.
\wolf{10/21: really needs an intuitve annotated figure. It seems there are two perspectives:
1. the triples: S-P-O at the instance level: S and O are from cell values, P are from a column as a whole
2. a binary representation: S-P1, S-P2: S here is the column of the individual subjects. Pi are the columns as a whole. 
It seems obvious that way, but by explicitly mentioning these different views, it will help people say from the sematnic web community (where everything is S-P-O) to follow along}
After that we extract all the data lake tables containing the subject column and at least one of its properties. 
Next, we project out the matching columns with the query table and form a semantic tree for the data lake table. 
Finally, we compare two semantic trees and determine the unionability score.
\wolf{10/21: those are 4 steps that may be numbered, named 
(1. query table interpretation, 2. candidate table filtering, 3. candidate table interpretation,
4. candidate table scoring), and then later referred to again in more detailed.
Question: do you envison that *every* implementation of a table union search paradigm needs to follow these 4 steps 
(thus this is generic, and only the measure for 4 is new), or was there already some design decison made to choose that process instead of any other one can come up with?}

It is not always accurate to use the attribute names or the attribute values to create the semantic trees. 
For example, \texttt{Name} in \cref{fig:entity_films} and \texttt{Film Title} in \cref{fig:relation_parks_films} have different attribute names and attribute values although they are unionable. 
Conversely, there can also be the attributes having same name but different semantics. 
For instance, attribute \texttt{Name} of table in \cref{fig:entity_films} represents \textit{film name} whereas, attribute \texttt{Name} of Table (b) in \cref{fig:crime_and_musuem_tables} represents the name of the museums. 
Also, all the open data lake tables may not have the attribute name information. Therefore, instead of using such weak signals, we use a knowledge base to annotate the semantic graphs.
\wolf{10/21: important distinction: do you perform that labeling based on column names only, or rather by also looking at the cell values in a column, or even by looking at the values in a column you like to label and also the neighboring values or column names (because of increased signal from the 2nd dimsion of tables)?}
\aamod{10/25: We use values in the column together with its neighboring values.}
More precisely, we use knowledge base types to annotate the nodes and Knowledge base properties to annotate the edges. If the entities are not covered by the knowledge base, we also take a help of a synthetic knowledge base to annotate the query table that we create using the data lake tables.
During query time, we compare the number of matching annotations between the query table and the data lake tables to determine the unionability score. We will explain the annotation details in \cref{section:unionability_components}, synthetic knowledge base in \cref{section:synthetic_knowledge_base} and unionability score in \cref{section:semantic_union_search}.


==> sections/unionability_details.tex <==
%rjm \section{Preliminaries}
\section{Relationship Unionability}

We now introduce the building blocks of SANTOS (SemANtic Table uniOn Search).
SANTOS performs unionability based on not just the semantics of
%columns
columns ({\em column semantics}),
%rjm ~\cref{section:column_semantics}), 
but also the semantics of binary relationships between
%attributes
columns ({\em relationship semantics}).
%rjm~\cref{subsection:relation_semantics}).  
We now show how we model these semantics.


\introparagraph{Column Semantics}
Like previous approaches to semantic annotation or column-type discovery in data lakes~\cite{2020_ota_d4,hulsebos_19_sherlock,zhang_20_sato}, we will attempt to associate each column with a semantic annotation (for example, a class or type).
This may be a type in a KB or sometimes (particularly when using unsurpervised techniques~\cite{nargesian_18_TUS,2020_ota_d4}), we may determine that a set of columns have the same, but unknown semantics (for example, they are {\em attribute unionable}~\cite{nargesian_18_TUS}).   Hence, we call this {\em column semantics} rather than column type.  As an example, even if our KB does not include Park information, we may still be able to determine that the first columns of Table~\cref{fig:running_examples}(a) and (b) share the same (but unknown) semantics.  
%Of course, we do not require that every column be assigned semantics (that is, the column semantics for a column $c$ may be empty).  
%rjm As the discovery process is uncertain, we assign a column semantics confidence score (between zero and one) to each column with a non-empty semantics.  
%This may be a type in a KB or sometimes (particularly when using unsurpervised techniques~\cite{nargesian_18_TUS,2020_ota_d4}), we may determine that a set of columns have the same, but unknown semantics (for example, they are {\em attribute unionable}~\cite{nargesian_18_TUS}).   
We call this {\em column semantics}.
As the discovery process is uncertain, each \ak{{\em \type} in the column semantics} is associated with a confidence score.



%Of course, we do not require that every column be assigned semantics (that is, the column semantics for a column $c$ may be empty).  
%rjm As the discovery process is uncertain, we assign a column semantics confidence score (between zero and one) to each column with a non-empty semantics.  
%This may be a type in a KB or sometimes (particularly when using unsurpervised techniques~\cite{nargesian_18_TUS,2020_ota_d4}), we may determine that a set of columns have the same, but unknown semantics (for example, they are {\em attribute unionable}~\cite{nargesian_18_TUS}).   
%Unlike previous approaches, our approach allows the {\em column semantics} to contain 
%a
%tree of
%types related by an ISA relation \cite{21_hogan_knoweledge_graph_survery}. 
%rjm let move to Sec 4 on our yago-specific instantiation of these concepts
%\ak{
%The types in ISA relation forms a type hierarchy with a root type. The direct descendants of the root type are called \em{Top level types} denoted by $T_{top}$.}
%The ISA relation may be modeled in a KB or discovered though a learning process. 
%As the discovery process is uncertain, each {\em type in the column semantics} is associated with a confidence score.  

%\renee{Moved Grace's definition from alt\_unionability\_components forward with some tweaks.  I suggest leaving the top level type discussion for the next section on "our" instantiation of these definitions.}

%rjm macro so we can change the notation
\begin{definition}[Column Semantics]
\label{def:cs}
%For a column $c$ in a table $\dltable$, its column semantics is
%a type $t$
%a set of types.
%rjm as we discussed, this is not a distribution.
%that captures the semantic distribution of its values.
%the hierarchy of 
%a list of types $t_1,  \dots t_\tau$.  If $\tau > 1$ then for all $i$ $t_i$ ISA $t_{i+1}$. 
%a tree $CS(c)$ of types related by ISA relationships with root $t_r$.\footnote{This can be easily generalized for KBs that permit multiple inheritance.}
%Column semantics for
\ak{We denote the column semantics 
for 
column $c$ in a table $\dltable$
%is a set of annotations and we denote
using $CS(c)$ and each \type $a \in CS(c)$ has a confidence score that ranges from 0 to 1.
}
\grace{4/8: is it also a set of column annotations, like relationship semantics?}
%\grace{4/5: I thought we discussed that this isn't true (scores sum to one or less -- scores can sum up to greater than 1)}
%\aamod{resolved}
\end{definition}
%rjm I addressed this and removed distribution
%\renee{4/6:  don't use the word distribution if it is not a distribution.}

\begin{example}
\label{ex:columnsemantics}
Consider Table (b) of \cref{fig:running_examples}, the column semantics for the column \texttt{Park Name} may be \{\textit{Place, Tourist Attraction, Park}\} and for \texttt{Film Title} may be \{\textit{Creative Work, Movie}\}.
\end{example}
% \rjm{
% \begin{definition}[Column Semantics]
% \label{def:cs}
% For a column $c$ in a table $\dltable$, its column semantics is a distribution over 
% %the hierarchy of 
% %a list of types $t_1,  \dots t_\tau$.  If $\tau > 1$ then for all $i$ $t_i$ ISA $t_{i+1}$. 
% a tree $CS(c)$ of types related by ISA relationships with root $t_r$.\footnote{This can be easily generalized for KBs that permit multiple inheritance.}
% We denote the column semantics for 
% column $c$ using $CS(c)$. Each type $t \in CS(c)$,  has a  confidence score  where these scores sum to one or less.
% \end{definition}
% }

%rjm \ak{ alternative definition:
%rjm \begin{definition}[Column Semantics]
%rjm\label{def:cs}
%rjmFor a column $c$ in a table $\dltable$, its column semantics is a distribution over 
%the hierarchy of 
%rjma set of types $t_1, \dots t_\tau$. If $\tau > 1$ then there exists a type $t_j$ such that $t_j \in T_{top}$ and for all $i \ne j$, $t_i$ is the descendant of $t_{j}$. We denote the column semantics for
%rjmcolumn $c$ using $CS(c)$. Each type $t \in CS(c)$,  has a  confidence score  where these scores sum to one or less.
%rjm\end{definition}
%rjm }

%rjm:  let's be sure we never say just semantics but qualify it by col/rela to address this comment
%\wolf{3/23: 1. currently ``semantics'' appears to be used both for the type of a column, and for the relationships across columns.
%2. would it be cleaner to clearly differentiate those: the former called ``type detection'' instead of ``semantic [something]''
%with a footnote that some prior work uses the word semantics for type detection, while this paper suggests to use semantic as the 
%relationships between columns?  Maybe not.
%The former is a very restricted relationship. COLUMN IsInstanceOf TYPE.}
%\aamod{03/30: Column type detection might sound like annotating each column with 1 type. However, we are doing it differently. Hence, we want to distinguish it from type detection.}

\introparagraph{Relationship Semantics}
In addition to column semantics used in previous table union search approaches~\cite{nargesian_18_TUS,2020_bogatu_d3l}, we use relationship semantics to guide the search.  Each pair of columns may have at most one relationship with a confidence score.\footnote{\rjm{Note when using a KB, there may be more than one name for a relation (for example a name for both the relation and its inverse), but we only permit one mathematical relation to be assigned to a relationship, even if it has multiple names.}}
% \grace{4/4: Is this true? For instance, although we have undirected edges for relationships now, it can technically be two relationships: Movie directedBy Director vs. Director directed Movie}
% \renee{addressed this by adding a footnote.  inverses are different names for the same mathematical relation.}
Using a KB, we may assign a column pair with a known relationship (for example, a property) in the KB \cite{tanon_20_yago, 21_hogan_knoweledge_graph_survery}, or again using unsupervised techniques we may determine a set of column pairs have the same (but unknown) relationship.  Note that a relationship is any binary relation (in particular, it does not need to be a function).


\begin{definition}[Relationship Semantics]
\label{def:rs}
The relationship semantics of a pair of columns $c_1$ and $c_2$ (denoted $RS(c_1, c_2)$) in a table $\dltable$ is either empty or a relation $p$ with a confidence score between 0 and 1.  
\end{definition}

\rjm{
\begin{example}
\label{ex:relationshipsemantics}
Examples of relationships in Table (b) of \cref{fig:running_examples} include \texttt{DirectedBy}, between 
\texttt{Film Title} and \texttt{Film Director}
and \texttt{HasPhone}, a relationship between \texttt{Park Name} and \texttt{Park Phone}.  Each will have a confidence score assigned by the discovery technique.
There may be no relationship discovered between \texttt{Film Title} and \texttt{Park Name} or \texttt{Park Phone}.  
\end{example}
}
\introparagraph{Semantic Graphs}
A relationship can be represented as 
a triple 
\ak{( Subject -- Predicate -- Object)} 
% (Subject \begin{tikzpicture}
%   \draw (-2,0) -- node[above] {Predicate} ++(2,0);
% \end{tikzpicture} Object)
or 
an edge in a graph whose  nodes  are
the %attributes
columns of a table and an edge connects a pair of %attributes.
columns.
% (or a predicate or a property, depending on your choosen
% vocabulary).  
%rjm resolved above
%\wolf{3/23: ``Relationships are most widely interpreted as a triple (SOURCE, RELATIONSHIP, TARGET). [CITE KG surveys and RDF literature].
%In this interpretation `a relationship' is the commonly a binary relationship between two entities. 
%The binary relationships we are focusing on in this paper is the relationships between an ordered pair of columns in the same table.
%And we use the natural representation as a labeled directed edge between such columns interpreted as nodes...''}
%\aamod{03/27: In SANTOS, binary relationships are bidirectional. For example, \cref{fig:running_examples}(f) can not only be unioned with a table about famous person born and their birthplace but also with a table that is about cities and the properties of cities like geo, famous person , etc. To model this difference, we did not call it S-P-O because in that case we cannot use object as subject. Therefore, we introduced intent column and in \cref{fig:running_examples}(f), user can mark both famous person and birthplace as intent column as per the analysis. For example, if a user wants to collect the information about famous person, he can mark famous person as intent, and occupation, birthplace will be the properties of famous person. Note that we also allow property of property. Therefore, Geo is property of birthplace and the semantic tree will be a tree having 2 levels below root.
%Conversely, if user wants to use birthplace as the intent column, famous person and Geo are its properties and occupation is the property of property (famous person).}
%rjm moved this to example above
%rjm Examples of relationships include %rjm \texttt{directed-by} i.e.,
%rjm \texttt{Film Title} \begin{tikzpicture}
%rjm   \draw (-2,0) -- node[above] {\texttt{directed-by}} ++(2,0);
%rjm \end{tikzpicture} \texttt{Film Director}
% \texttt{directed\_by}, i.e. \texttt{Film Title}--\texttt{directed\_by}--\texttt{Film Director}.
%\aamod{I prefer to write it \texttt{Film Title}--\texttt{directed\_by}--\texttt{Film Director} as in undirected case, arrow does not look nice.}
%\aamod{I searched for the replacement of $\xrightarrow{\texttt{directed-by}}$ with same text/style but undirected arrow. However, seems like its not available \url{https://latex-tutorial.com/arrow-latex/}. Therefore, I used tikzpicture. Would appreciate if anyone knows.}
%$\xrightarrow{\texttt{directed-by}}$ \texttt{Film Director} 
%\renee{please make the line undirected!}
%a relationship between {\tt Film Title} and {\tt Film Director} 
%rjm in Table (b) of \cref{fig:running_examples}, and \texttt{has-phone}, a relationship between \texttt{Park Name} and \texttt{Park Phone}. 

%rjm resolved above
%\wolf{3/23: 
%using a variant of following notation would make it easier to follow (the user does not need to keep all the triples in their mind but would `see' the relationship)
%\texttt{Film\_Title} $\xrightarrow{\texttt{directed-by}}$ \texttt{Film\_Director}.
%Maybe to propose the following short form, it is still intuitive:
%\texttt{Film\_Title} $\rightarrow$ (\texttt{directed-by}) \texttt{Film\_Director}
%}
%\aamod{03/30: updated}
%Note that we have named these
%columns to make the relationship clear, but in a table with \texttt{Park}, \texttt{Film} and %\texttt{Phone} columns,
%it is unclear if \texttt{Phone} has a semantic relationship with
%\texttt{Film} or with \texttt{Park}.  
%\wolf{3/23: maybe use some notation 
%\texttt{Film} $\rightarrow$ \texttt{Phone}
%or
%\texttt{Park} $\rightarrow$ \texttt{Phone}.
%BTW, texttt is more modern version of tt:
%\url{https://texfaq.org/FAQ-2letterfontcmd}}
%\aamod{03/29: updated and will update on other places while making the passes.}
%rjm resolved - they are relations
%\wolf{3/23: Somewhere here you likely want to discuss the issue of whether you allow relationships that are not functional.
%It seems for you there is not semantic relationship between Park and Phone in above example. Because the relationship is NOT FUNCTIONAL.
%But there is still a relationship, it is just not what you want. Somewhere early here discuss this valid restriction.}
For now, we assume we have an oracle (which may be a knowledge base or
any relationship discovery tool) that provides a set of binary relationships between
columns.   These relationships
form the edges of a 
%\rjm{a} 
{\em semantic graph} for a table.
%rjm resolved:  yes and added to text
%\wolf{3/23: is the semantic graph always table-specific? Thus you don't have one semantic graph in the data lake, but one per table?} 
%\aamod{03/27: Yes, each data lake table has its own semantic graph. We have mentioned that in Definition below.}
%rjm:  this is just definitions for the moment, I don't think we need what is below
%In \cref{subsection:relation_semantics}, we will discuss how we find these
%relationships. Note that, we create semantic graph for each table.




\begin{definition}[Semantic Graph]
\label{def:semanticgraph}
Given a set of columns $\mathcal C = \{c_1, c_2 \dots c_m\}$ \rjm{each with non-empty column semantics} of a table $\dltable$, 
the semantic graph of $\dltable$ 
%rjm resolved to R
%\wolf{3/23: why D for table instead of T? D is usually used for data, thus more the instance than the schema.}
%\aamod{03/29: We used $T$, $T_{top}$, $ts(t)$ etc for representing the column semantics (types). Therefore, we used $D$ for the data lake tables. Would you suggest to use something different for the types?}
is a graph $G_\dltable = (V,E)$ where 
each vertex $v_i$ represents column $c_i$  
%with column semantics $CS(c_i)$
and each undirected edge $e_{ij}$ 
%rjm resolved below
% \wolf{3/23: is this an edge or an arc = directed edge? 
%Is a semantic graph still valide even if it has singleton vertices, e.g. the relationship of a column is not clear?
%Can there be multiple SGs for the same table? E.g. a complete graph between all pairs, and another one that only reflect functional relationships?}
represents a
%the 
%\rjm{a} 
relationship between columns $c_i$ and $c_j$ \rjm{with non-empty relationship semantics $RS(c_i, c_j)$.}
%Note that some column pairs may not have relationship (and therefore no edge).
\rjm{Column pairs with an empty relationship semantics have no edge in the graph.}
\end{definition}

\rjm{
\begin{example}
\label{ex:semanticgraph}
A possible
%rjm Also, the 
semantic graph for the data lake Table (b) about parks and films is shown in \cref{fig:running_examples} (e). As illustrated by this example, the semantic graphs of data lake tables may not be connected graphs depending on the relationship discovery. 
\end{example}
}

%\introparagraph{Query and Data Lake Tables}
\introparagraph{Unionability Search over Semantic Graphs}
In SANTOS, a user (a data scientist) provides a Query Table (denoted by Q) and specifies its \textit{intent column} (denoted by $I$), meaning a column of interest within the query table.
%that forms relationships of interest with other columns. 
SANTOS analyzes the query table to create a semantic graph which we restrict to being a tree rooted at the intent column.   We find relationship from the intent column to other columns in the query table, then transitively search for relationships from these columns.
We call the semantic graph of the query table, the {\em Query Semantic Tree}.  This process allows a   user to direct the search to have the %subject or
%aamod: let's not add the word subject as we are mentioning intent everywhere.
intent that they are interested in.
We search for data lake tables that contain a column with a similar (matching) semantics to the intent column and with similar relationships.
\rjm{More specifically, we will look for a tree within the semantic graph of each data lake table that matches a subtree of the query tree rooted at the intent column.
%the intent column of the query table and a tree of matching relationships rooted at the intent column. 
%rjm resolved - no my writing was ambiguous, I fixed this
%\grace{4/4: Two different trees?} 
We do not require that the full query semantic tree be covered by a data lake table.  We assume a scoring function that considers the strength of column and relationship matching as well as how much of the query tree is matched.}
%rjm:  too procedural 
%Using our relationship oracle, we then form a semantic tree for the query table rooted at the intent column \footnote{\label{footnote:multiple_intents} Our approach can easily be expanded to the query tables having multiple intent columns. However in this work, we restrict query table to have a single intent column.}. All non-root nodes refer to \textit{property columns} or their properties.
%rjm too procedural
%At ingestion into the data lake, we form a semantic graph for each data lake table. \wolf{3/23: graph or forest? ingestion means offline before the query arrives? ingestion of the data lake or into?}
%\aamod{03/29: This can be any arbitrary graph for relation tables (like \cref{fig:running_examples}(b) and tree for the entity tables(like \cref{fig:running_examples}(a) and (c).}
% We do not have an intent column for data lake tables as they can have many potential intent columns. Their semantic graphs may not be trees but we do assume they are acyclic and has a single relationship between any pair of columns. This corresponds to an assumption like the \textit{universal relation model} but only within a single table.
%\rjm{
%To do this,  
% (as motivated in Example~\cref{}).  When searching for {\bf parks} we do not want to return only tables with cities and their locations (two descriptive attributes) with no information about parks.  
%}

\begin{example}
% Returning to our example in Table (a) of
Again consider Table (a) about parks in
\cref{fig:running_examples} as a query table. Suppose a user has identified
\texttt{Park Name} as the intent column.  
%rjm Let there be three relationships, 
%rjm first two stating \texttt{Supervisor} and \texttt{City} are the properties of \texttt{Park Name}, and the third stating \texttt{Geo} is a property of \texttt{City}. 
We find two relationships involving the intent column
(1) Park Name -- LedBy--Supervisor and 
(2) Park Name -- LocatedIn -- City
 as shown in \cref{fig:running_examples}(d).
% (1) Park Name \begin{tikzpicture}
%   \draw (-2,0) -- node[above] {LedBy} ++(2,0);
% \end{tikzpicture} Supervisor
%  and (2)
% Park Name \begin{tikzpicture}
%   \draw (-2,0) -- node[above] {LocatedIn} ++(2,0);
% \end{tikzpicture} City. 
We find a third relationship involving City:
i.e., City--GeoCoordinates--Geo.
% City \begin{tikzpicture}
%   \draw (-2,0) -- node[above] {GeoLocatedIn} ++(2,0);
% \end{tikzpicture} Geo.
%rjm resolved relationships are relations
%\wolf{3/23: So here in contra(st to def before you imply only functional relationships? 
%Also how do you define precisely the relationship with Geo? If relationships are only between intent and property, then this one does not fit that assumption} \aamod{03/30: updated in the paragraph before that non-root nodes can be either property of the property of property.}
The semantic graph for the Query Table (a) is depicted in \cref{fig:running_examples}~(d). 
%rjm resolved changed to graph
%\wolf{3/23: which is the best name to use consistently: semantic graph vs semantic tree vs semantic forest vs semantic DAG vs semantic digraph?}
%\aamod{03/29: For the data lake tables, we decided to use semantic graph. For query tables, it is a semantic tree. Also, when we match data lake table with a query table, we convert it into a tree according to the query table's columns. (discussed below this example).}
%rjm moved this to SG example
%A possible
%semantic graph for the data lake Table (b) about parks and films is shown in \cref{fig:running_examples} (e). As illustrated by this example, the semantic graphs of data lake tables may not be connected graphs depending on the relationship discovery. 
%rjm this is confusing dl tables have no intent columns!
%rjm This is a realistic scenario since, as discussed in \cref{section:intro}, a table may not have a single \textit{intent column}.
By having an intent column, 
%rjm we can devise scoring functions that prioritize matching on this column.
we can focus our search on data lake tables that can be mapped into a subtree of the query semantic tree rooted at the intent column.
For example, we can determine if the semantic graph of Table (b), which is depicted in \cref{fig:running_examples}(e) contains a subtree that maps to the query semantic tree.  If the column semantics for 
(a) \texttt{Park Name} and \texttt{City} match those of 
(b) \texttt{Park Name} and \texttt{Park City} and the relationship semantics of \texttt{locatedIn} matches \texttt{locatedIn} well enough,
then we can say that (b) is a candidate unionable table that unions on $\Pi_{Park Name, Park City}$.
\ak{
Notice however the semantic graph of \cref{fig:running_examples}(f)
about famous person and their birthplace in \cref{fig:running_examples}(c).
Although there is a possible matching relationship involving \texttt{Birthplace} and \texttt{Geo} (with City--GeoCoordinates--Geo), this table is not a candidate unionable table as there is no possible intent column and no
semantic tree matching relationships rooted at the intent column.}
%\renee{add relationship names to figures (d) and (e)}
\end{example}

%\renee{you can add a negative example to the example above if you want.}

%\renee{Please change if this is not true.  Does the search permit a a dl table to be mapped to disconnected parts of the query semantic tree?}

%rjm moved to example - if you want a negative example, add it fully to example above
%rjm Given a query table and its semantic graph (which we restrict to being a tree), we will match portions of the semantic graphs of data lake tables into the semantic tree of the query. In other words, we extract the portion of data lake table's semantic graph that matches with the query table starting with the root node.
%rjm and convert it into a tree rooted at the node that matches with query table's intent column node. 
%rjm For instance, from the semantic graph (\cref{fig:running_examples}(e)) of table about parks and films in \cref{fig:running_examples}(b),
%rjm will be converted into a semantic tree rooted at \texttt{Park Name} with only one branch having \texttt{Park City} as leaf when we match it with the semantic tree (\cref{fig:running_examples}(d)) of table about park in (\cref{fig:running_examples}(a))
%rjm we can find 
%high scoring 
%\aamod{ I thought the word "high scoring" is typo and removed it. Please correct me if I am wrong.}
%rjm matching into portions of the query semantic tree (\cref{fig:running_examples}(d)).
%\wolf{3/23: Great! Can you formalize this with the help of tree homomorphisms?}
%rjm Therefore, a data lake table about parks and films can still match a query table requesting information on parks. 
%rjm \ak{Note that the data lake table's column that matches with $I$ in the query table must participate in forming a relationship that matches with a relationship formed by $I$ in the query table's semantic tree. 
%rjm In other words, it must match to the connected part of the query semantic tree.
%rjm For instance, when \cref{fig:running_examples}(c) about people and their birth places is a query table with \texttt{Person} as an intent column, \cref{fig:running_examples}(a) about \texttt{Parks} will not be considered as a unionable table although there is a column \texttt{Supervisor} matching with intent column and a matching relationship 
%rjm Birthplace \begin{tikzpicture}
%rjm   \draw (-2,0) -- node[above] {GeoLocatedIn} ++(2,0);
%rjm \end{tikzpicture} Geo
%rjm with
%rjm City \begin{tikzpicture}
%rjm   \draw (-2,0) -- node[above] {GeoLocatedIn} ++(2,0);
%rjm \end{tikzpicture} Geo. This is because the intent column is not participating in forming any relationship. Based on these concepts, we quantify the match between query table and each data lake table using a scoring function $S$ (\cref{section:semantic_union_search}).
%rjm }



%rjm resolved - not functional
%\wolf{3/23: why intent/property instead of key/value?
%IMPORTANT: Are you allow non-key intent columns, e.g. to specify a query table that has ``relational'' instead of ``functional'' relationships between columns? (e.g. a table that lists film title, and actors each in a different row)?}

%rjm resolve - no clarified by saying a "portion of query semantic tree"
%\wolf{3/23: Wait, so you area assuming a relationship between Filme and Phone in the example further above?}

%rjm:  no relationship to URA, this would be distracting, right
%\wolf{3/23: Interesting, but I can't follow. Please elaborate here in detail about the connection to the (controversial) universal relation assumption.
%In particular, please cite something}

%rjm clarified that the restriction on query table is to focus the search.  
%\wolf{3/23: Important to discuss the difference between Fig 1a and 1c: tree vs forest.
%do you require table with forests in the data lake, and with trees as query table?}

\introparagraph{SANTOS Top-k Union Search}
%\rjm{TBD define search problem}
\ak{
Now we will formally define SANTOS Union Search.
\begin{definition}[SANTOS Top-k Union Search]
\label{def:new_santos_unionability}
Given a set of Data lake Tables $\mathcal{\dltable}$, a query table $Q$ with a specified intent column $I$, 
a Query Semantic Tree rooted at $I$, denoted $SG(Q)$.
We assume a 
%relationship
semantic graph matching or 
scoring function $S$ that for each $\dltable \in \mathcal{\dltable}$ returns the highest scoring subtree of $SG(\dltable)$ that matches a subtree of $SG(Q)$ rooted at $I$.
%what portion of the query semantic tree rooted at $I$ matches with a sub tree extracted from the semantic graph of each $\dltable \in \mathcal{\dltable}$,
%rooted at the column that matches $I$, 
The SANTOS union search problem is to find the top-k data lake tables having the highest score modeled by $S$.
\end{definition}
}
\grace{4/4:
(2) Currently, "relationship scoring function $S$ that quantifies what portion of the query semantic tree rooted at $I$ matches with a sub tree extracted from the semantic graph of each $\dltable \in \mathcal{\dltable}$" makes me think that we're matching a portion of the query semantic tree to a subtree of the DLT (matching portion of QT into portion of DLT). I thought we wanted to see what portion of the DLT subtree we can match with the query semantic tree (see what part of DLT matches QT).
}
\renee{4/4:  No, I don't think the DLT needs to match the full QT, right? I've tried to reword to make this clear, let me know if you like the new wording.} 
\grace{4/4: It looks better, thank you!}

%In the next sections, we define the criteria for matching a data lake table to the query table.
% \subsection{Representing Tables with Semantic Trees}
% We will create an abstraction over query tables, 
% called a {\em semantic tree}, which represents the relationships of interest between attributes within a table.  

% \rjm{Not sure I understand this comment, a digraph is a pair of letters pronounced as one, like "ph" in "Phokion". Do you mean directed graph?  We are using undirected graphs, not sure we need a special name for it.  I will make this clear}
% \wolf{10/28: better to introduce the more general concept here first

% \subsection{Interpreting Tables as Semantic Digraphs}
% We will create an abstraction over tables, 
% called a {\em semantic digraphs}, which represents the relationships between columns of a table.  
% }

% \subsubsection{Semantic Tree}\label{section:semantic_trees}
% An important goal of SANTOS is to accurately represent the relationship between attributes 
% 	% \wolf{10/28: ``attribute'' is here used as synonym for column.
% 	% Later, ``attributes'' is also used to refer to only a subset of columns, namely those that are ``attributes of interest'' of a intent column.
% 	% Thus ``attributes'' is here a homograph with two different meanings: 1. all columns, 2. properties of entities.
% 	% Using columns throughout would avoid that double-use.}
% within a table and use this information to find the most relevant unionable tables.  To do this, we will use the notion of a \emph{semantic tree} of a table.
% Tables contain not just attributes but they represent semantic relationships between these attributes.  
% The table in \cref{fig:entity_films}, for example, represents a relationship between film name (\texttt{Name}) and its \texttt{Released Year}.  
% It also represents a relationship between a film and its \texttt{Director}, etc. 
% A \emph{semantic tree} is a structured way to represent these relationships. 
%rjm again I will address you comment.
%\wolf{10/28: I really think that the concept of a relationship is best to be explained early.
%Especially in terms of triples that people from KB and knowledge graphs are more familiar with. Something like:
%``A relationship between column represents a template of intent-Predicate-Object (S-P-O) triples between cells in rows of a table.
%As example consider the set of values (Summertime, Alamos Square) in the first row of Fig 1. 
% Their relative relationship in terms of S-P-O triples can be interpreted as 
% S: Summertime, P: Location, O: Alamos Square. 
% Actually for any row, the respective pairs of values form triple
% S: x in Name column, P: Location, y in Location.
% We abstract the `template' of such relationship as a directed pair
% (Name, Location) at the level of the table schema, implying the triple relationships across cell and column type.
%''}
% To define a semantic tree formally, first we start by defining a general \emph{semantic graph}.
% The more general notion of a semantic graph is to represent information in data lake tables.
% \wolf{10/28: it appears conceptually easier to first define the idea of a semantic graph (semantic digraph) as the general concept representing the table schema in terms of S-P-O triples = directed edges = arrows *for any table*. Notice that the ``semantic graph'' is actually a directed graph}
% Next, we make it specific and define the \emph{semantic tree} that captures relationships of interest to a user within a query table.  
%rjm we do not require FDs
%rjm I'm not familiar with HASSE diagrams.  I fear introducing an unfamiliar concept and saying "we aren't that" would be a distraction.
%\wolf{10/26: in what ways are those semantic graphs or trees different from existing concepts? 
%In particular 1) the HASSE diagram 
%\url{https://en.wikipedia.org/wiki/Hasse_diagram}
%of all FDs in a table? Also, 2) how does past work (e.g. the knowledge graph survey by Hogan et al.\ section 6.4.1) think about interpreting tables in terms of triples? 
%I am a bit worried about a review comment asking: why introduce a new concept and not leverage existing notions? Maybe there is a difference, then it is good to point out the conceptual differences and the added benefit of this new and enhanced perspective.}
% For now, we assume we have an oracle (which may be a knowledge base or other source) which provides a set of binary relationships (or properties) between attributes of a given type.  These relationships will form the edges of the {\em semantic graph}.  In \cref{subsection:relation_semantics}, we will discuss how we these relationships.


% \begin{definition}[Semantic Graph]
% Given a set of attributes $\mathcal A = \{A_1, A_2 \dots A_n\}$ of a table T, 
% \wolf{10/28: better use $k$, because $n$ is later also used as number of tables (which is also a more natural use for ``n'')}
% the semantic graph of T is a graph $G_T = (V,E)$ where, each attribute is a vertex in the graph ($\forall (A_i \in \mathcal A) \exists \ (v_i \in V)$) and $\forall (A_i, A_j) \exists \ (e_{ij} \in E)$ where, $(A_i, A_j)$ represents a pair of attributes having a relationship.
% \end{definition}


% \wolf{10/28: suggestion:
% \begin{definition}[Semantic Graph]
% Given a set of attributes $\mathcal A = \{A_1, A_2 \dots A_k\}$ of a table $T$, 
% the semantic graph of $T$ is a graph $G_T = (V,E)$ where 
% each vertex $v_i$ represents an attribute $A_i$ in the table
% and each edge $e_{ij}$ represents a relationship between attributes $A_i$ and $A_j$.
% \end{definition}
% }

%rjm I don't know what a Hasse diagram is and doubt a reader will
%\wolf{10/28: ``In practice, we don't show all semantic relationships but use the more compact form of a Hasse diagram, 
%implying addition transitive relationships from the transitive closure of relationships [CITE]. 
%As example, we don't show (Title, Borough Code) as this is implied from transitivity
%from both (Title, Borough) and (Borough, Borough Code).''}


%\begin{definition}[Semantic Tree]
%A semantic graph $G_T = (V,E)$ of Table $T$ having a set of attributes  $\mathcal A$ = $\{A_1, A_2 \dots A_n\}$ and their corresponding vertices $V = \{v_1, v_2 \dots v_n\}$ is said to be a semantic tree if there exists a root node $v_i \in V$ such that $\forall (v_j \in V \setminus v_i) \exists (e_{ij} \in E$) from $v_i$ to $v_j$ where, $i$ can be any value between  1 to n and $j = \{1, 2, 3, \dots n\} \setminus i$.
%\end{definition}
%rjm addressed
%\wolf{10/26: give the earlier semantic graph definition, it is easy to just in words state that
%``a semantic tree is a semantic graph that forms a rooted forest [or similar]'' because the limitations of graphs to trees is standard}

% We discuss in the next section how we form semantic graph for each data lake table.  
% % Over a query table, we will form a restricted
% %form of semantic graph called a {\em semantic tree}.  
% %b=More specifically, a semantic tree represents the relationships of interest to a user issuing the union query.  
% \wolf{3/23: The following sentence gets repeated in 3.2. It is better introduced there in 3.2, focus here just one those semantic digraphs per table
% without yet reference to query table vs data lake table. That comes in 3.2}
% For the query table, the  SANTOS query model permits a user to select an {\em intent
%   column}, meaning a column of interest within the query table that forms relationships with other columns. 
%   Hence,
% over a query table, we create a semantic graph with a tree
% where the root is an intent column chosen by the user.  All non-root
% nodes refer to {\em property columns} or their properties.
% \wolf{3/23: why intent/property instead of key/value?
% IMPORTANT: Are you allow non-key intent columns, e.g. to specify a query table that has ``relational'' instead of ``functional'' relationships between columns? (e.g. a table that lists film title, and actors each in a different row)?}
% We assume that all semantic graphs are acyclic, with
% a single relationship between any pair of columns (including
% transitive relationships). 
% \wolf{3/23: Wait, so you area assuming a relationship between Filme and Phone in the example further above?}
% %rjm remove this if it doesn't make sense to you
% This corresponds to an assumption like the
% {\em universal relation model} but only within a single table. \grace{Do we need this final sentence?}
% \wolf{3/23: Interesting, but I can't follow. Please elaborate here in detail about the connection to the (controversial) universal relation assumption.
% In particular, please cite something}

% %\begin{definition}intent Column]
% %Given a semantic tree $G_T = (V,E)$ for Table $T$ having a set of attributes $\mathcal A$ = $\{A_1, A_2 \dots A_n\}$ and their corresponding vertices $V = \{v_1, v_2 \dots v_n\}$, $A_i$ corresponded by \ $v_i$ is said to be a intent column if $v_i$ is the root node of $G_T$.
% %\end{definition}

% %rjm addressed
% %\wolf{10/26: problem with that definition: there is no semantic interpretation of the edges as of now. Thus we do not know what the semantic meaning of a root node is in that formalism. By the definition, I could always randomly draw a tree across the attributes and it would still fulfill the current definitions.
% %rjm. I don't know what a Hogan graph is, is this commonly used?
% %Suggestion: do very clearly define what you like to capture with a intent column, ideally in terms of related concepts defined in past work, above all past work on table interpretation. The Hogan knowledge graph survey may be the best starting point to look.
% %rjm:  we do not require a relationship to be an FD or 1-many
% %Once you have define what you like a intent column to be (what it is, not how you characterize it based on syntax, like FDs), 
% %then you can argue that your syntactic definition maps that semantic goal.
% %}
% %A semantic tree may also have additional levels, in which the children (properties) of the root node (intent column) have additional children (properties). 
% \begin{example}
% % Returning to our example in Table (a) of
% Again consider Table (a) about parks in
% \cref{fig:running_examples} as a query table. Suppose a user has identified
% \texttt{Park Name} as the intent column.  Let there be
% three relationships, first two stating \texttt{Founding Date} and \texttt{City} are the properties of \texttt{Park Name}, and the third stating \texttt{Geo} is a property of \texttt{City}. 
% \wolf{3/23: So here in contrast to def before you imply only functional relationships? 
% Also how do you define precisely the relationship with Geo? If relationships are only between intent and property, then this one does not fit that assumption}
% Then we have the semantic tree depicted in \cref{fig:running_examples}~(d). 
% \wolf{3/23: which is the best name to use consistently: semantic graph vs semantic tree vs semantic forest vs semantic DAG vs semantic digraph?}
% Also, the semantic graph for Table (c) about parks and films as a data lake table is shown in \cref{fig:running_examples} (e).
% \end{example}

% \begin{example}
% Consider Table (c) in \cref{fig:running_examples}, and the semantic
% tree  in \cref{fig:entity_table_intent_graph}~(b). An attribute
% \texttt{Name}, representing the name of the films has been selected by the
% user  to be the intent column.
% The property nodes represent the columns \texttt{Location},
% \texttt{Released Year}, \texttt{Director}, \texttt{Actor1} and
% \texttt{Actor2} which have a relationship with \texttt{Name}.
% \end{example}


% \renee{I suggest adding this figure to Fig 4 and making nodes of figure 4 smaller.  So you have a 4A (a line with two levels) and 4b (current fig 4)}
% \renee{Why are there arrows in Fig 4?  Aren't this undirected edges?}
% \aamod{Done! My initial intuition was considering query table as a directed tree so that we have a root node naturally. However, I realized that's not necessary because we already said that the user is marking the root node for us.} 


% \begin{figure}[h]
%   \centering
%   \includegraphics[scale = 0.4]{figures/Fig_semantic_tree_film_and_museum_table}
%   \caption{
%   Examples of Semantic Tree for (a) Table of \cref{fig:crime_and_musuem_tables}~(a) about museums and (b) Table of \cref{fig:entity_films}~(b) about films with \texttt{Title} as the intent column in both cases.}
%   \label{fig:entity_table_intent_graph}
% \end{figure}


% \begin{figure}[h]
%   \centering
%   \begin{subfigure}[t]{.31\linewidth}
%   	\centering
%   	\includegraphics[scale=0.45]{figures/Fig_SemanticTreeExample_a}
%   	\caption{Semantic digraph}	
% 	\label{Fig_SemanticTreeExample_a}
%   \end{subfigure}
%   \begin{subfigure}[t]{.68\linewidth}
%   	\centering
%   	\includegraphics[scale=0.45]{figures/Fig_SemanticTreeExample_b}
%   	\caption{Example instantiation}	
%   \label{Fig_SemanticTreeExample_b}
%   \end{subfigure}  
%   % \includegraphics[scale=0.45]{figures/Fig_SemanticTreeExample}
%   \caption{
% \wolf{10/28: suggestions:
% 1. to use PDFs instead of PNG (please double-check with Nikos how to do this on a Windows machine), 
% 2. to use scale instead of linewidth (and use the same font sizes across all figures to make sure all figures across the paper have the same appearance in fonts size *in the paper*),
% 3. all figures use consistent appearance including same size for nodes (in above earlier PNG fig some nodes were ellipses and of different size) and nicely aligned and nicely equi-distant, and nice consistent line widths
% 4. use subfigures to be able to refer to individual subfigures from the text (exception are big overview pictures with lots of annotations)
% % 
% %rjm addressed
% %5. text including: 
% % ``Examples of Semantic digraph (a) and instantiations as instance triples (b) for the table in \cref{fig:crime_and_musuem_tables}~(a) about museums. 
% % We use bold fonts for attribute names and non-bold fonts for cell values. The intent column is shown as dark circled node. Blue is used for representing the names of relationships (or the property in S-P-O triples).''
% }
%   }
%   \label{Fig_SemanticTreeExample}
% \end{figure}

% \rjm{please remove comments once addressed or even noted!  we agreed
%   to move data example to later section - Figure 5.  This section is
%   not able the data}



% \subsection{Representing Tables with Semantic Trees}
% \roee{consider including somewhere: Given a query table and its respective semantic tree, an appropriate level (depth) of representing data lake table is selected.}

% We now use the notation of semantic trees to represent the query table and data lake table. As the data lake tables representation is not dependent of the one of the query table we begin by describing the data lake tables.

% \subsection{Query and Data Lake Tables}
% In SANTOS,  a user (a data scientist) provides a Query Table (denoted by $Q$) and specifies its \emph{intent column}. 
% %\renee{Since the semantic graph may not be a tree, don't we need the user to tell us which subset of the graph to use as the query tree?}
% %\aamod{In Query Table, once the intent column is marked, we assume that all other columns are either the properties of the intent column or the properties of properties. We have experiments on similar QTs.}
% Using our relationship oracle we can form a semantic tree for the query table.  
% \wolf{3/23: Important to discuss the difference between Fig 1a and 1c: tree vs forest.
% do you require table with forests in the data lake, and with trees as query table?}
% % With guidance from the user, 
% We then select a subset of this graph that forms a tree rooted at the intent column.
% %rjm We consider other columns to be properties and create a corresponding semantic tree. 
% %jm Additionally, we also support a table having \textit{multi-level semantic tree} as a query table. 
% %\wolf{10/27: how does a multi-level semantic tree differ from one with multiple intents? Multi-level means there is some transitive FD, thus a non-leaf node could be interpreted as alternative intent (which in turn is an object of the root node)?}
% %While creating the semantic tree for the query table, first we check if each property column is an immediate property of the intent column. 
% %If the column is not an immediate property, we also check if it is the property of other properties. 
% %We use a knowledge base and functional dependencies to perform such checks, which we will discuss in details in \cref{section:unionability_components} and \cref{section:synthetic_knowledge_base}.
% %rjm:  I suggest we address this is one place later in the paper
% %\wolf{10/27: What is the relation between these semantic %trees and FDs? Is it:
% %semantic tree = FDs over an infinitely large database?
% %But some FDs are just spurious?
% %Thus edges in semantic tree are schema FDs?
% %
% %Or is it rather that you allow S-P-[O1, O2], thus multiple %value instances for each attribute. For example:
% %(S: Film: Batman, P: Actor, O: Alice), (S: Film: Batman, P: Actor, O: Bob), ...?
% %}
% %\renee{Please correct this if this is not what you intended.}
% %aamod: This looks good.
% At ingestion into the data lake, we form a semantic graph for each
% data lake table.  
% We do not have an intent column for data lake
% tables as they can have many potential intent columns. %(intuitively, a data lake may have many columns which a user could select as intent columns), 
% Their semantic graphs may not be trees but we do assume they
% are acyclic.  

% \wolf{3/23: What is the exact assumption of graph. Does it need to be forest, or can it be a DAG?
% Suggestion to specify this right under the semantic graph definition.
% Then in 3.2 here specify that in this model, ``we assume the semantic forests of query tables to be trees, thus they have one single root.''
% Is this restriction necessary for the method to work, or could it be extended easily?
% Say I want to extend a table (film, actor) with more instances of actors playing in films. Is this application excluded or covered?}



% Notice that, depending on the relationship oracle, the semantic graphs of data lake tables may not be connected graphs
% as shown in \cref{fig:running_examples}(e). 
% \wolf{3/23: But those are still DAGs. Best to see by adding a direction to the edges = arcs. }
% \wolf{3/23: I see now why don't want to call those key / value relationships. But is intent / property standard? Why not then use Subject Object, with the name of the relationship being the Predicate? That's a standard concept from RDF: S-P-O triples. Also easy to interpret with labeled directed edges}
% This is a realistic scenario since, as discussed in \cref{section:intro}, a table may not have a single intent column.  
% Given a query table and its semantic tree, we will match portions of
% the semantic graphs of data lake tables into the semantic tree of the query.  
% \wolf{3/23: Great! Can you formalize this with the help of tree homomorphisms?}
% So a data lake table about parks and films can still match a query table requesting information on parks.  In the next sections, we define the criteria for matching a data-lake table to the query table and define SANTOS unionability.

% % \begin{figure}[h]
% %   \centering
% %   \includegraphics[scale = 0.4]{figures/Fig_semantic_graph_film_park_table}
% %   \caption{Semantic graph for a data lake table about parks and films in \cref{fig:relation_parks_films}.
% % %rjm we decided to keep everything undirected.  
% % %  \wolf{10/27: do include arrows. Also, please use PDF vector graphics and not PNG for figures. 
% % %  Also, best to draw them in a space-saving way.
% % %  Shouldn't park name be the root node on top?
% % %  Do you have it as a PowerPoint file PPTX? 
% % %  I could make a pass over the figures directly. \aamod{10/28: This is a data lake graph where any column can be a "potential intent column. Therefore, we do not show the arrow."}}
% % %rjm In data lake table, all columns are "potential intent columns"
% % %\wolf{10/27: Is film studio also a possible intent column. Say one tries to find the countries of studios?}
% %   }
% %   \label{fig:relation_table_intent_graph}
% % \end{figure}

% %rjm I have taken aamod's suggestion to move this later

% % \subsection{\unionability}\label{section:unionablity_def}

% % In this section, we 
% % %explain the concept behind our new unionability definition which we call
% % define \unionability \, a relationship-aware definition of unionability.

% % \subsubsection{Unionability Scenarios}

% % \begin{figure}[h]
% %     \centering
% %   \includegraphics[width=\linewidth]{figures/unionability_scenario.png}
% % %   \includegraphics[scale = 0.6]{figures/unionability_scenario.png}
% %   \caption{Possible Data lake Table scenarios for unioning with a Query Table. The tables rows are not shown.
% % %	\wolf{10/27: suggestions: 1) put the query table on top. 2) Keep things nicely aligned both vertically and horizontally.
% % %	3) Maybe you want to also show which tables are false positives or false negatives for competitor methods. 
% % %	\aamod{10/28: 1) Resolved! 2) I would appreciate more suggestion on this figure. Since the number of tables is three in the lower-right part, I tried my best to optimize the aesthetics as well as space. I would prefer to have column names in a single row rather than overflowing to the second row. 3) We planned to write the paper using an approach which we called positive approach. Therefore, we are trying to keep the related works away from the early sections rather than comparing with them in each step, at least not until section 4. Shall we think differently?}
% % 	}
% %   }
% % \label{fig:unionability_scenario}
% % \end{figure}
% % Let us consider the example table scenarios in \cref{fig:unionability_scenario} that can arise when we search for the unionable tables in a data lake. 
% % Note that we adapted the tables in \cref{fig:crime_and_musuem_tables} from a real table in UK government open data. 
% % \wolf{10/27: perhaps CITE}
% % For convenience, we only show the table schemata (possible values are given in \cref{fig:crime_and_musuem_tables}).
% % Suppose the query table is 
% % about \texttt{Museum} (\textit{intent column}) 
% % and the user is looking for \texttt{Borough Name} and \texttt{Ward Name} (\textit{property columns}) of the museums. Tables (a)-(g) represent data lake tables.
% % Since Table (a) has all the information in the semantic tree of   the query table, we consider this table to be 
% % unionable with the query table using this semantic tree.
% % One can simply project away the extra information (i.e., \texttt{Street Address}) and union the rest.
% % Similarly, Table (b) also provides all the information about museums that the user is interested in.
% % Therefore, we consider Table (b) also to be 
% % unionable with this query table and semantic tree.
% % Next, we also have Table (c) that encodes the museums and their \texttt{Ward Name} but not \texttt{Borough Name}.
% % Similar is the case with Table (d) that presents the \texttt{Borough Name} information but not \texttt{Ward Name}.
% % Since these tables are able to provide at least some information in the query, we also consider them to be unionable.
% % Next, Table (e) provides the information like \texttt{Borough Name} and \texttt{Ward Name}.
% % However, we do not know whether this information is about museums (our query intent column).
% % Hence, we consider that the tables like table (e) are not unionable with this semantic tree.
% % \wolf{10/27: So here you may want to emphasize that union scores that only aggregate columns scores can't distinguish these scenarios.
% % That is the sweet spot of what the method can do. The next example (f) covers a different issue.
% % One issue you like bring up: what about a data lake table (museum, borough name, street address)?}
% % \aamod{10/28: (museum, borough name, street address) is covered by example tables (a) and (d) together. We can project out unmatching column (street address) and make it like table (d)}

% % Moreover, Table (f) provides the \texttt{Street Address} information about the museums which the query table is not looking for. 
% % Hence, this table is good to be joined with the query table as it adds an extra column to the query table. 
% % However, it is not a proper fit for unioning. Recall that searching for the joinable tables is not under the scope of this work~\cite{2019_zhu_josie,lshEnsemble}.
% % Finally, we can also have  tables like Table (g) that only provides the name of the museums.
% % In fact, such tables are also not a good fit to be unioned because they are not offering any information that the user is looking for.
% % Just providing the names of the museums without any properties is not enough.

% % Based on these observations, we now provide our definition of unionability.  We later define a unionability score which will score Table X higher than Table Y...%, which we call \emph{\unionability}.


% % \subsubsection{Unionability Definition Revisited}

% % We now revisit the definition of unionability and introduce \unionability. 

% % \begin{definition}[SANTOS Table Unionability]
% % \label{definition:santos_unionability}
% % Let $Q$ be a Query Table with the semantic tree $T$ containing a intent columns $Q.S$, and additional 
% % property columns $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ having relations $Q.r_1$, $Q.r_2$ $\dots$ $Q.r_m$ with $Q.S$ respectively. %resolved
% % %\wolf{10/27: what are those relations? Q.S entry is S, Q.Pi header %is P, Q.Pi values is O?
% % %What about using m for the number of columns, and thus $P_{m-1}$ being the max?}
% % In addition, let $D$ be a data lake table with columns $D.A_1$, $D.A_2$ $\dots$ $D.A_n$. 
% % \wolf{10/27: you also use $n$ later for number of tables; best here to use $k$ or so. Also would $T$ easier than $D$ for table?} \aamod{10/28: T is used later on for the set of KB types.}
% % $D$ is \emph{SANTOS unionable} with a Query Table $Q$ if $D$ (1) contains a column $D.A_i$ such that $D.A_i$ is unionable with $Q.I$, (2) has at least one column $D.A_j$ ($i\neq j$) such that $D.A_j$ is unionable with some property $Q.P_k$ and (3) has relation between $D.A_i$  and $D.A_j$ that corresponds to $Q.r_k$.
% % \end{definition}

% % %resolved
% % %\wolf{10/27: above definition relies on an earlier definition of what it means for two columns to be unionable.
% % %It also requires a formal definition of relation.}


% % In simple words, \emph{a Data Lake Table D is \emph{SANTOS Unionable} with a Query Table Q if D contains the intent column of Q and at least one property column of Q having same relationship with the intent column.}

% % Our definition naturally provides a way of ranking the tables with a continuous unionability score that we will discuss later in \cref{section:semantic_union_search}.

% % % \begin{definition}[SANTOS Table Unionability]
% % % Let, $Q$ denotes a Query Table and $D$ denotes a Data Lake Table. Let, $Q.I$ be the intent column of $Q$ and $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ be its properties having relations $Q.r_1$, $Q.r_2$ $\dots$ $Q.r_m$ with $Q.I$ respectively. A data lake table D is SANTOS unionable with a Query Table Q if D contains a column $D.I$ such that  $D.I$ is unionable with $Q.I$ and has at least one $D.P_i$ such that $D.P_i$ is unionable with $Q.P_i$ and has relation $r_i$ with $D.I$ where, $i = 1, 2, \dots m$.
% % % \end{definition}
% % % Our definition naturally provides a way of ranking the tables with a continuous unionability score that we will discuss later in \cref{section:semantic_union_search}.



% % % \subsection{\unionability}\label{section:unionablity_def}
% % % \roee{shouldn't this be included in the next subsection? I think that this section should contained processing information of data lake tables (above) and query tables (here) without referring to the way we account for their unionability, which is introduced in the next section: Then Q and D are considered unionable only if the D's semantic tree (1) contains a node of the same type as the intent column and
% % % (2) there is a large number of matches between their children as well.}

% % % In order to solve the problems seen in searching for the unionable tables, we introduce a notion of \unionability.
% % % We now revisit the definition of unionability and introduce \unionability. 
% % % \wolf{10/21: what about calling this just ``semantic unionability'' to separate the approach (using relationships = semantics of tables) from the name of one particular instantiation of a system that uses semantics (SANTOS)} \roee{The reason we need a ``new'' name is that the TUS paper uses the term ``semantic unionability'' and it is diffrent from what we describe in this paper}



% % % \begin{definition}[\unionability]
% % % A data lake table D is unionable with Query Table Q if D contains the intent column of Q and as many property columns of Q with same relations as possible. 
% % % \wolf{10/21: what are ``relations'' here exactly? 
% % % You see, S-P-O are between instances: S and O are usually cell values, P are either 1. column names (or if missing the abstract concept for which there are instances, or 2. table names as a whole [like in a binary table]. }
% % % In worst case, 
% % % \wolf{10/21: better no ``worst cases" for formal definitions: better to define concepts binary: yes or now}
% % % D must contain the intent column of Q and at least one property column from Q with the same relation.
% % % \zixuan{as many property as possible here looks confusing. I prefer to rewrite this to: "A data lake table D is unionable with a Query Table Q if D contains the intent column of Q and at least one property column from Q with the same relation." Then if we want to show the concept of unionability score which is if D contains more property columns of Q, then D gets higher unionability score, we may need to propose a new definition.}
% % % \end{definition}

% % % \roee{suggested definition:
% % % \begin{definition}[\unionability]
% % % Let $Q$ be a query table with the intent column $Q.S$ and set of its properties $Q.P_1$, $Q.P_2$ $\dots$ $Q.P_m$ having relationship with $Q.S$. A data table $D$ is SANTOS unionable with $Q$ is it has the same intent column as $Q.S$ with at least one property from $Q.P$.
% % % \end{definition}}
% % % \aamod{10/22: @Roee, this definition looks good and we were using it before. But it missed the relation semantics part. This will consider president-birthplace-city and president-deathplace-city as same which we don't want. We need to somehow preserve the relationship between the columns.}

% % Hereafter, whenever we say unionablity, we mean \unionability \ unless mentioned otherwise. The formal definition refer to the minimal conditions for \unionability. However, in practice, we wish to find unionable tables that contain the same intent column as the query table and \emph{as many properties with same relation as possible}.

% % \aamod{10/25: I would advocate to move the definition of SANTOS Problem below either to \cref{section:semantic_union_search} so that we can also include the scoring function details or to section 1 and make it generic.}

% % Next, we define the problem of searching for the unionable tables formally.

% % \begin{definition}[Semantic Table Union Search (SANTOS) Problem]
% % Given a set of Data lake Tables $\mathcal{D}$ = \{$D_1$, $D_2$, \dots $D_n$\}, 
% % % \wolf{10/21: better replace x as variable with m or n for a constant}
% % a Query Table $Q$ with a intent column $Q.S$, a knowledge base $\mathcal{K}$, a positive integer $k$ and a scoring function $f(\mathcal D, Q, Q.S, \mathcal K , k)$ such that $k\leq n$, SANTOS problem is to search for the top-k Data lake Tables that are unionable with $Q$.
% % \end{definition}

% % \wolf{10/27: Above definition requires a scoring function by which one can rank}


% % % \begin{definition}[Semantic Table Union Search (SANTOS) Problem]
% % % Given a set of Data lake Tables \{$D_1$, $D_2$, \dots $D_x$\}, 
% % % \wolf{10/21: better replace x as variable with m or n for a constant}
% % % a Query Table Q, an intent column I marked in the Query Table and a positive integer k such that $k \leq x$, SANTOS problem is to search for the top-k Data lake Tables that are unionable with Q.
% % % \end{definition}

% % \wolf{10/21: suggestion: would it makes sense to first define early the table union search problem, without any mentioning of concepts from this paper. E.g. table union search is defined as INPUT: query table, repository, k. OUTPUT: top-k tables that are 1. most unable 2. independently (thus they are not integrated together, just added independently: that seems to be the definition here. Then explain that 1. they key problem is to design a good metric of ``most unable''. Earlier work tried to do this just based on pairwise column comparisons and then aggregating those individual pairwise comparisons into an overall score. This work suggest and *improved* measure that also takes into account the relative relations among columns (thus input is not just sets (or bags) of words = column independently: a table is a set of columsn, but rather, the 2nd dimensions: rows}
% % \roee{I think we can go either way. Have an intuitive discussion about unionability and why earlier work is different and formally define it here.} \roee{In addition, the problem definition here is different since we require a intent column being annotated in the query table}

% % \aamod{10/19: In the definition of SANTOS problem above, Should we also consider knowledge base as a given entity?}

% % \roee{In the reminder of the Section we can decide if we want to elaborate more on the way we solve the problem before we actually solve it (n the populated text), have a more formal discussion with respect for example to the semantic web community or provide steps for actually applying the unionability (second comment be Wolfgang). @Aamod, after reading the section again, try to say what is expected here. It may also be a short description of what we aim to do in the reminder of the paper in this context: `` In the following sections we suggest KB to generate semantic trees for tables, then we..."}

% % Once a user provides \emph{Q} marked with intent column \emph{I} and its properties, 
% % we represent it in the form of a semantic tree as discussed before.
% % \wolf{10/21: really needs an intuitve annotated figure. It seems there are two perspectives:
% % 1. the triples: S-P-O at the instance level: S and O are from cell values, P are from a column as a whole
% % 2. a binary representation: S-P1, S-P2: S here is the column of the individual intents. Pi are the columns as a whole. 
% % It seems obvious that way, but by explicitly mentioning these different views, it will help people say from the sematnic web community (where everything is S-P-O) to follow along}
% % After that we extract all the data lake tables containing the intent column and at least one of its properties. 
% % Next, we project out the matching columns with the query table and form a semantic tree for the data lake table. 
% % Finally, we compare two semantic trees and determine the unionability score.
% % \wolf{10/21: those are 4 steps that may be numbered, named 
% % (1. query table interpretation, 2. candidate table filtering, 3. candidate table interpretation,
% % 4. candidate table scoring), and then later referred to again in more detailed.
% % Question: do you envison that *every* implementation of a table union search paradigm needs to follow these 4 steps 
% % (thus this is generic, and only the measure for 4 is new), or was there already some design decison made to choose that process instead of any other one can come up with?}

% % It is not always accurate to use the column names or the column values to create the semantic trees. 
% % For example, \texttt{Name} in \cref{fig:entity_films} and \texttt{Film Title} in \cref{fig:relation_parks_films} have different column names and column values although they are unionable. 
% % Conversely, there can also be the columns having same name but different semantics. 
% % For instance, column \texttt{Name} of table in \cref{fig:entity_films} represents \textit{film name} whereas, column \texttt{Name} of Table (b) in \cref{fig:crime_and_musuem_tables} represents the name of the museums. 
% % Also, all the open data lake tables may not have the column name information. Therefore, instead of using such weak signals, we use a knowledge base to annotate the semantic graphs.
% % \wolf{10/21: important distinction: do you perform that labeling based on column names only, or rather by also looking at the cell values in a column, or even by looking at the values in a column you like to label and also the neighboring values or column names (because of increased signal from the 2nd dimsion of tables)?}
% % \aamod{10/25: We use values in the column together with its neighboring values.}
% % More precisely, we use knowledge base types to annotate the nodes and Knowledge base properties to annotate the edges. If the entities are not covered by the knowledge base, we also take a help of a synthetic knowledge base to annotate the query table that we create using the data lake tables.
% % During query time, we compare the number of matching annotations between the query table and the data lake tables to determine the unionability score. We will explain the annotation details in \cref{section:unionability_components}, synthetic knowledge base in \cref{section:synthetic_knowledge_base} and unionability score in \cref{section:semantic_union_search}.

